Categories generated by a trivalent vertex

This is the first paper in a general program to automate skein theoretic arguments. In this paper, we study skein theoretic invariants of planar trivalent graphs. Equivalently, we classify trivalent categories, which are nondegenerate pivotal tensor categories over $\mathbb C$ generated by a symmetric self-dual simple object $X$ and a rotationally invariant morphism $1 \rightarrow X \otimes X \otimes X$. Our main result is that the only trivalent categories with $\dim \operatorname{Hom}(1, X^{\otimes n})$ bounded by $1,0,1,1,4,11,40$ for $0 \leq n \leq 6$ are quantum $SO(3)$, quantum $G_2$, a one-parameter family of free products of certain Temperley-Lieb categories (which we call ABA categories), and the $H3$ Haagerup fusion category. We also prove similar results where the map $1 \rightarrow X^{\otimes 3}$ is not rotationally invariant, and we give a complete classification of nondegenerate braided trivalent categories with dimensions of invariant spaces bounded by $1,0,1,1,4$. Our main techniques are a new approach to finding skein relations which can be easily automated using Gr\"obner bases, and evaluation algorithms which use the discharging method developed in the proof of the $4$-color theorem.

==> polynomials/Q_11,19.tex <==
40 t^{19}-468 t^{18}+2168 t^{17}-4681 t^{16}+1776 t^{15}+13663 t^{14}-24528 t^{13}-4787 t^{12}+47802 t^{11}-22763 t^{10}-43836 t^9+38169 t^8+21052 t^7-28775 t^6-4266 t^5+12220 t^4-512 t^3-3072 t^2+288 t+d^{11} \left(56 t^{18}+104 t^{17}-260 t^{16}-968 t^{15}-816 t^{14}+824 t^{13}+2310 t^{12}+1618 t^{11}-755 t^{10}-2430 t^9-2120 t^8-666 t^7+487 t^6+780 t^5+539 t^4+236 t^3+68 t^2+12 t+1\right)+d^4 \left(-5408 t^{19}+35942 t^{18}-51594 t^{17}-99884 t^{16}+242134 t^{15}+144908 t^{14}-476774 t^{13}-201952 t^{12}+545699 t^{11}+195536 t^{10}-511033 t^9-165727 t^8+443367 t^7+225939 t^6-209849 t^5-185177 t^4+1683 t^3+47502 t^2+19887 t+3038\right)+d^5 \left(-5184 t^{19}+25180 t^{18}-3220 t^{17}-111623 t^{16}+15352 t^{15}+300300 t^{14}+48612 t^{13}-557713 t^{12}-288157 t^{11}+549170 t^{10}+401051 t^9-351247 t^8-330674 t^7+169464 t^6+243095 t^5+9975 t^4-80655 t^3-35155 t^2-3010 t+507\right)+d^3 \left(-2608 t^{19}+21544 t^{18}-50956 t^{17}-14294 t^{16}+196932 t^{15}-123279 t^{14}-301918 t^{13}+331415 t^{12}+203319 t^{11}-501794 t^{10}-33749 t^9+565540 t^8+48573 t^7-414073 t^6-134692 t^5+152114 t^4+97544 t^3-13699 t^2-26382 t-6364\right)+d^6 \left(-1472 t^{19}+1788 t^{18}+20296 t^{17}-16361 t^{16}-120254 t^{15}+33715 t^{14}+327823 t^{13}+18835 t^{12}-566416 t^{11}-324616 t^{10}+402761 t^9+434332 t^8-94552 t^7-270715 t^6-40004 t^5+103715 t^4+57781 t^3-259 t^2-7837 t-1702\right)+d^2 \left(-384 t^{19}+3956 t^{18}-12664 t^{17}+7489 t^{16}+31550 t^{15}-48828 t^{14}+7560 t^{13}+50436 t^{12}-140984 t^{11}+16037 t^{10}+293943 t^9-48561 t^8-328729 t^7+12285 t^6+221932 t^5+19987 t^4-90948 t^3-20748 t^2+16796 t+5928\right)+d^{10} \left(96 t^{19}+436 t^{18}-224 t^{17}-3520 t^{16}-4470 t^{15}+3434 t^{14}+11338 t^{13}+3858 t^{12}-12858 t^{11}-16823 t^{10}-3410 t^9+9852 t^8+9913 t^7+1675 t^6-4321 t^5-4764 t^4-2627 t^3-883 t^2-175 t-16\right)+d \left(128 t^{19}-1276 t^{18}+4940 t^{17}-7492 t^{16}-8142 t^{15}+43612 t^{14}-16713 t^{13}-106439 t^{12}+77826 t^{11}+163472 t^{10}-135781 t^9-168241 t^8+138992 t^7+118644 t^6-87619 t^5-58068 t^4+30816 t^3+17732 t^2-4808 t-2624\right)+d^9 \left(672 t^{19}+464 t^{18}-4340 t^{17}-8813 t^{16}+4032 t^{15}+22154 t^{14}+1864 t^{13}-41695 t^{12}-35098 t^{11}+20996 t^{10}+42100 t^9+733 t^8-40121 t^7-34725 t^6-5381 t^5+11700 t^4+10877 t^3+4714 t^2+1104 t+114\right)+d^7 \left(1616 t^{19}-7232 t^{18}+1856 t^{17}+31458 t^{16}-32262 t^{15}-109673 t^{14}+39663 t^{13}+222886 t^{12}+18147 t^{11}-344481 t^{10}-269142 t^9+132371 t^8+269612 t^7+68113 t^6-95344 t^5-72031 t^4-2103 t^3+17366 t^2+7946 t+1191\right)+d^8 \left(1752 t^{19}-2918 t^{18}-9598 t^{17}+5933 t^{16}+24208 t^{15}-14786 t^{14}-71683 t^{13}-17226 t^{12}+95163 t^{11}+56806 t^{10}-106899 t^9-152630 t^8-30443 t^7+75353 t^6+63863 t^5+6832 t^4-18457 t^3-13007 t^2-3886 t-470\right)+384

==> polynomials/Q_21,33.tex <==
-9 t^{29}+299 t^{28}-3799 t^{27}+25701 t^{26}-102525 t^{25}+235735 t^{24}-217903 t^{23}-347781 t^{22}+1284982 t^{21}-1165201 t^{20}-976223 t^{19}+2936180 t^{18}-1624461 t^{17}-1632262 t^{16}+3007626 t^{15}-1755003 t^{14}-1050408 t^{13}+3357932 t^{12}-1491391 t^{11}-2490239 t^{10}+2003800 t^9+1124744 t^8-1118504 t^7-366432 t^6+332396 t^5+91238 t^4-46221 t^3-13534 t^2+1056 t+d \left(-4 t^{32}+101 t^{31}-1246 t^{30}+9816 t^{29}-52026 t^{28}+178806 t^{27}-340911 t^{26}+73138 t^{25}+1246169 t^{24}-2442818 t^{23}-133696 t^{22}+5810364 t^{21}-4039063 t^{20}-8172991 t^{19}+8948626 t^{18}+10731407 t^{17}-13390808 t^{16}-13148547 t^{15}+15276241 t^{14}+12667825 t^{13}-11229393 t^{12}-9279731 t^{11}+3654612 t^{10}+5138231 t^9+1149312 t^8-1928518 t^7-1619772 t^6+350334 t^5+632281 t^4+27046 t^3-97797 t^2-18468 t+832\right)+d^{12} \left(-20592 t^{33}+305136 t^{32}-1489189 t^{31}+2148484 t^{30}+5654323 t^{29}-22479574 t^{28}+8057824 t^{27}+71938028 t^{26}-99971446 t^{25}-107365044 t^{24}+335512343 t^{23}+12922154 t^{22}-745252527 t^{21}+252755745 t^{20}+1282764149 t^{19}-465937688 t^{18}-1663776789 t^{17}+524650436 t^{16}+1868206308 t^{15}-108465231 t^{14}-1476701770 t^{13}-243873178 t^{12}+865806895 t^{11}+397114857 t^{10}-271353404 t^9-247103605 t^8+5877510 t^7+72841191 t^6+28147637 t^5+388237 t^4-1736506 t^3-34393 t^2+147351 t+24507\right)+d^{11} \left(-18304 t^{33}+233376 t^{32}-1112397 t^{31}+2389387 t^{30}-1425202 t^{29}-5614277 t^{28}+24141945 t^{27}-40245095 t^{26}-46448480 t^{25}+243297921 t^{24}-38868126 t^{23}-695330936 t^{22}+303230093 t^{21}+1344212174 t^{20}-620644227 t^{19}-1960474599 t^{18}+750393775 t^{17}+2338925517 t^{16}-360736806 t^{15}-1987191382 t^{14}+21940719 t^{13}+1426619801 t^{12}+348417574 t^{11}-645029072 t^{10}-330451131 t^9+152578655 t^8+158004700 t^7+19528805 t^6-18951819 t^5-6966884 t^4-727021 t^3-395666 t^2-232847 t-37599\right)+d^{13} \left(-9464 t^{33}+184444 t^{32}-845195 t^{31}+188279 t^{30}+7491541 t^{29}-13235801 t^{28}-23653762 t^{27}+76546889 t^{26}+27724897 t^{25}-237154301 t^{24}+28537133 t^{23}+491828005 t^{22}-181342687 t^{21}-783665112 t^{20}+405926131 t^{19}+1137056929 t^{18}-393761129 t^{17}-1275960229 t^{16}+197870445 t^{15}+1191421514 t^{14}+157630991 t^{13}-785061986 t^{12}-340961031 t^{11}+317303715 t^{10}+278485232 t^9-26734148 t^8-110296624 t^7-38237746 t^6+9624466 t^5+10422568 t^4+2531630 t^3-63489 t^2-127036 t-16399\right)+d^{10} \left(-8216 t^{33}+40508 t^{32}+171509 t^{31}-1029392 t^{30}-2637662 t^{29}+22565503 t^{28}-22862398 t^{27}-100889301 t^{26}+205670084 t^{25}+207946648 t^{24}-718899177 t^{23}-211238260 t^{22}+1533515681 t^{21}+14726704 t^{20}-2314066679 t^{19}+257616195 t^{18}+2652304736 t^{17}-358019487 t^{16}-2349020650 t^{15}+359240322 t^{14}+1912782995 t^{13}+112960166 t^{12}-1031584291 t^{11}-275009991 t^{10}+351478301 t^9+192654914 t^8-31694138 t^7-49254602 t^6-17350825 t^5-7139574 t^4-3475849 t^3-664618 t^2+89528 t+35320\right)+d^6 \left(-1008 t^{33}+3504 t^{32}+34359 t^{31}-114276 t^{30}-768012 t^{29}+3713305 t^{28}+1443714 t^{27}-31825072 t^{26}+34657698 t^{25}+95972336 t^{24}-182056666 t^{23}-147303386 t^{22}+437310079 t^{21}+147776268 t^{20}-662277379 t^{19}-165132970 t^{18}+720688245 t^{17}+300622644 t^{16}-597106644 t^{15}-568177708 t^{14}+276251433 t^{13}+757307781 t^{12}+222264410 t^{11}-479116395 t^{10}-418129418 t^9+23253749 t^8+172017961 t^7+71770117 t^6-2528715 t^5-9869914 t^4-4108287 t^3-1291733 t^2-123960 t+47634\right)+d^5 \left(-692 t^{33}+10286 t^{32}-88173 t^{31}+584817 t^{30}-2630330 t^{29}+6232342 t^{28}-1534262 t^{27}-27248317 t^{26}+46128995 t^{25}+36476291 t^{24}-149179853 t^{23}+5151263 t^{22}+269370016 t^{21}-63461993 t^{20}-357791266 t^{19}+26775820 t^{18}+428844187 t^{17}+170299382 t^{16}-481262283 t^{15}-470475918 t^{14}+380127518 t^{13}+665381727 t^{12}-50656565 t^{11}-499498785 t^{10}-194973341 t^9+136486851 t^8+133931680 t^7+25379132 t^6-19734031 t^5-14539197 t^4-2655738 t^3+815682 t^2+249466 t-26834\right)+d^9 \left(-624 t^{33}-95160 t^{32}+1186029 t^{31}-5035095 t^{30}+4716635 t^{29}+27026215 t^{28}-74313872 t^{27}-22881222 t^{26}+287411168 t^{25}-150588603 t^{24}-610835987 t^{23}+598887297 t^{22}+835519050 t^{21}-1202614127 t^{20}-756578834 t^{19}+1677518127 t^{18}+414332501 t^{17}-1860869727 t^{16}-155435157 t^{15}+1739069642 t^{14}+376219713 t^{13}-960210684 t^{12}-323514336 t^{11}+357575027 t^{10}+188430845 t^9-61521430 t^8-76227385 t^7-39910192 t^6-18677882 t^5-1588431 t^4+4086401 t^3+1898712 t^2+220738 t-15966\right)+d^7 \left(-352 t^{33}-37864 t^{32}+524879 t^{31}-2657401 t^{30}+5514728 t^{29}-79935 t^{28}-16383345 t^{27}+12779168 t^{26}+11565547 t^{25}+22945661 t^{24}-15459345 t^{23}-210635809 t^{22}+125574899 t^{21}+554026781 t^{20}-366338283 t^{19}-872115637 t^{18}+579267625 t^{17}+948351069 t^{16}-618799567 t^{15}-825435412 t^{14}+432504462 t^{13}+687361200 t^{12}+45764814 t^{11}-266918369 t^{10}-227908801 t^9-113960893 t^8+13745269 t^7+66263191 t^6+37411741 t^5+5867440 t^4-1702365 t^3-950868 t^2-325447 t-76436\right)+d^4 \left(-248 t^{33}+4660 t^{32}-46616 t^{31}+311681 t^{30}-1341356 t^{29}+3172879 t^{28}-1654825 t^{27}-10168432 t^{26}+19241858 t^{25}+12834701 t^{24}-57737333 t^{23}-11574625 t^{22}+136326302 t^{21}+1683799 t^{20}-269618725 t^{19}+24963393 t^{18}+423331991 t^{17}-32152480 t^{16}-515374573 t^{15}-45582056 t^{14}+451971055 t^{13}+174671774 t^{12}-223896082 t^{11}-198454191 t^{10}+5137235 t^9+91110724 t^8+48930362 t^7-7614291 t^6-16683493 t^5-4069450 t^4+775751 t^3+269077 t^2+50760 t+33678\right)+d^3 \left(-48 t^{33}+948 t^{32}-9512 t^{31}+60362 t^{30}-228074 t^{29}+344153 t^{28}+794032 t^{27}-4158130 t^{26}+3484202 t^{25}+12817842 t^{24}-26430381 t^{23}-17106945 t^{22}+84008249 t^{21}-8809402 t^{20}-167688323 t^{19}+75987831 t^{18}+237941769 t^{17}-136406219 t^{16}-264457523 t^{15}+121759787 t^{14}+237968106 t^{13}-37599874 t^{12}-158329422 t^{11}-30655817 t^{10}+63969876 t^9+33450642 t^8-11183074 t^7-10730200 t^6+316119 t^5+924882 t^4-286447 t^3-26852 t^2+52887 t+1272\right)+d^2 \left(-4 t^{33}+62 t^{32}-351 t^{31}-492 t^{30}+24796 t^{29}-204882 t^{28}+877342 t^{27}-1944350 t^{26}+922786 t^{25}+5816929 t^{24}-11959938 t^{23}-1762644 t^{22}+29099690 t^{21}-14356662 t^{20}-46813836 t^{19}+35913851 t^{18}+66680782 t^{17}-54487947 t^{16}-85713379 t^{15}+59403217 t^{14}+90322656 t^{13}-43862753 t^{12}-70529901 t^{11}+18993515 t^{10}+36700497 t^9-3230236 t^8-11009237 t^7-511821 t^6+1320003 t^5+226778 t^4+128615 t^3-5650 t^2-50804 t-10464\right)+d^{21} \left(12 t^{33}+6 t^{32}-212 t^{31}-364 t^{30}+765 t^{29}+2655 t^{28}+900 t^{27}-5202 t^{26}-6562 t^{25}+1426 t^{24}+7992 t^{23}+4502 t^{22}-2120 t^{21}-3435 t^{20}-1065 t^{19}+414 t^{18}+365 t^{17}+61 t^{16}-20 t^{15}-9 t^{14}-t^{13}\right)+d^{20} \left(168 t^{33}-164 t^{32}-2895 t^{31}-461 t^{30}+15961 t^{29}+12811 t^{28}-43111 t^{27}-52866 t^{26}+83992 t^{25}+163607 t^{24}-54784 t^{23}-304081 t^{22}-160680 t^{21}+208275 t^{20}+305865 t^{19}+75129 t^{18}-135430 t^{17}-135913 t^{16}-35160 t^{15}+25810 t^{14}+27301 t^{13}+10690 t^{12}+1081 t^{11}-899 t^{10}-500 t^9-126 t^8-17 t^7-t^6\right)+d^8 \left(896 t^{33}-98456 t^{32}+1163847 t^{31}-5445050 t^{30}+9561367 t^{29}+9684364 t^{28}-60837808 t^{27}+46192293 t^{26}+122426962 t^{25}-200341484 t^{24}-76359578 t^{23}+320422371 t^{22}-137188401 t^{21}-201089233 t^{20}+422992429 t^{19}-114983447 t^{18}-629678358 t^{17}+287425473 t^{16}+576779915 t^{15}-195899686 t^{14}-216936837 t^{13}+233053625 t^{12}+133291897 t^{11}-79461443 t^{10}-53210959 t^9-53808149 t^8-83625517 t^7-30973380 t^6+21840341 t^5+20145844 t^4+4926190 t^3+135278 t^2+22803 t+37919\right)+d^{19} \left(1072 t^{33}-2580 t^{32}-15639 t^{31}+23303 t^{30}+89872 t^{29}-91688 t^{28}-336217 t^{27}+215319 t^{26}+1009536 t^{25}-7967 t^{24}-1888803 t^{23}-823071 t^{22}+2344037 t^{21}+2074846 t^{20}-1948308 t^{19}-3538747 t^{18}-280227 t^{17}+3077286 t^{16}+2548585 t^{15}-183066 t^{14}-1676239 t^{13}-1180169 t^{12}-120418 t^{11}+381343 t^{10}+317335 t^9+109214 t^8-7095 t^7-28643 t^6-16920 t^5-5976 t^4-1421 t^3-226 t^2-22 t-1\right)+d^{18} \left(4092 t^{33}-15402 t^{32}-40554 t^{31}+161316 t^{30}+159950 t^{29}-811237 t^{28}-505072 t^{27}+2613141 t^{26}+1797222 t^{25}-5411405 t^{24}-4542515 t^{23}+8766494 t^{22}+10632092 t^{21}-8236325 t^{20}-17789356 t^{19}-569758 t^{18}+16137297 t^{17}+8301487 t^{16}-8049772 t^{15}-9356589 t^{14}+1008709 t^{13}+6721976 t^{12}+3609935 t^{11}-1183415 t^{10}-2534442 t^9-1332355 t^8-74889 t^7+335952 t^6+250563 t^5+102153 t^4+27110 t^3+4716 t^2+495 t+24\right)+d^{14} \left(7696 t^{33}-6400 t^{32}-83619 t^{31}-441348 t^{30}+2805088 t^{29}-74177 t^{28}-18900914 t^{27}+13769054 t^{26}+66691506 t^{25}-66540076 t^{24}-168324792 t^{23}+165026836 t^{22}+334857334 t^{21}-247306225 t^{20}-490711954 t^{19}+319313958 t^{18}+681371282 t^{17}-211419263 t^{16}-743660696 t^{15}-34410517 t^{14}+577398132 t^{13}+225125473 t^{12}-278002257 t^{11}-235366366 t^{10}+35523424 t^9+112621670 t^8+35305263 t^7-20046032 t^6-19275838 t^5-5476381 t^4+140347 t^3+488893 t^2+122537 t+10636\right)+d^{17} \left(10256 t^{33}-51188 t^{32}-36294 t^{31}+478393 t^{30}-236459 t^{29}-2184521 t^{28}+1848686 t^{27}+6495435 t^{26}-5854692 t^{25}-14224646 t^{24}+12633845 t^{23}+28371429 t^{22}-13133475 t^{21}-40160330 t^{20}+7412849 t^{19}+44579692 t^{18}-288967 t^{17}-48168081 t^{16}-19987369 t^{15}+31699108 t^{14}+31732257 t^{13}-3394900 t^{12}-19642985 t^{11}-8324703 t^{10}+5053007 t^9+6697633 t^8+2161499 t^7-941652 t^6-1298368 t^5-669364 t^4-207346 t^3-40601 t^2-4694 t-247\right)+d^{16} \left(17216 t^{33}-102376 t^{32}+64133 t^{31}+682178 t^{30}-1301134 t^{29}-1896603 t^{28}+6324087 t^{27}+1653164 t^{26}-18139417 t^{25}+4799925 t^{24}+38744279 t^{23}-16852454 t^{22}-59779048 t^{21}+43820871 t^{20}+103031645 t^{19}-44991259 t^{18}-148099703 t^{17}-8750328 t^{16}+132336721 t^{15}+56125683 t^{14}-78137474 t^{13}-71761396 t^{12}+16293497 t^{11}+48794572 t^{10}+17857651 t^9-10966757 t^8-12204485 t^7-2840920 t^6+2018763 t^5+1935423 t^4+783681 t^3+182777 t^2+24112 t+1412\right)+d^{15} \left(18144 t^{33}-111192 t^{32}+167037 t^{31}+242205 t^{30}-1129980 t^{29}+1335571 t^{28}+1152129 t^{27}-9846574 t^{26}+8190971 t^{25}+33302079 t^{24}-41969721 t^{23}-82457415 t^{22}+109267078 t^{21}+191257677 t^{20}-127335747 t^{19}-285534872 t^{18}+90020974 t^{17}+328533549 t^{16}-5253966 t^{15}-304611991 t^{14}-112159679 t^{13}+172056996 t^{12}+144629975 t^{11}-32000049 t^{10}-86810759 t^9-28381943 t^8+18311914 t^7+18500157 t^6+4865333 t^5-1294653 t^4-1349643 t^3-441440 t^2-71617 t-4878\right)+288

==> polynomials/Q_22,36.tex <==
8 t^{33}-216 t^{32}+2568 t^{31}-17122 t^{30}+65916 t^{29}-117755 t^{28}-116186 t^{27}+1067362 t^{26}-1771185 t^{25}-1400289 t^{24}+8626014 t^{23}-6580216 t^{22}-16049970 t^{21}+29571036 t^{20}+9540828 t^{19}-57285027 t^{18}+16762322 t^{17}+67623090 t^{16}-45437258 t^{15}-53414489 t^{14}+54270634 t^{13}+29707719 t^{12}-41413709 t^{11}-12659985 t^{10}+21791274 t^9+4955925 t^8-7849629 t^7-1996017 t^6+1729833 t^5+646918 t^4-134920 t^3-100862 t^2-17456 t+d \left(16 t^{34}-380 t^{33}+3624 t^{32}-15192 t^{31}-1135 t^{30}+298116 t^{29}-1257878 t^{28}+1502829 t^{27}+4425315 t^{26}-16650828 t^{25}+8088638 t^{24}+48435555 t^{23}-76936982 t^{22}-54361856 t^{21}+207870877 t^{20}-24306724 t^{19}-325190482 t^{18}+167076168 t^{17}+344099207 t^{16}-273140213 t^{15}-267434949 t^{14}+276092777 t^{13}+165026805 t^{12}-200686071 t^{11}-89446109 t^{10}+108948871 t^9+45938311 t^8-42333379 t^7-21122490 t^6+9678484 t^5+6960198 t^4-320343 t^3-1037290 t^2-250822 t-18368\right)+d^2 \left(112 t^{34}-3216 t^{33}+38476 t^{32}-240823 t^{31}+757355 t^{30}-362591 t^{29}-5719786 t^{28}+17690771 t^{27}-4797244 t^{26}-73935218 t^{25}+120559991 t^{24}+103332257 t^{23}-424238818 t^{22}+74335825 t^{21}+801474161 t^{20}-514505376 t^{19}-983013231 t^{18}+960516818 t^{17}+840867709 t^{16}-1095982240 t^{15}-506010722 t^{14}+899531392 t^{13}+203514098 t^{12}-587550124 t^{11}-60524928 t^{10}+322649647 t^9+40328087 t^8-140091404 t^7-41948448 t^6+35925768 t^5+22239278 t^4-545340 t^3-3843080 t^2-1201080 t-114632\right)+d^{10} \left(-106080 t^{36}+1294176 t^{35}-5343936 t^{34}+2658578 t^{33}+44076240 t^{32}-110064422 t^{31}-70144342 t^{30}+577079805 t^{29}-294370598 t^{28}-1540101363 t^{27}+1541751023 t^{26}+2906841192 t^{25}-3447419887 t^{24}-5139414419 t^{23}+4952281102 t^{22}+9508264997 t^{21}-4932067441 t^{20}-16272755902 t^{19}+2506971908 t^{18}+23165822896 t^{17}+3900912955 t^{16}-24559032642 t^{15}-13634926185 t^{14}+13534001728 t^{13}+15158228049 t^{12}+717280634 t^{11}-4492348224 t^{10}-809431281 t^9+1538988087 t^8+916775648 t^7+24784332 t^6-183501960 t^5-99009166 t^4-26894741 t^3-4013141 t^2-270938 t-1529\right)+d^{11} \left(-95472 t^{36}+1150968 t^{35}-4770792 t^{34}+3834090 t^{33}+28580214 t^{32}-76403184 t^{31}-18353860 t^{30}+276096914 t^{29}-137590900 t^{28}-527771424 t^{27}+233006925 t^{26}+947854310 t^{25}+363088084 t^{24}-2252937924 t^{23}-1908438027 t^{22}+4962974885 t^{21}+3805212688 t^{20}-7962265747 t^{19}-4913991352 t^{18}+9768066378 t^{17}+5259552422 t^{16}-10241347524 t^{15}-7822504862 t^{14}+5762901537 t^{13}+9116927518 t^{12}+2983828844 t^{11}-1476951183 t^{10}-1445975076 t^9-76461386 t^8+507952639 t^7+356471885 t^6+101597482 t^5-2310156 t^4-11610447 t^3-3991903 t^2-640845 t-43061\right)+d^9 \left(-79968 t^{36}+1028160 t^{35}-4534152 t^{34}+2884414 t^{33}+39911082 t^{32}-111838260 t^{31}-59240122 t^{30}+666097352 t^{29}-526154179 t^{28}-1854585102 t^{27}+2948763587 t^{26}+2968595503 t^{25}-7673356110 t^{24}-3232634882 t^{23}+12967946890 t^{22}+3894697154 t^{21}-15693853385 t^{20}-7622379609 t^{19}+13007951363 t^{18}+14139703390 t^{17}-3356495640 t^{16}-16227467887 t^{15}-8470518191 t^{14}+7077218397 t^{13}+9098132033 t^{12}+1541283190 t^{11}-941067058 t^{10}+1160364623 t^9+1291374739 t^8-184076738 t^7-698804208 t^6-353510005 t^5-60553974 t^4+9159331 t^3+5928299 t^2+1039324 t+65767\right)+d^8 \left(-44064 t^{36}+603024 t^{35}-2923408 t^{34}+3153810 t^{33}+22287116 t^{32}-76480490 t^{31}-15639456 t^{30}+457980711 t^{29}-508713851 t^{28}-1246091646 t^{27}+2771739078 t^{26}+1442316366 t^{25}-7467218018 t^{24}+734256211 t^{23}+12769419719 t^{22}-5205035098 t^{21}-14847150708 t^{20}+8974254737 t^{19}+10938868435 t^{18}-10153075981 t^{17}-2256387449 t^{16}+12027765029 t^{15}-3414978419 t^{14}-15667971629 t^{13}-1899892660 t^{12}+11154117956 t^{11}+7737283861 t^{10}+110375481 t^9-2425088692 t^8-1650525412 t^7-581416046 t^6-40397626 t^5+81542146 t^4+46602715 t^3+11899351 t^2+1517407 t+90571\right)+d^{12} \left(-38896 t^{36}+602888 t^{35}-3171064 t^{34}+6057298 t^{33}+5630300 t^{32}-42479372 t^{31}+52502910 t^{30}+42382697 t^{29}-178730659 t^{28}+183499919 t^{27}+75901603 t^{26}-613967470 t^{25}+634672730 t^{24}+929891307 t^{23}-1720903443 t^{22}-1072893332 t^{21}+2409229383 t^{20}+1679824589 t^{19}-1736342620 t^{18}-2747965931 t^{17}-893474839 t^{16}+1621909560 t^{15}+2091233246 t^{14}+901911459 t^{13}+812118610 t^{12}+1457281389 t^{11}+926245290 t^{10}-156899617 t^9-451372557 t^8-145978446 t^7+78024136 t^6+87980417 t^5+37863517 t^4+9447585 t^3+1447631 t^2+132015 t+6038\right)+d^7 \left(-17952 t^{36}+261936 t^{35}-1417984 t^{34}+2503014 t^{33}+6533022 t^{32}-33419986 t^{31}+14294720 t^{30}+161037956 t^{29}-246144412 t^{28}-416788723 t^{27}+1237075495 t^{26}+274584282 t^{25}-3427871743 t^{24}+1685603502 t^{23}+5704825059 t^{22}-6530599650 t^{21}-5220772405 t^{20}+13527857983 t^{19}+319023359 t^{18}-21349105528 t^{17}+5568497803 t^{16}+29028329087 t^{15}-4102992258 t^{14}-31149104781 t^{13}-6801246181 t^{12}+19630552788 t^{11}+12751097644 t^{10}-3080637809 t^9-6041127122 t^8-1948935218 t^7+366103838 t^6+445444858 t^5+145894071 t^4+27126485 t^3+3335781 t^2+102172 t-54948\right)+d^6 \left(-5304 t^{36}+82416 t^{35}-503832 t^{34}+1336260 t^{33}-51534 t^{32}-8934168 t^{31}+21392338 t^{30}-12416379 t^{29}-28429808 t^{28}+68415806 t^{27}-68899102 t^{26}-50968433 t^{25}+206219497 t^{24}+219522043 t^{23}-533302125 t^{22}-1689789077 t^{21}+2119265267 t^{20}+5912259212 t^{19}-5701096737 t^{18}-13602522861 t^{17}+8447201613 t^{16}+22767026979 t^{15}-4453354542 t^{14}-26153369478 t^{13}-5875311512 t^{12}+17297385954 t^{11}+11080204095 t^{10}-3934161814 t^9-6280555968 t^8-1428825604 t^7+994715232 t^6+662845289 t^5+106023559 t^4-24267404 t^3-11160409 t^2-1164841 t+43004\right)+d^5 \left(-1080 t^{36}+17832 t^{35}-124142 t^{34}+450402 t^{33}-624692 t^{32}-2429950 t^{31}+17440499 t^{30}-45583865 t^{29}+19445913 t^{28}+199479133 t^{27}-428424163 t^{26}-165070958 t^{25}+1451599566 t^{24}-583975460 t^{23}-2816785681 t^{22}+1705025721 t^{21}+4229948528 t^{20}-1413532510 t^{19}-5676519111 t^{18}-2152486286 t^{17}+6014880039 t^{16}+8159924021 t^{15}-2793011425 t^{14}-11649561926 t^{13}-3224955168 t^{12}+8371056193 t^{11}+6205104455 t^{10}-2011373106 t^9-3843765513 t^8-924652949 t^7+770389529 t^6+533862104 t^5+71761288 t^4-39970636 t^3-17965065 t^2-2940151 t-236224\right)+d^4 \left(-136 t^{36}+2380 t^{35}-18724 t^{34}+77508 t^{33}-32236 t^{32}-1707975 t^{31}+10297401 t^{30}-24720337 t^{29}-3325304 t^{28}+155539000 t^{27}-264973705 t^{26}-241680046 t^{25}+1140857118 t^{24}-304806677 t^{23}-2477067249 t^{22}+1784196436 t^{21}+3581064579 t^{20}-3236982893 t^{19}-3936580417 t^{18}+3011721386 t^{17}+3299499659 t^{16}-792223131 t^{15}-1393188204 t^{14}-1371191137 t^{13}-1106276654 t^{12}+1341941768 t^{11}+2231629725 t^{10}+49208448 t^9-1396347350 t^8-660856048 t^7+249605387 t^6+308765647 t^5+71309951 t^4-25317370 t^3-17950813 t^2-3661809 t-206066\right)+d^3 \left(-8 t^{36}+148 t^{35}-1076 t^{34}-1810 t^{33}+107092 t^{32}-943693 t^{31}+3961554 t^{30}-6546085 t^{29}-11672153 t^{28}+71193274 t^{27}-78545218 t^{26}-181352887 t^{25}+504820455 t^{24}+39480920 t^{23}-1310326107 t^{22}+732843520 t^{21}+2057744570 t^{20}-1917430015 t^{19}-2218549251 t^{18}+2642205466 t^{17}+1687581944 t^{16}-2342629925 t^{15}-743197585 t^{14}+1474059518 t^{13}-132892179 t^{12}-855045206 t^{11}+462412043 t^{10}+609941544 t^9-263340542 t^8-391532470 t^7+2422598 t^6+134672306 t^5+46474377 t^4-9377006 t^3-9716652 t^2-2531789 t-268300\right)+d^{22} \left(8 t^{36}+16 t^{35}+40 t^{34}-78 t^{33}-166 t^{32}+116 t^{31}+350 t^{30}-98 t^{29}-328 t^{28}-22 t^{27}+130 t^{26}+60 t^{25}+8 t^{24}\right)+d^{21} \left(136 t^{36}+136 t^{35}+370 t^{34}-1420 t^{33}-1046 t^{32}+3866 t^{31}+579 t^{30}-7365 t^{29}+4342 t^{28}+13906 t^{27}-6424 t^{26}-17176 t^{25}-706 t^{24}+9846 t^{23}+4840 t^{22}-673 t^{21}-1333 t^{20}-500 t^{19}-86 t^{18}-6 t^{17}\right)+d^{20} \left(1080 t^{36}+12 t^{35}+1148 t^{34}-10302 t^{33}+2576 t^{32}+37867 t^{31}-20511 t^{30}-59612 t^{29}+54051 t^{28}+25183 t^{27}-118568 t^{26}+110932 t^{25}+300532 t^{24}-108546 t^{23}-411884 t^{22}-108102 t^{21}+216863 t^{20}+173817 t^{19}+12977 t^{18}-43485 t^{17}-26340 t^{16}-7054 t^{15}-807 t^{14}+25 t^{13}+15 t^{12}+t^{11}\right)+d^{19} \left(5304 t^{36}-5100 t^{35}-4 t^{34}-35552 t^{33}+53454 t^{32}+185605 t^{31}-233934 t^{30}-330549 t^{29}+375369 t^{28}+238428 t^{27}-217819 t^{26}+440929 t^{25}-138101 t^{24}-1540276 t^{23}+867530 t^{22}+3567049 t^{21}+159084 t^{20}-4177209 t^{19}-2572423 t^{18}+1446419 t^{17}+2360348 t^{16}+800430 t^{15}-370930 t^{14}-455517 t^{13}-179808 t^{12}-19483 t^{11}+12977 t^{10}+7350 t^9+1926 t^8+297 t^7+26 t^6+t^5\right)+d^{18} \left(17952 t^{36}-34272 t^{35}-9456 t^{34}-28570 t^{33}+252132 t^{32}+446781 t^{31}-1330989 t^{30}-1002274 t^{29}+2989900 t^{28}+2116346 t^{27}-3366881 t^{26}-4499296 t^{25}-97440 t^{24}+6033058 t^{23}+8627446 t^{22}-217728 t^{21}-11963759 t^{20}-3614393 t^{19}+14435379 t^{18}+8766343 t^{17}-12610427 t^{16}-15799262 t^{15}-328876 t^{14}+9861151 t^{13}+6893005 t^{12}+433704 t^{11}-2153496 t^{10}-1518012 t^9-425006 t^8+49007 t^7+97681 t^6+46482 t^5+13437 t^4+2616 t^3+340 t^2+27 t+1\right)+d^{13} \left(38896 t^{36}-38896 t^{35}-1516788 t^{34}+7270050 t^{33}-7990094 t^{32}-25288516 t^{31}+75307226 t^{30}-7385178 t^{29}-207595623 t^{28}+187572351 t^{27}+320517735 t^{26}-494104788 t^{25}-400412388 t^{24}+878457214 t^{23}+658083579 t^{22}-1367035576 t^{21}-1179588597 t^{20}+1996995875 t^{19}+1802392141 t^{18}-2725711660 t^{17}-3020799273 t^{16}+2076904006 t^{15}+4036589117 t^{14}+1051039727 t^{13}-1137498491 t^{12}-554309503 t^{11}+362506508 t^{10}+337020197 t^9-13071172 t^8-136724079 t^7-81071556 t^6-18581926 t^5+2303120 t^4+2826429 t^3+846604 t^2+122898 t+7355\right)+d^{17} \left(44064 t^{36}-124032 t^{35}-27928 t^{34}+273990 t^{33}+496838 t^{32}+60532 t^{31}-4017255 t^{30}+123852 t^{29}+13489489 t^{28}+650691 t^{27}-27609186 t^{26}-9548625 t^{25}+41049392 t^{24}+30030207 t^{23}-45265998 t^{22}-54156098 t^{21}+33068026 t^{20}+80330400 t^{19}+27418831 t^{18}-38809220 t^{17}-43208701 t^{16}-6318180 t^{15}+13094650 t^{14}+1923844 t^{13}-8599497 t^{12}-2839309 t^{11}+5865178 t^{10}+6481358 t^9+2365544 t^8-501144 t^7-988016 t^6-549824 t^5-183986 t^4-40791 t^3-5942 t^2-521 t-21\right)+d^{16} \left(79968 t^{36}-291312 t^{35}-47824 t^{34}+1398030 t^{33}-207924 t^{32}-2932342 t^{31}-4472854 t^{30}+9782369 t^{29}+26073422 t^{28}-31145470 t^{27}-71107802 t^{26}+63371699 t^{25}+145457719 t^{24}-75974501 t^{23}-247780231 t^{22}+27920050 t^{21}+317462911 t^{20}+67959278 t^{19}-259865516 t^{18}-61296809 t^{17}+261819665 t^{16}+167407963 t^{15}-112142715 t^{14}-173746329 t^{13}-52248805 t^{12}+36667343 t^{11}+35359819 t^{10}+7610460 t^9-3270727 t^8-1032764 t^7+1598931 t^6+1558109 t^5+700377 t^4+191214 t^3+32709 t^2+3257 t+145\right)+d^{14} \left(95472 t^{36}-424320 t^{35}-500432 t^{34}+6168354 t^{33}-8441228 t^{32}-17293180 t^{31}+45742568 t^{30}+20866465 t^{29}-110435556 t^{28}-36880274 t^{27}+214269578 t^{26}+135668503 t^{25}-407446969 t^{24}-294010571 t^{23}+699518067 t^{22}+414227391 t^{21}-914245428 t^{20}-490698793 t^{19}+699525537 t^{18}+266219334 t^{17}-368928252 t^{16}+312987476 t^{15}+995557113 t^{14}+607159625 t^{13}-155589875 t^{12}-428234967 t^{11}-219443427 t^{10}+17434104 t^9+63878401 t^8+12415261 t^7-20040504 t^6-18287913 t^5-8056303 t^4-2221447 t^3-397427 t^2-43168 t-2192\right)+d^{15} \left(106080 t^{36}-456144 t^{35}-124896 t^{34}+3630882 t^{33}-3515958 t^{32}-9556662 t^{31}+9909376 t^{30}+25795524 t^{29}-3626240 t^{28}-88553299 t^{27}-17520775 t^{26}+236757342 t^{25}+57617905 t^{24}-423582526 t^{23}-154412735 t^{22}+531896916 t^{21}+313068811 t^{20}-535636840 t^{19}-534324941 t^{18}+412471295 t^{17}+830084323 t^{16}+213807109 t^{15}-331782787 t^{14}-204050103 t^{13}+48246671 t^{12}+34067126 t^{11}-58893937 t^{10}-56688844 t^9-8834052 t^8+13749313 t^7+10825500 t^6+3820637 t^5+673619 t^4+17532 t^3-16349 t^2-2942 t-165\right)-992

==> polynomials/Q_36,60.tex <==
-104 t^{60}+3576 t^{59}-56054 t^{58}+530653 t^{57}-3376929 t^{56}+15099955 t^{55}-47299744 t^{54}+94621123 t^{53}-60696618 t^{52}-320437416 t^{51}+1287976099 t^{50}-2178528207 t^{49}+273243876 t^{48}+7973281214 t^{47}-19318183045 t^{46}+12853221061 t^{45}+39986339023 t^{44}-113625066709 t^{43}+67166206650 t^{42}+219429050918 t^{41}-471128283103 t^{40}+36207929759 t^{39}+1022529869310 t^{38}-1073509368726 t^{37}-1033885837760 t^{36}+2731291126003 t^{35}-216631299912 t^{34}-4040875497616 t^{33}+2585296324286 t^{32}+3983361379473 t^{31}-4895049623560 t^{30}-2500490294041 t^{29}+5872989410539 t^{28}+558221441057 t^{27}-5183474679679 t^{26}+775354296291 t^{25}+3504304817909 t^{24}-1148417849264 t^{23}-1795764528947 t^{22}+901192937907 t^{21}+634964877248 t^{20}-520719584796 t^{19}-86855690493 t^{18}+255954194008 t^{17}-63142755326 t^{16}-119980455460 t^{15}+52419042752 t^{14}+53813384120 t^{13}-18861067632 t^{12}-20275946592 t^{11}+2807934112 t^{10}+5419601152 t^9+393040704 t^8-833863104 t^7-221588416 t^6+41820928 t^5+26209536 t^4+3117568 t^3-251904 t^2-75776 t+d^{17} \left(-31557012664 t^{60}+654862330416 t^{59}-4864431295564 t^{58}+10772703036149 t^{57}+47771294921796 t^{56}-286811317991056 t^{55}+92089881926742 t^{54}+2396834300022274 t^{53}-3755478903514269 t^{52}-11213405808179444 t^{51}+29537097648838927 t^{50}+33071931323603514 t^{49}-142686427165202074 t^{48}-56363601216973967 t^{47}+513940194084376511 t^{46}+5313825922087310 t^{45}-1513766534053181358 t^{44}+271232623044234626 t^{43}+3814831606853595348 t^{42}-785087157244311722 t^{41}-8281810435781640624 t^{40}+919777245433698792 t^{39}+15308267959018282983 t^{38}+820126918317979492 t^{37}-23758137963276208567 t^{36}-6100462082633277434 t^{35}+30436407246358196081 t^{34}+15045566287231421197 t^{33}-31215322864045370777 t^{32}-24757707064091955345 t^{31}+23931951112758067241 t^{30}+30037318283925247141 t^{29}-11237331340781619375 t^{28}-27332771409289394178 t^{27}-433839927175073604 t^{26}+18399254645834377630 t^{25}+6123152960390157275 t^{24}-8746191883508301679 t^{23}-6028186397654824245 t^{22}+2496191641754773502 t^{21}+3560738092298159903 t^{20}+17015600318503669 t^{19}-1417816237526306567 t^{18}-444922306232350933 t^{17}+344327882520854019 t^{16}+246691377640293629 t^{15}-20528012778555135 t^{14}-70041743829385835 t^{13}-17109614280520420 t^{12}+9253665230725018 t^{11}+6012044024875299 t^{10}+335515428640164 t^9-741794834219300 t^8-257953746684894 t^7-27626695300 t^6+20621084147032 t^5+5333773893283 t^4+352957632126 t^3-75164969726 t^2-15603328152 t-855178509\right)+d^{18} \left(-25494992680 t^{60}+418769941864 t^{59}-2001692090206 t^{58}-3347399926556 t^{57}+58405873133597 t^{56}-115178714497427 t^{55}-463426381632243 t^{54}+1852208312530117 t^{53}+1495079270195778 t^{52}-13866198093749176 t^{51}+910071152389497 t^{50}+68860609726986818 t^{49}-31212236359520125 t^{48}-256761040841963427 t^{47}+167822096927665824 t^{46}+770143161671608866 t^{45}-587726296989986983 t^{44}-1968312447997716656 t^{43}+1558602595390009925 t^{42}+4492109657936282184 t^{41}-3148071905002830594 t^{40}-9234170137324234813 t^{39}+4540883587590547224 t^{38}+16627393120956848488 t^{37}-3696045101287553905 t^{36}-25319985576011558930 t^{35}-1561336124320299116 t^{34}+31584287820617043728 t^{33}+11161962844265254304 t^{32}-31044539037504620168 t^{31}-21342004107246563612 t^{30}+22182895699026827461 t^{29}+26312817626477446981 t^{28}-8801829620823319044 t^{27}-22941305332460089342 t^{26}-2115861230520864541 t^{25}+14003226008694682510 t^{24}+6298946277169170946 t^{23}-5432166175741656352 t^{22}-5115981716587776536 t^{21}+752116250642115018 t^{20}+2475827794668835649 t^{19}+550720007603256584 t^{18}-726340872220431135 t^{17}-435697147876862486 t^{16}+77646705170703987 t^{15}+150239974153305739 t^{14}+30916742939277310 t^{13}-24447635742431883 t^{12}-14562567597085168 t^{11}-301084487486024 t^{10}+2250928163329458 t^9+758748281782371 t^8-31170108539027 t^7-84009851855956 t^6-21640771314244 t^5-727446256596 t^4+752514196296 t^3+172145506094 t^2+15293454189 t+449614796\right)+d^{16} \left(-22441109928 t^{60}+566430831632 t^{59}-5400660305244 t^{58}+21821354328833 t^{57}-4500646996031 t^{56}-268407523023459 t^{55}+702074535637471 t^{54}+913432580410172 t^{53}-6396246801701635 t^{52}+2646164770251866 t^{51}+31393325921186993 t^{50}-41653577768331377 t^{49}-103372670826693446 t^{48}+233046244873764319 t^{47}+253257203864777296 t^{46}-884630449703205187 t^{45}-517793471430068528 t^{44}+2585698980555696868 t^{43}+1045626507457040370 t^{42}-6085036192246408605 t^{41}-2319294311838860208 t^{40}+11761237486491740496 t^{39}+5253427333008196060 t^{38}-18827258733841004212 t^{37}-10805949082474993810 t^{36}+24834331578573683930 t^{35}+18918963858763064667 t^{34}-26309648958733804393 t^{33}-27323105265293362863 t^{32}+21017525735131641276 t^{31}+31817273769873298084 t^{30}-10611908364279670346 t^{29}-29305911115213899111 t^{28}+260539066386735899 t^{27}+20965465410500195188 t^{26}+5493795318863308672 t^{25}-11383122239620731697 t^{24}-6157329047068377982 t^{23}+4427742081881772004 t^{22}+4223115367396133032 t^{21}-934059484158636188 t^{20}-2078743503502108413 t^{19}-194166035098544122 t^{18}+719159156552735727 t^{17}+270537847577331444 t^{16}-147667877262339603 t^{15}-119761130014334709 t^{14}+3587665554926999 t^{13}+28991333084729720 t^{12}+7635761821479771 t^{11}-3178490635910406 t^{10}-2154429367093441 t^9-161496294435526 t^8+213798063508485 t^7+74057877050525 t^6+2067489841612 t^5-4111309320174 t^4-1028327009717 t^3-84352156607 t^2+2400285263 t+559284938\right)+d^{19} \left(-6789973104 t^{60}+11848435952 t^{59}+1049177754310 t^{58}-9504511559138 t^{57}+23238419833503 t^{56}+72883442010016 t^{55}-461263430003663 t^{54}+106254255732392 t^{53}+3714858746371533 t^{52}-4525533282080449 t^{51}-19526286792931648 t^{50}+34502725973556468 t^{49}+79266319200559507 t^{48}-160232019548726868 t^{47}-268701929820079902 t^{46}+536871328699347919 t^{45}+778493912345047900 t^{44}-1403881394713252463 t^{43}-1953738095564391583 t^{42}+3011676428330448657 t^{41}+4382113271653015193 t^{40}-5316691386939450313 t^{39}-8899739474369654409 t^{38}+7290507070678181700 t^{37}+15885103619207657086 t^{36}-6626593487159941932 t^{35}-23822444834539564735 t^{34}+1125693829379480756 t^{33}+28770162087468044763 t^{32}+8576023545527220473 t^{31}-26647693709329875149 t^{30}-17961106129947173977 t^{29}+17062758674619910966 t^{28}+21437807643863878857 t^{27}-4779989699458040001 t^{26}-17176223468770641458 t^{25}-3673603656154221871 t^{24}+9003600286340587420 t^{23}+5644858952408197773 t^{22}-2433163821394212729 t^{21}-3643145398885334305 t^{20}-338840831901902612 t^{19}+1343546634320314948 t^{18}+633383798702759238 t^{17}-221827935105727772 t^{16}-280409602770095021 t^{15}-40214605019397231 t^{14}+57634591243883428 t^{13}+30172904693839227 t^{12}-1187990952154425 t^{11}-5961558606262205 t^{10}-1865915244561923 t^9+199543726679787 t^8+285552765622753 t^7+70655314343658 t^6-1167793092299 t^5-4561542406405 t^4-1098232300521 t^3-110845687739 t^2-2608151081 t+232673008\right)+d^{15} \left(-5942554800 t^{60}+236849326632 t^{59}-3196259567198 t^{58}+19985570889055 t^{57}-51318587896526 t^{56}-65151057633907 t^{55}+739605835551194 t^{54}-1197554391232815 t^{53}-3228105568160609 t^{52}+13091140215457008 t^{51}+1462147098024739 t^{50}-69942078046629913 t^{49}+53565904726038133 t^{48}+258265793354655163 t^{47}-334850644347333934 t^{46}-750573489593661411 t^{45}+1225344545672207574 t^{44}+1844948170871042288 t^{43}-3268267133270742027 t^{42}-3987980217489610586 t^{41}+6837725269131082814 t^{40}+7715964404895533093 t^{39}-11567397470285173697 t^{38}-13394306198988096665 t^{37}+15871712603316883748 t^{36}+20598281026180161320 t^{35}-17245626450754971979 t^{34}-27385020412578156710 t^{33}+13894668292210115627 t^{32}+30603316016703047176 t^{31}-6766786482811452116 t^{30}-28100533458051923307 t^{29}-590753092896847435 t^{28}+20900268620088933041 t^{27}+4900551419951435376 t^{26}-12503776052242534782 t^{25}-5613800579284612509 t^{24}+5919287830922310747 t^{23}+4266333251413478952 t^{22}-2031392913195583310 t^{21}-2468882830144278025 t^{20}+304924065725719599 t^{19}+1078688675879105983 t^{18}+158741463919803106 t^{17}-329968856630379637 t^{16}-136138732839884098 t^{15}+58663451041189243 t^{14}+50997471414206142 t^{13}-144173575022506 t^{12}-10776991233645130 t^{11}-2877911044626116 t^{10}+994184214975785 t^9+673741938784152 t^8+56574379971615 t^7-53525334139792 t^6-17993713825617 t^5-905639468902 t^4+614946290125 t^3+141436490395 t^2+10859812011 t+151010431\right)+d^{25} \left(-4918325424 t^{60}+61147871308 t^{59}-131509412112 t^{58}-1014336471587 t^{57}+3802084071867 t^{56}+7942085518929 t^{55}-41923797769909 t^{54}-38712306257172 t^{53}+289116846994690 t^{52}+117728056691897 t^{51}-1498107043874641 t^{50}-155957389046685 t^{49}+6616630796451373 t^{48}+271174402895994 t^{47}-25628930698658269 t^{46}-7159809966078586 t^{45}+79093775077149180 t^{44}+54136874351386503 t^{43}-174251408388720206 t^{42}-202671308582919670 t^{41}+264639120621692047 t^{40}+495612756802372498 t^{39}-256770959943604652 t^{38}-934010328650639644 t^{37}-6654010524661542 t^{36}+1389409459820987727 t^{35}+685369758056022555 t^{34}-1475590866455364672 t^{33}-1603673608433904846 t^{32}+844523178869261515 t^{31}+2170889438411763529 t^{30}+327815676690866067 t^{29}-1864082971312350883 t^{28}-1324032667182983457 t^{27}+795725973423079520 t^{26}+1471371215271331856 t^{25}+264291256352190763 t^{24}-837783658776258937 t^{23}-647524290914007126 t^{22}+113541975485165807 t^{21}+414748183318598781 t^{20}+183163995180694151 t^{19}-84657281326441794 t^{18}-125690289400549184 t^{17}-39163668716897103 t^{16}+21653767102776854 t^{15}+24260452416889106 t^{14}+7064840026857913 t^{13}-2345343054153502 t^{12}-2783150293472878 t^{11}-939999741333523 t^{10}+13936376737003 t^9+141996041181764 t^8+61497777540934 t^7+11909350247938 t^6-43041423485 t^5-660458658827 t^4-185890669759 t^3-26879896664 t^2-2114849993 t-71788902\right)+d^{26} \left(-3621781064 t^{60}+31358592336 t^{59}+24755450998 t^{58}-788455877705 t^{57}+451728787394 t^{56}+9695712421123 t^{55}-7562074289605 t^{54}-78087871782308 t^{53}+49116214658466 t^{52}+450401607144420 t^{51}-170856665611315 t^{50}-1929461131359799 t^{49}+380585562007458 t^{48}+6595623216165475 t^{47}-805011078896542 t^{46}-20583352774555370 t^{45}-770818229600658 t^{44}+59622647639323854 t^{43}+26058563281584246 t^{42}-132872136646841197 t^{41}-127420558853815946 t^{40}+193302796083254400 t^{39}+331351537349272670 t^{38}-147169237613517412 t^{37}-585232629047761289 t^{36}-82852373146469433 t^{35}+761404477153215831 t^{34}+510646226206049566 t^{33}-652555782820868613 t^{32}-949558780130890439 t^{31}+162391809962366868 t^{30}+1047998669222219662 t^{29}+453196255361629962 t^{28}-661967409196334801 t^{27}-765157184470011273 t^{26}+59947539116213060 t^{25}+591192213039668030 t^{24}+314088453021755338 t^{23}-184481638693417979 t^{22}-296064226528398413 t^{21}-78061603240202360 t^{20}+102747672838645616 t^{19}+98579835162417405 t^{18}+15233772686123253 t^{17}-29599667140331316 t^{16}-22989516297892062 t^{15}-3903616645376497 t^{14}+4405002002103138 t^{13}+3478171974895845 t^{12}+898947511164481 t^{11}-216558460604678 t^{10}-265998171093352 t^9-98988653037723 t^8-13784885001860 t^7+3698401043513 t^6+2520127752992 t^5+686072371703 t^4+111127132443 t^3+10852896464 t^2+560464970 t+9745926\right)+d^{24} \left(-2163680496 t^{60}+54148859448 t^{59}-346294407430 t^{58}+108977640545 t^{57}+5729930543098 t^{56}-12332851723058 t^{55}-43315601271398 t^{54}+156832971137354 t^{53}+209936916074637 t^{52}-1192595449212386 t^{51}-875816124757393 t^{50}+6571589736349340 t^{49}+4406250157029566 t^{48}-27044066158914051 t^{47}-23411255545222887 t^{46}+81263715635099558 t^{45}+96070665677839759 t^{44}-177114933032385974 t^{43}-284558063926030568 t^{42}+293099779609412009 t^{41}+669093124759792019 t^{40}-349615901232152227 t^{39}-1346842626298750153 t^{38}+84437798054843320 t^{37}+2213974700868324993 t^{36}+857162479157100533 t^{35}-2710478430727528748 t^{34}-2409727997328529375 t^{33}+2140918968392694164 t^{32}+3813226455599931204 t^{31}-369784405608548346 t^{30}-4009189218759699631 t^{29}-1736645078963487908 t^{28}+2602581886219923828 t^{27}+2809977529631644915 t^{26}-482640208308570218 t^{25}-2270112810866564054 t^{24}-918968686780943632 t^{23}+899501346702190055 t^{22}+1022226917538746310 t^{21}+85982874553420998 t^{20}-453093498732110386 t^{19}-287588843094981789 t^{18}+29280760775667678 t^{17}+123296793005331293 t^{16}+55562299566448174 t^{15}-8732765860101288 t^{14}-19743651851547647 t^{13}-7731812257764971 t^{12}+527561874516284 t^{11}+1730404698760547 t^{10}+707904044860208 t^9+67539695384170 t^8-55781037560138 t^7-28921261464425 t^6-6530960188637 t^5-579584767153 t^4+74156218099 t^3+27902387173 t^2+3276168215 t+148179087\right)+d^{27} \left(-1413979936 t^{60}+6674514572 t^{59}+48433441040 t^{58}-247724544705 t^{57}-698877751804 t^{56}+3726885438759 t^{55}+7171899942362 t^{54}-32868683225941 t^{53}-60748522359738 t^{52}+186803156672935 t^{51}+403733747286512 t^{50}-675431627045040 t^{49}-1934711933940367 t^{48}+1427420582668737 t^{47}+6518323186152710 t^{46}-1426337859919254 t^{45}-16864652527492200 t^{44}-1075700673591638 t^{43}+39807081537048740 t^{42}+16163530893191681 t^{41}-81942579417463960 t^{40}-76260045506363056 t^{39}+112264545708952883 t^{38}+198443257610502951 t^{37}-59442866696682267 t^{36}-323638892757993057 t^{35}-106103682084229338 t^{34}+351556589204115908 t^{33}+330195777375105465 t^{32}-206775896216774826 t^{31}-476970568368963693 t^{30}-79903570908567298 t^{29}+401612944261621087 t^{28}+317609567146448811 t^{27}-136926462658851593 t^{26}-332052649560321232 t^{25}-107281747334462255 t^{24}+159431316244565125 t^{23}+168806508326828972 t^{22}+11812211858070682 t^{21}-85781730873522608 t^{20}-60139452261897091 t^{19}+2867230919248254 t^{18}+28171127970201958 t^{17}+16519428742706809 t^{16}-30893024790614 t^{15}-5493402331203013 t^{14}-3318031323224889 t^{13}-511094981349103 t^{12}+481956447671912 t^{11}+375088006143833 t^{10}+117774635384743 t^9+4780148409845 t^8-12289308203512 t^7-6109990083069 t^6-1615285111481 t^5-259574722369 t^4-22080314384 t^3-34845599 t^2+175149168 t+11714264\right)+d^{28} \left(-66407608 t^{60}-2452963736 t^{59}+18462305952 t^{58}+27878395967 t^{57}-389722809302 t^{56}-83846974821 t^{55}+4470381551884 t^{54}-60302255043 t^{53}-36219949906314 t^{52}-8117328282180 t^{51}+215904373413057 t^{50}+155747734047013 t^{49}-886004422297780 t^{48}-1201489256116474 t^{47}+2214002240260843 t^{46}+5073870534755552 t^{45}-2571364688320007 t^{44}-13315353656021144 t^{43}-1387837044247625 t^{42}+25868921756527725 t^{41}+13669049403363775 t^{40}-42849861848343955 t^{39}-46132390968922491 t^{38}+49683259002672922 t^{37}+105487120689261812 t^{36}-8615463110368406 t^{35}-152377002928718951 t^{34}-86285319495653992 t^{33}+127783430305825143 t^{32}+177120195870804145 t^{31}-23979671618464229 t^{30}-192129473919563960 t^{29}-100083460134289872 t^{28}+105803972135470545 t^{27}+152017006338608245 t^{26}+16682856196960179 t^{25}-100098215692197470 t^{24}-76904032461143428 t^{23}+13733498272711951 t^{22}+55137130508163311 t^{21}+28670311548152742 t^{20}-9728978020168445 t^{19}-20185884686959804 t^{18}-8899821029951793 t^{17}+2463827134454175 t^{16}+4950519138828044 t^{15}+2359588260684182 t^{14}-15272916673162 t^{13}-656103861510639 t^{12}-397289864801204 t^{11}-96917673802712 t^{10}+16927593531517 t^9+24180246268365 t^8+10350186927140 t^7+2532150333081 t^6+314795395121 t^5-13944518537 t^4-13854708105 t^3-2681646953 t^2-256820817 t-10501243\right)+d^7 \left(-36596432 t^{60}-847751268 t^{59}+37555395052 t^{58}-490836789256 t^{57}+3308632964301 t^{56}-12331621607477 t^{55}+19674314194117 t^{54}+30964177882407 t^{53}-210915806220217 t^{52}+312135865408644 t^{51}+376654101046626 t^{50}-1914306136412934 t^{49}+1517812662505067 t^{48}+4145301999079875 t^{47}-9478063377384095 t^{46}-496275190656173 t^{45}+23642937053618712 t^{44}-21256901231760313 t^{43}-31013465462800271 t^{42}+67399472877316814 t^{41}+6431266252073386 t^{40}-123199455341930053 t^{39}+67724444376142886 t^{38}+154687121834574290 t^{37}-178217915074623075 t^{36}-133050130639344817 t^{35}+280923575010115544 t^{34}+59476428686024995 t^{33}-330006063371502811 t^{32}+34693693346599164 t^{31}+310703970819028488 t^{30}-110464904925190347 t^{29}-245465131287774313 t^{28}+143698522468077787 t^{27}+170658165854245399 t^{26}-133064077689817938 t^{25}-109586843633412771 t^{24}+95291743680607451 t^{23}+66078900469361251 t^{22}-53461140100358851 t^{21}-36043420067421778 t^{20}+23546524952531361 t^{19}+16874554568650978 t^{18}-8247787312110157 t^{17}-6683608061180725 t^{16}+2294624658385937 t^{15}+2286851111202934 t^{14}-436268243354033 t^{13}-661794960371327 t^{12}+10337007203890 t^{11}+142899947597818 t^{10}+23499367378941 t^9-18301059508589 t^8-6695257420296 t^7+694109154318 t^6+722649427398 t^5+90559605856 t^4-18692748880 t^3-5817992448 t^2-430994720 t+210688\right)+d^6 \left(-29401832 t^{60}+392149516 t^{59}+1924527444 t^{58}-75749436141 t^{57}+701834183905 t^{56}-3342423303479 t^{55}+8173051383223 t^{54}-2696904736791 t^{53}-45201813117636 t^{52}+126687863072062 t^{51}-59760741215632 t^{50}-405233849316968 t^{49}+901059486357232 t^{48}-57681909736955 t^{47}-2589536003881731 t^{46}+3503898370929724 t^{45}+2325891078487450 t^{44}-10831473378936458 t^{43}+6053954406118832 t^{42}+16745675068718991 t^{41}-26464397758710276 t^{40}-9831634750372910 t^{39}+52643227422990665 t^{38}-18111434133388081 t^{37}-68439207228782861 t^{36}+61495362534560245 t^{35}+59699495041015107 t^{34}-102061005543033838 t^{33}-26982534044709223 t^{32}+122302646684047670 t^{31}-13830169473658728 t^{30}-117532535201240018 t^{29}+43324833726840719 t^{28}+95555368011736417 t^{27}-51608544722399858 t^{26}-67707872381446273 t^{25}+42349920436123802 t^{24}+42064411502964603 t^{23}-26617257779360273 t^{22}-22627184542143533 t^{21}+13508438585475771 t^{20}+10469852614859370 t^{19}-5790236459050120 t^{18}-4289689746370119 t^{17}+2107005391775480 t^{16}+1629864721936228 t^{15}-588092370160847 t^{14}-557803831306695 t^{13}+91811106447311 t^{12}+150380346109166 t^{11}+5235641578305 t^{10}-26852981951133 t^9-5749174437695 t^8+2467741708469 t^7+1087030581489 t^6-13217378324 t^5-76127042640 t^4-12939415296 t^3+266851776 t^2+232435136 t+14268160\right)+d^5 \left(-10635152 t^{60}+231228916 t^{59}-1714471606 t^{58}+648793908 t^{57}+73990776367 t^{56}-560067498666 t^{55}+1998692789748 t^{54}-3076981716490 t^{53}-3592376455685 t^{52}+26797712848000 t^{51}-45972637286598 t^{50}-15516493912679 t^{49}+201579634952078 t^{48}-299622919758700 t^{47}-145732396009681 t^{46}+1085038805410687 t^{45}-1103950497858671 t^{44}-1343329571870871 t^{43}+4183111237226906 t^{42}-1456891914087680 t^{41}-7262211274238147 t^{40}+9150019907356869 t^{39}+5798196685141064 t^{38}-19507178008614918 t^{37}+3812964329825395 t^{36}+26295472967325144 t^{35}-19850312617956837 t^{34}-24201373079317594 t^{33}+35416073464827988 t^{32}+13793938961605424 t^{31}-43449775614453320 t^{30}-1081494633972022 t^{29}+41521142850993842 t^{28}-7668178537899638 t^{27}-32357946428911599 t^{26}+10309956182627299 t^{25}+20960688003352597 t^{24}-8725233080686904 t^{23}-11431369778752395 t^{22}+5802616892886684 t^{21}+5410640818318211 t^{20}-3236065154195905 t^{19}-2373029234883753 t^{18}+1487268970418559 t^{17}+1016202286765960 t^{16}-516383305743675 t^{15}-400904174156087 t^{14}+114341693008907 t^{13}+126491570468059 t^{12}-8277198974597 t^{11}-27862239742995 t^{10}-3188019163458 t^9+3737474292024 t^8+1052757074068 t^7-221704126372 t^6-129582529064 t^5-6730557792 t^4+5406059488 t^3+1051148288 t^2+37525632 t-3217664\right)+d^4 \left(-2540544 t^{60}+66134432 t^{59}-714896586 t^{58}+3890304267 t^{57}-8064711401 t^{56}-28845909615 t^{55}+258639939158 t^{54}-799950881936 t^{53}+886586866283 t^{52}+2077751011868 t^{51}-9826785128516 t^{50}+13694940899043 t^{49}+10419372590500 t^{48}-71058776766097 t^{47}+91995173927610 t^{46}+73933694412286 t^{45}-380724794451901 t^{44}+316387832498809 t^{43}+568688853242160 t^{42}-1373881502395929 t^{41}+171771676719685 t^{40}+2589042638545688 t^{39}-2520185089639734 t^{38}-2526103239341990 t^{37}+5893656964534169 t^{36}-9525816643212 t^{35}-8401371203050857 t^{34}+4513582239882325 t^{33}+8345986947526837 t^{32}-8822232438802076 t^{31}-5727501749587289 t^{30}+10793977428001849 t^{29}+2117073832515934 t^{28}-9896799563003951 t^{27}+758689120384964 t^{26}+7252980330502863 t^{25}-2127240210385911 t^{24}-4448036679844156 t^{23}+2190607645494613 t^{22}+2417334163853275 t^{21}-1567652767448255 t^{20}-1238923874021251 t^{19}+835711282573852 t^{18}+604406560829852 t^{17}-322730232551932 t^{16}-260113281944970 t^{15}+81727733592053 t^{14}+88693941291988 t^{13}-9547773761258 t^{12}-21877687667502 t^{11}-1290724140934 t^{10}+3604682649192 t^9+727478950476 t^8-348385493908 t^7-129946955684 t^6+10474605616 t^5+10681165280 t^4+1216817088 t^3-148168704 t^2-34759168 t-1332992\right)+d^3 \left(-421808 t^{60}+12192280 t^{59}-154178562 t^{58}+1105564220 t^{57}-4770274781 t^{56}+11094130330 t^{55}-617981867 t^{54}-89418058365 t^{53}+303744841881 t^{52}-375287267286 t^{51}-582999292545 t^{50}+3190177868385 t^{49}-4582327907036 t^{48}-3220899178282 t^{47}+22299265951301 t^{46}-26623695123375 t^{45}-26694515107650 t^{44}+110628908946091 t^{43}-72236509805104 t^{42}-176371261302679 t^{41}+347253424129269 t^{40}+13251492429979 t^{39}-670968313787502 t^{38}+547790367067468 t^{37}+687050466631547 t^{36}-1352989097961284 t^{35}-109684848252583 t^{34}+1924093146108899 t^{33}-926317790227284 t^{32}-1844982606716281 t^{31}+1906811378596211 t^{30}+1138234875353051 t^{29}-2361700629962815 t^{28}-227147358306394 t^{27}+2207194377724674 t^{26}-430966687577834 t^{25}-1693996150619988 t^{24}+648706327293503 t^{23}+1123249320312559 t^{22}-530658787123259 t^{21}-659462505510857 t^{20}+299173253847000 t^{19}+338966375258193 t^{18}-117670436223297 t^{17}-146000157144189 t^{16}+29426280737307 t^{15}+49757291202420 t^{14}-2933079748863 t^{13}-12717575466462 t^{12}-793586692840 t^{11}+2341261229992 t^{10}+386981821120 t^9-300372321872 t^8-81617636384 t^7+23967447424 t^6+10664425248 t^5-340266496 t^4-663706624 t^3-87720960 t^2+1777408 t+675840\right)+d^2 \left(-47352 t^{60}+1472456 t^{59}-20482106 t^{58}+167584468 t^{57}-885279077 t^{56}+3052540388 t^{55}-6082394591 t^{54}+1055965572 t^{53}+35286233319 t^{52}-112854124690 t^{51}+129191190764 t^{50}+196941663147 t^{49}-978503717151 t^{48}+1255575413398 t^{47}+1048345594171 t^{46}-5825546862691 t^{45}+6187920386560 t^{44}+6832388480909 t^{43}-25260112337619 t^{42}+16092192208318 t^{41}+37737318522648 t^{40}-76485230993450 t^{39}+3292231431058 t^{38}+142373064519290 t^{37}-130922701552308 t^{36}-135751625359508 t^{35}+307306685455106 t^{34}-352724864727 t^{33}-431243109841290 t^{32}+232000142820903 t^{31}+422675349427221 t^{30}-448503733629761 t^{29}-294502379629090 t^{28}+549798962340830 t^{27}+133798465099636 t^{26}-513884020507799 t^{25}-22031644163502 t^{24}+389384066855039 t^{23}-18923545798830 t^{22}-244514252496380 t^{21}+16288265948606 t^{20}+126993217985473 t^{19}-4369267318785 t^{18}-53460262384655 t^{17}-1348690300965 t^{16}+17677985935139 t^{15}+1600604339060 t^{14}-4457664317878 t^{13}-637913378556 t^{12}+856853562608 t^{11}+146544478560 t^{10}-134180569488 t^9-25369966736 t^8+17831173296 t^7+4604618224 t^6-1368177088 t^5-581549824 t^4-18266368 t^3+14274048 t^2+1162752 t-67584\right)+d \left(-3256 t^{60}+107064 t^{59}-1593608 t^{58}+14190486 t^{57}-83771470 t^{56}+339339001 t^{55}-913514425 t^{54}+1290446480 t^{53}+1104956562 t^{52}-10677597195 t^{51}+25205842799 t^{50}-17954935384 t^{49}-60266213274 t^{48}+201047400681 t^{47}-201888039320 t^{46}-271775921347 t^{45}+1108066726984 t^{44}-1056340788638 t^{43}-1419629500220 t^{42}+4789683056345 t^{41}-2787394531558 t^{40}-7787709672846 t^{39}+14532368145477 t^{38}+1635877247676 t^{37}-29131127975308 t^{36}+20199197108331 t^{35}+33859324661805 t^{34}-52628269428192 t^{33}-18820317968954 t^{32}+79634901734351 t^{31}-11717508246266 t^{30}-87182423636496 t^{29}+41368349157516 t^{28}+74401867695765 t^{27}-55225062463015 t^{26}-51667126474640 t^{25}+50413875189217 t^{24}+30243568683979 t^{23}-34833875009941 t^{22}-15341889890629 t^{21}+18668387630852 t^{20}+6735603949684 t^{19}-7713349055215 t^{18}-2396779723174 t^{17}+2415228969693 t^{16}+570228535712 t^{15}-584510048112 t^{14}-27596734756 t^{13}+133842099496 t^{12}-35920917136 t^{11}-39230836976 t^{10}+11808000224 t^9+11192856320 t^8-729998528 t^7-1910213952 t^6-269862528 t^5+122244352 t^4+39989504 t^3+1910784 t^2-547840 t-53248\right)+d^{36} \left(3584 t^{60}+22400 t^{59}-39872 t^{58}-645512 t^{57}-1010296 t^{56}+6348692 t^{55}+24809392 t^{54}-8323358 t^{53}-209679906 t^{52}-325548611 t^{51}+664005160 t^{50}+2813800985 t^{49}+1573887395 t^{48}-9061790298 t^{47}-20027171690 t^{46}-403612601 t^{45}+60132363883 t^{44}+89597573846 t^{43}-22360231561 t^{42}-238617398188 t^{41}-283899888268 t^{40}+79277475879 t^{39}+617777959970 t^{38}+678965623950 t^{37}-78443671810 t^{36}-1071648818887 t^{35}-1227808568921 t^{34}-172817079206 t^{33}+1207926684251 t^{32}+1609335846170 t^{31}+653125030315 t^{30}-762378752079 t^{29}-1423620327259 t^{28}-943176898726 t^{27}+66314566075 t^{26}+742795203959 t^{25}+732085261624 t^{24}+290189851631 t^{23}-131959161001 t^{22}-288351255944 t^{21}-215079153064 t^{20}-71019762599 t^{19}+26979762337 t^{18}+53911898828 t^{17}+39099452643 t^{16}+16360633072 t^{15}+1900453106 t^{14}-3178111810 t^{13}-3227423288 t^{12}-1925412493 t^{11}-866606917 t^{10}-314395153 t^9-94142874 t^8-23420768 t^7-4823217 t^6-812260 t^5-109431 t^4-11377 t^3-859 t^2-42 t-1\right)+d^{35} \left(86016 t^{60}+398720 t^{59}-1777552 t^{58}-13718068 t^{57}-934856 t^{56}+179686884 t^{55}+356999508 t^{54}-958747433 t^{53}-4391727424 t^{52}-1087603169 t^{51}+23331406497 t^{50}+42286703795 t^{49}-38838322899 t^{48}-225972711853 t^{47}-193016215960 t^{46}+446345655650 t^{45}+1182618869026 t^{44}+449253942745 t^{43}-2216420093534 t^{42}-3872289101912 t^{41}-539187529087 t^{40}+6376169345161 t^{39}+8647785775563 t^{38}+435267391155 t^{37}-11762931682922 t^{36}-13789308925961 t^{35}-811494051381 t^{34}+14655762010202 t^{33}+16007495837614 t^{32}+1784603922318 t^{31}-12892441298055 t^{30}-13823403609234 t^{29}-2387528781118 t^{28}+8508331342823 t^{27}+9437169298635 t^{26}+2414376531677 t^{25}-4285463170626 t^{24}-5453578632494 t^{23}-2264384225684 t^{22}+1196361699688 t^{21}+2398431864828 t^{20}+1591362999911 t^{19}+279051453009 t^{18}-484658508887 t^{17}-569180101984 t^{16}-328119364305 t^{15}-88392026493 t^{14}+31336713240 t^{13}+54913614043 t^{12}+39143110229 t^{11}+19767530573 t^{10}+7844568367 t^9+2533373198 t^8+673410260 t^7+147171979 t^6+26162982 t^5+3704706 t^4+403341 t^3+31790 t^2+1618 t+40\right)+d^{34} \left(964096 t^{60}+2875712 t^{59}-26792456 t^{58}-119760542 t^{57}+218544626 t^{56}+1938604255 t^{55}+1003692614 t^{54}-15255781739 t^{53}-31514750321 t^{52}+48471465774 t^{51}+246050537655 t^{50}+123771608237 t^{49}-873381447358 t^{48}-1678123385265 t^{47}+681233715643 t^{46}+5971420622797 t^{45}+5803820231286 t^{44}-7401682781919 t^{43}-21809644217168 t^{42}-10655441456894 t^{41}+27807558373819 t^{40}+48087435330995 t^{39}+8010567184856 t^{38}-59367988707788 t^{37}-67633268751483 t^{36}+9118094200666 t^{35}+84626991518860 t^{34}+62504026336343 t^{33}-35187839393353 t^{32}-91359848105347 t^{31}-41399623481209 t^{30}+51296185856644 t^{29}+81705341369584 t^{28}+27103156076935 t^{27}-43060687594746 t^{26}-59487296523511 t^{25}-22067377390536 t^{24}+20586815022337 t^{23}+32094665764623 t^{22}+15830719245786 t^{21}-4133377323123 t^{20}-11807036217370 t^{19}-8027292186017 t^{18}-1332366626612 t^{17}+2401944111774 t^{16}+2618898136348 t^{15}+1327503164522 t^{14}+201043133890 t^{13}-271747425833 t^{12}-299223664864 t^{11}-183896725680 t^{10}-83193917771 t^9-29723866904 t^8-8590558100 t^7-2017866121 t^6-382341897 t^5-57335590 t^4-6576624 t^3-543765 t^2-28926 t-745\right)+d^{33} \left(6653632 t^{60}+8482528 t^{59}-215363012 t^{58}-514196507 t^{57}+2722297516 t^{56}+10521744477 t^{55}-12328576179 t^{54}-106303432522 t^{53}-61635932287 t^{52}+562216942829 t^{51}+1081802372742 t^{50}-1157904402140 t^{49}-5849084986138 t^{48}-3189975443179 t^{47}+14578481303358 t^{46}+26030027104030 t^{45}-7148543643062 t^{44}-66041148449925 t^{43}-53338513962074 t^{42}+68497135214031 t^{41}+150576968033141 t^{40}+23209688983984 t^{39}-196160173814201 t^{38}-176769565385222 t^{37}+133868182832519 t^{36}+326756157543900 t^{35}+68441167592787 t^{34}-359178853001083 t^{33}-378356449487396 t^{32}+87615120357668 t^{31}+479501130545190 t^{30}+331149595911466 t^{29}-154140804159693 t^{28}-415254122429899 t^{27}-226882218975225 t^{26}+123193064308493 t^{25}+262249778324356 t^{24}+131836911890211 t^{23}-59432473812804 t^{22}-128410174861806 t^{21}-71694314413519 t^{20}+9830693101893 t^{19}+44122339592229 t^{18}+31637740522392 t^{17}+6622158866625 t^{16}-7426595227323 t^{15}-8468267103950 t^{14}-4188933144031 t^{13}-591699959379 t^{12}+802064003098 t^{11}+822922341588 t^{10}+469327604104 t^9+194959530068 t^8+63108998553 t^7+16250601365 t^6+3328414190 t^5+534160119 t^4+65075661 t^3+5680446 t^2+317443 t+8553\right)+d^{32} \left(31259072 t^{60}-16313144 t^{59}-1067967314 t^{58}-671328602 t^{57}+16163993762 t^{56}+27181707086 t^{55}-125737673009 t^{54}-372121451059 t^{53}+402096488625 t^{52}+2626235617818 t^{51}+1093016386968 t^{50}-10007932901418 t^{49}-15184621960974 t^{48}+16485088320251 t^{47}+60180619341663 t^{46}+15456552343339 t^{45}-121291384092307 t^{44}-126702063315240 t^{43}+134884814686199 t^{42}+302596319323479 t^{41}-64754056843191 t^{40}-562026346869351 t^{39}-225850788453315 t^{38}+820515751207802 t^{37}+1012658263607578 t^{36}-417915302735170 t^{35}-1784023010366798 t^{34}-993126157576957 t^{33}+1264714832186197 t^{32}+2130949705819489 t^{31}+446557143345708 t^{30}-1668710321905729 t^{29}-1704239115159709 t^{28}+101189544161748 t^{27}+1463195415930485 t^{26}+1065244327882571 t^{25}-231651593103062 t^{24}-916744653166713 t^{23}-575321033610577 t^{22}+100912770441598 t^{21}+404813696873672 t^{20}+262320269761278 t^{19}+2639684256817 t^{18}-120185748892803 t^{17}-94399886224245 t^{16}-24470416793623 t^{15}+16514740896376 t^{14}+21217926648180 t^{13}+11069840272103 t^{12}+2343531495373 t^{11}-1085028979336 t^{10}-1332171078444 t^9-740049008315 t^8-285922809489 t^7-83673049470 t^6-18957829656 t^5-3308419705 t^4-433101025 t^3-40264838 t^2-2379989 t-67445\right)+d^{31} \left(103430256 t^{60}-256865136 t^{59}-3381107262 t^{58}+4226063147 t^{57}+54817433256 t^{56}-4006745609 t^{55}-516569419504 t^{54}-463569275973 t^{53}+2831896385953 t^{52}+5198727495808 t^{51}-8017357599873 t^{50}-27322992628325 t^{49}+4372415839371 t^{48}+82599447495362 t^{47}+40218143584717 t^{46}-173434216317695 t^{45}-155320068246586 t^{44}+355010702095117 t^{43}+517694538098498 t^{42}-593561970977853 t^{41}-1628267228403524 t^{40}-35607633940441 t^{39}+3096146210338655 t^{38}+2711185364168566 t^{37}-2511498088585249 t^{36}-5860586046703553 t^{35}-1362076459665349 t^{34}+6002299049657018 t^{33}+5947916182329374 t^{32}-2155606391606791 t^{31}-7674765663127034 t^{30}-3483825651437371 t^{29}+4592818218512920 t^{28}+6524216065679842 t^{27}+1119698533302988 t^{26}-4226100415925156 t^{25}-4001869244378612 t^{24}-114849798901849 t^{23}+2484752284509534 t^{22}+1923882957916833 t^{21}+24538090810682 t^{20}-1006998413087346 t^{19}-765581109582534 t^{18}-105640716193130 t^{17}+249611008743422 t^{16}+226107319655058 t^{15}+74614942409733 t^{14}-21670595478966 t^{13}-38835903157918 t^{12}-22147942658187 t^{11}-6285880237658 t^{10}+318078322406 t^9+1313220666159 t^8+757481798164 t^7+275092292418 t^6+72208319618 t^5+14094763956 t^4+2020337935 t^3+202737104 t^2+12800780 t+384414\right)+d^8 \left(107163712 t^{60}-8893882888 t^{59}+187438146282 t^{58}-1891271014581 t^{57}+10568158232276 t^{56}-31155803581076 t^{55}+19806213209824 t^{54}+181935088861330 t^{53}-584808963957529 t^{52}+225714975709118 t^{51}+2358496227996557 t^{50}-4541928473178210 t^{49}-2514696607541830 t^{48}+17775017972056875 t^{47}-11448232399744411 t^{46}-36366408833925051 t^{45}+59294965941529665 t^{44}+33950919385756491 t^{43}-146799707990752299 t^{42}+35266336575510915 t^{41}+240101268973440191 t^{40}-202834133197708049 t^{39}-271373077359991002 t^{38}+446216667803301466 t^{37}+188163625964532291 t^{36}-685188131201111718 t^{35}-5197095519784769 t^{34}+825448145982412851 t^{33}-197987689077635626 t^{32}-815595903558377561 t^{31}+336232243842907674 t^{30}+675164527160910285 t^{29}-375036194367667157 t^{28}-476865663444797589 t^{27}+333404195163104131 t^{26}+297276763221440138 t^{25}-249562113713924516 t^{24}-173381118921479065 t^{23}+156564508883223988 t^{22}+98610693198350421 t^{21}-79088281216995564 t^{20}-52509270316060045 t^{19}+30621306699688598 t^{18}+23957949193015364 t^{17}-8677798421450855 t^{16}-8893269802319378 t^{15}+1621480063204834 t^{14}+2670795029456851 t^{13}-61151348405277 t^{12}-628063435599778 t^{11}-89374664727928 t^{10}+99339136047146 t^9+33114458562102 t^8-6717186699089 t^7-5022197165810 t^6-425257458178 t^5+256342988669 t^4+69202519506 t^3+3781950184 t^2-582227176 t-59625968\right)+d^{30} \left(235293368 t^{60}-1137880996 t^{59}-6247972388 t^{58}+25721164778 t^{57}+97049677020 t^{56}-248192874668 t^{55}-987658463680 t^{54}+1179294700525 t^{53}+6459065227345 t^{52}-2184320458953 t^{51}-27750315497425 t^{50}-1781224416707 t^{49}+92112590171702 t^{48}+15417074781564 t^{47}-314772026884450 t^{46}-148781357077013 t^{45}+985353741789960 t^{44}+1155694668293164 t^{43}-1751958641015842 t^{42}-4245170747744252 t^{41}+131861530835322 t^{40}+8074489333288277 t^{39}+6034727069078796 t^{38}-8018931779091090 t^{37}-14164607508787743 t^{36}+1469364943128675 t^{35}+19290680625269914 t^{34}+10790769797095646 t^{33}-15832738008348015 t^{32}-23255004389195437 t^{31}+474281062665188 t^{30}+23687898108623325 t^{29}+16624652019531190 t^{28}-8838769280521651 t^{27}-20000373570307800 t^{26}-7404641997838627 t^{25}+9329643272689418 t^{24}+11764053648877933 t^{23}+2404137234080738 t^{22}-5397378755028110 t^{21}-5234624580625725 t^{20}-901645654916219 t^{19}+1927598290166907 t^{18}+1783270199729859 t^{17}+448243139747794 t^{16}-381763780028047 t^{15}-431368166753088 t^{14}-178000868410953 t^{13}+3575290465082 t^{12}+49128465749256 t^{11}+31879513578041 t^{10}+10779081711766 t^9+1315009391668 t^8-695692893277 t^7-498207466980 t^6-173957121436 t^5-40522190045 t^4-6599675316 t^3-731933055 t^2-50174320 t-1615550\right)+d^{29} \left(308640872 t^{60}-2704682376 t^{59}-2698537066 t^{58}+60678483840 t^{57}+3458620160 t^{56}-667068805570 t^{55}+64488582657 t^{54}+4755338612599 t^{53}-1032303332861 t^{52}-26902675487766 t^{51}+8109862405670 t^{50}+141794945199586 t^{49}+1456847347449 t^{48}-635325677981926 t^{47}-424631816855250 t^{46}+1892555037189413 t^{45}+2788226590613377 t^{44}-2799270076392109 t^{43}-8631589914332732 t^{42}-435053584512323 t^{41}+15816919558182048 t^{40}+10406928173457386 t^{39}-19821765927573959 t^{38}-27265515710215458 t^{37}+14881846155969606 t^{36}+49024971986481258 t^{35}+10167754431299315 t^{34}-57756799008618365 t^{33}-51588343350282693 t^{32}+30487668335853822 t^{31}+75373833381630894 t^{30}+20727385260254322 t^{29}-56310025024496364 t^{28}-56174510679780384 t^{27}+8682962494205980 t^{26}+49814885820163892 t^{25}+27758008286893190 t^{24}-15166908803258403 t^{23}-28249599855518715 t^{22}-10250876193205596 t^{21}+8852861060359536 t^{20}+11447532526394590 t^{19}+3528540333861897 t^{18}-2760428832711546 t^{17}-3355768733266932 t^{16}-1220518577282619 t^{15}+352029639224870 t^{14}+623375555284162 t^{13}+311537917702254 t^{12}+44593974545487 t^{11}-40385663687325 t^{10}-32852621146436 t^9-12555379586192 t^8-2555082535009 t^7-3399777177 t^6+186565861217 t^5+68580110760 t^4+14120246991 t^3+1828725264 t^2+140678488 t+4963590\right)+d^9 \left(805000032 t^{60}-36160441556 t^{59}+604316135624 t^{58}-5192727624381 t^{57}+24535567182131 t^{56}-53335072035503 t^{55}-44321988460661 t^{54}+547315736095540 t^{53}-974577884555184 t^{52}-1189181418568975 t^{51}+6599029486663341 t^{50}-4066519747793321 t^{49}-19686381241038223 t^{48}+33959735201727907 t^{47}+27536971418640756 t^{46}-114072814981594551 t^{45}+15520678740170792 t^{44}+245524269405244362 t^{43}-177862439072414720 t^{42}-367840789025996242 t^{41}+497097707806511108 t^{40}+365369696334444896 t^{39}-923597808141602309 t^{38}-140983606697881054 t^{37}+1327559886369013932 t^{36}-290008891325621467 t^{35}-1576450336098979663 t^{34}+773023360605908933 t^{33}+1608632872402512879 t^{32}-1099138743233473307 t^{31}-1441532436447533293 t^{30}+1146640348701448909 t^{29}+1139581479140756626 t^{28}-955863051353808869 t^{27}-791177155664146081 t^{26}+668350729792325814 t^{25}+485389120033535166 t^{24}-405703493153987126 t^{23}-272471254585940428 t^{22}+213983384262939947 t^{21}+145594700728107586 t^{20}-92711265327711746 t^{19}-72062363739608741 t^{18}+29696566255838037 t^{17}+30163786810503313 t^{16}-5849637884568385 t^{15}-9928258370152805 t^{14}+146633920748901 t^{13}+2483357568683765 t^{12}+363810619933223 t^{11}-438968932817352 t^{10}-144948153790557 t^9+40467019225570 t^8+27434821944798 t^7+1235664476074 t^6-2160035346053 t^5-522471661343 t^4+3342499577 t^3+16317004488 t^2+2042645620 t+63133456\right)+d^{10} \left(2738396136 t^{60}-98801504192 t^{59}+1423243246346 t^{58}-10637890210993 t^{57}+41652227193316 t^{56}-51852280793371 t^{55}-237587713046743 t^{54}+1047592252404622 t^{53}-623757304468530 t^{52}-4927297233789232 t^{51}+10247300739578767 t^{50}+8754207133484797 t^{49}-48363844486955296 t^{48}+14033868257130659 t^{47}+136882476731337728 t^{46}-133358812993681574 t^{45}-262945180666528581 t^{44}+446102432572107876 t^{43}+340221547433649508 t^{42}-1000189755417105547 t^{41}-223999869721974371 t^{40}+1705612157383813610 t^{39}-201633796409121340 t^{38}-2334172691097106698 t^{37}+924308071288974541 t^{36}+2654676420905329895 t^{35}-1769486040841821485 t^{34}-2601595382667651736 t^{33}+2453833575631438863 t^{32}+2300420769626037043 t^{31}-2708824891866789459 t^{30}-1916508064327974508 t^{29}+2438034871094792767 t^{28}+1515826132175082276 t^{27}-1800264341809988702 t^{26}-1099356637285391336 t^{25}+1099499384361235526 t^{24}+703819021576444940 t^{23}-564701787782610322 t^{22}-396088166284163785 t^{21}+245328096022600535 t^{20}+199990234281164805 t^{19}-84807744973366695 t^{18}-89155074198783587 t^{17}+18894330735023450 t^{16}+32519776789882237 t^{15}-467553540742160 t^{14}-8927338031956771 t^{13}-1432426181654640 t^{12}+1707773835552584 t^{11}+595464947937014 t^{10}-184223619711161 t^9-127557878429353 t^8-2259008439456 t^7+13423731392667 t^6+3045802006034 t^5-271459333174 t^4-199885759123 t^3-26373627450 t^2-424686330 t+97321912\right)+d^{23} \left(6282930320 t^{60}-40844522004 t^{59}-256493313104 t^{58}+2591560133822 t^{57}-1527021990743 t^{56}-37353662367431 t^{55}+65333725528321 t^{54}+306970576205733 t^{53}-698639644655295 t^{52}-1868274821301476 t^{51}+4372904235917844 t^{50}+9335254053185916 t^{49}-18534695144429819 t^{48}-38313228646957980 t^{47}+56574747916174004 t^{46}+125837186442771483 t^{45}-134062465776300252 t^{44}-340788032278107828 t^{43}+263881042087494148 t^{42}+824699795151899051 t^{41}-370650694622872038 t^{40}-1779634531933913209 t^{39}+90026714672281920 t^{38}+3140986839316864381 t^{37}+1114870045376013296 t^{36}-4240830244487184861 t^{35}-3377377593839824837 t^{34}+4029531246463825590 t^{33}+5929857193856857274 t^{32}-1845661615369212507 t^{31}-7189335336273515034 t^{30}-1621679858908340505 t^{29}+5910971525244543486 t^{28}+4358175717444019736 t^{27}-2611146331995877766 t^{26}-4642676409181753787 t^{25}-548240141859828754 t^{24}+2766093722528617030 t^{23}+1777350294641158603 t^{22}-631965943266482300 t^{21}-1257840352276669065 t^{20}-354667460940250330 t^{19}+368253699855879565 t^{18}+331659301131576296 t^{17}+33890803764425744 t^{16}-92899685125054298 t^{15}-55706550256300229 t^{14}-1761993329314548 t^{13}+12602959666252068 t^{12}+6176025289584456 t^{11}+391564581543236 t^{10}-843355086283154 t^9-409585229853745 t^8-65282540533321 t^7+14728039186383 t^6+10256300644124 t^5+2494869763905 t^4+305526155612 t^3+11741410869 t^2-1378420852 t-133688022\right)+d^{11} \left(6358027712 t^{60}-198382884692 t^{59}+2512245599932 t^{58}-16189579382437 t^{57}+48926720626610 t^{56}+8340043369779 t^{55}-531116810815332 t^{54}+1233841567769595 t^{53}+1324644712327116 t^{52}-9512142858246847 t^{51}+5655891448314520 t^{50}+36696288927755312 t^{49}-56418119740390341 t^{48}-85238536478977594 t^{47}+236124379760602935 t^{46}+106305605901722088 t^{45}-665407407060966188 t^{44}+36390298391860305 t^{43}+1424630653557634109 t^{42}-526129635822055269 t^{41}-2447927612784859925 t^{40}+1453235932751924111 t^{39}+3474287094964466925 t^{38}-2684537869182943526 t^{37}-4134258922138754476 t^{36}+3897738164160932889 t^{35}+4168590891563711070 t^{34}-4766499281286868122 t^{33}-3638546217273671946 t^{32}+5091381188190113755 t^{31}+2899012903352764150 t^{30}-4786134299032763088 t^{29}-2284878717342687104 t^{28}+3884555912251177728 t^{27}+1835984209688647045 t^{26}-2637801889466232619 t^{25}-1402645154177126444 t^{24}+1457519003420893987 t^{23}+931640545950972903 t^{22}-644462489442822457 t^{21}-518079417551909395 t^{20}+222540358404629881 t^{19}+242467016570243254 t^{18}-51972091853574150 t^{17}-94392405797371917 t^{16}+1491957650757011 t^{15}+28524919919293070 t^{14}+4903245438368759 t^{13}-5995859352919526 t^{12}-2245394341388784 t^{11}+710152263620004 t^{10}+528717333119036 t^9+4353153586069 t^8-66859255138313 t^7-14971826893304 t^6+2547006140936 t^5+1541126087006 t^4+187953816151 t^3-12866025964 t^2-4475114541 t-254827824\right)+d^{14} \left(7470724744 t^{60}-107434672572 t^{59}+155129944340 t^{58}+6315720629176 t^{57}-52273997201154 t^{56}+144163000626986 t^{55}+169451417364834 t^{54}-1934060162145273 t^{53}+2555238605298889 t^{52}+9783149273113379 t^{51}-28292615852688633 t^{50}-24103804930939187 t^{49}+151802923655334150 t^{48}+6590133151401136 t^{47}-559571847536517062 t^{46}+183324986229321945 t^{45}+1588900792576938735 t^{44}-818345107789993394 t^{43}-3687226690078556104 t^{42}+2184472870986779616 t^{41}+7256151914507914767 t^{40}-4247800299108462018 t^{39}-12370983798224221994 t^{38}+6269364568096992334 t^{37}+18370857705008902557 t^{36}-6880948755135923845 t^{35}-23562029818230100382 t^{34}+5050159971286514097 t^{33}+25714504295935064664 t^{32}-1291451567092746983 t^{31}-23599458899991507615 t^{30}-2461224053400395422 t^{29}+18171889368528107448 t^{28}+4517905056290200359 t^{27}-11834727252277485490 t^{26}-4693082024990161289 t^{25}+6526670028973690716 t^{24}+3769219777842604997 t^{23}-2913248085907886216 t^{22}-2476994734983928289 t^{21}+898341332997206477 t^{20}+1290554794437811814 t^{19}-81553185886088005 t^{18}-504069631934024959 t^{17}-89050448407821346 t^{16}+138129527013285349 t^{15}+58717575148947381 t^{14}-21955811659636203 t^{13}-19332609463805629 t^{12}-169403316499856 t^{11}+3598407939049968 t^{10}+934102686398896 t^9-281464504738781 t^8-184156481685969 t^7-16292683711255 t^6+11375328670167 t^5+3666222149266 t^4+263018398834 t^3-56724420479 t^2-11475420104 t-567884394\right)+d^{12} \left(10713004264 t^{60}-293083356536 t^{59}+3227953522924 t^{58}-17117993169495 t^{57}+30680082879280 t^{56}+121911581376237 t^{55}-704844709690124 t^{54}+536987807641465 t^{53}+4313280117045276 t^{52}-9843230145958738 t^{51}-11703760212490351 t^{50}+58493230610000529 t^{49}+734266632276326 t^{48}-216918776795111680 t^{47}+122616488671648331 t^{46}+584602145162456883 t^{45}-569267179101073003 t^{44}-1233344963720663831 t^{43}+1627679653062919354 t^{42}+2141714552529754409 t^{41}-3476280341526634729 t^{40}-3182873915780231131 t^{39}+5918475337393648518 t^{38}+4156314775018161181 t^{37}-8290008038084156438 t^{36}-4807813518446954302 t^{35}+9767462599247538810 t^{34}+4892844410572252086 t^{33}-9914411147494907313 t^{32}-4374837197467011037 t^{31}+8910480458712779205 t^{30}+3558235015729478907 t^{29}-7221870436177397577 t^{28}-2842256329475665515 t^{27}+5214397547305029679 t^{26}+2309917103702878517 t^{25}-3203700744790852304 t^{24}-1769870119970594230 t^{23}+1574899614546784558 t^{22}+1150443070686149522 t^{21}-577876916523110540 t^{20}-601234383245087516 t^{19}+137070319205864512 t^{18}+250472894792580098 t^{17}-3724116870659149 t^{16}-81421881830500186 t^{15}-14735770947284520 t^{14}+18844130649306520 t^{13}+7514507220979272 t^{12}-2454670344035727 t^{11}-1971553772088291 t^{10}-18991813147029 t^9+285033679394996 t^8+65984849940779 t^7-15268982859000 t^6-9040835124844 t^5-955085831678 t^4+231313037561 t^3+69245666719 t^2+5777653579 t+84853751\right)+d^{13} \left(12538226280 t^{60}-291306580064 t^{59}+2598808196706 t^{58}-9100888361080 t^{57}-12566022213546 t^{56}+204399157836550 t^{55}-470165174925435 t^{54}-927391156165317 t^{53}+5583067028820761 t^{52}-1863148526441130 t^{51}-30617695566782830 t^{50}+38517037167583860 t^{49}+106408806303062833 t^{48}-216540408741369245 t^{47}-260663628497964107 t^{46}+779543808244326874 t^{45}+470143546599563019 t^{44}-2104671244143147524 t^{43}-634489293271480830 t^{42}+4563398046901087960 t^{41}+664649451647274244 t^{40}-8232673892939276898 t^{39}-674807947414197675 t^{38}+12560429856928202248 t^{37}+1024303204745861921 t^{36}-16277720394879051687 t^{35}-1964871425101175429 t^{34}+17921326455274557220 t^{33}+3199674660954815454 t^{32}-16832240284055997171 t^{31}-4046736005465252240 t^{30}+13673835290284285057 t^{29}+4137577486040016728 t^{28}-9796793223873607034 t^{27}-3690842856050349802 t^{26}+6201519139031217996 t^{25}+3012121558982364680 t^{24}-3324247169904495561 t^{23}-2180354310312672771 t^{22}+1374299287930652971 t^{21}+1299646357769213587 t^{20}-364994130804550824 t^{19}-603451188116570446 t^{18}+16125288113736724 t^{17}+212128541974621168 t^{16}+39375819075498866 t^{15}-53276868999533353 t^{14}-22261361411229483 t^{13}+7681136385758428 t^{12}+6547647331108761 t^{11}+76596052186502 t^{10}-1073311679860885 t^9-263774233626059 t^8+71005639461983 t^7+43963475568406 t^6+4144232745426 t^5-1940500083299 t^4-598941315688 t^3-51866877403 t^2+1735800914 t+365027941\right)+d^{20} \left(12667756240 t^{60}-298859095312 t^{59}+2370651954878 t^{58}-5799736761755 t^{57}-19060238455305 t^{56}+124374632424699 t^{55}-53034337574542 t^{54}-977142196725680 t^{53}+1648615867060525 t^{52}+4575291786230037 t^{51}-13430685630232094 t^{50}-15171351440572290 t^{49}+70806546323375103 t^{48}+43518705283899877 t^{47}-279278301479249902 t^{46}-138027561349205904 t^{45}+856505183884633672 t^{44}+471044311282723556 t^{43}-2077710159409703208 t^{42}-1419147660239735245 t^{41}+4091322808313743477 t^{40}+3576669643366665267 t^{39}-6616307159465274171 t^{38}-7660729875773249401 t^{37}+8427439571880463039 t^{36}+13806815668175216505 t^{35}-7309380390947163953 t^{34}-20295290823880097979 t^{33}+1596658389373069942 t^{32}+23371536052378861492 t^{31}+7311708133607141397 t^{30}-19861299394056161254 t^{29}-14669415358611128059 t^{28}+10691468157012440290 t^{27}+15996028367690527485 t^{26}-967875523743777140 t^{25}-11204260102702659458 t^{24}-4241537375038619232 t^{23}+4613494657441402303 t^{22}+4241281958050242492 t^{21}-431238716452858278 t^{20}-2082031101446095044 t^{19}-694469939157159982 t^{18}+497608341894786273 t^{17}+442485453025331675 t^{16}+21486755186604779 t^{15}-118238716169888033 t^{14}-52048440514411342 t^{13}+7391937564858721 t^{12}+13649500118147004 t^{11}+3749699524914665 t^{10}-824424917550924 t^9-815244760672307 t^8-184791376975533 t^7+18016076671965 t^6+20048719744748 t^5+4787837630586 t^4+417805442477 t^3-30025129249 t^2-9328730969 t-581472408\right)+d^{22} \left(16910994984 t^{60}-216513936556 t^{59}+532902274524 t^{58}+3962694177067 t^{57}-19647440481547 t^{56}-22422785680735 t^{55}+241938401887695 t^{54}-484194312613 t^{53}-1787766979309694 t^{52}+702377773626320 t^{51}+9380488633579234 t^{50}-4877247372354818 t^{49}-37706353471266900 t^{48}+21047596736653511 t^{47}+123480157632775411 t^{46}-71177590454194268 t^{45}-356182127146525161 t^{44}+181456135398066144 t^{43}+941812617284167870 t^{42}-254822728131154323 t^{41}-2154350444575363193 t^{40}-134694683144573171 t^{39}+3975837602651576705 t^{38}+1627306610562306277 t^{37}-5743225567983816533 t^{36}-4583124250664966849 t^{35}+6165049173221765373 t^{34}+8423439440665085849 t^{33}-3962699104899859667 t^{32}-11254523321657271449 t^{31}-759587702298389927 t^{30}+10823295233270299710 t^{29}+5706025937267125460 t^{28}-6672984556044701486 t^{27}-7785254801664075739 t^{26}+1243952508611979248 t^{25}+6038702538456339087 t^{24}+2162840395469908356 t^{23}-2554748530522300558 t^{22}-2464451259447935832 t^{21}+84972680370287824 t^{20}+1197101857753246874 t^{19}+547670438351597938 t^{18}-205122761786640395 t^{17}-292895629061179988 t^{16}-70270403207645360 t^{15}+53808340319149499 t^{14}+42890816678144975 t^{13}+6190027410298398 t^{12}-6387649425044076 t^{11}-3854819728052304 t^{10}-547181624069487 t^9+320717515556002 t^8+187434374481727 t^7+37395380228868 t^6-1561100004122 t^5-2633607797767 t^4-655155862116 t^3-80754087845 t^2-4783660837 t-83301912\right)+d^{21} \left(21322106048 t^{60}-357153883852 t^{59}+1792060458014 t^{58}+931742116404 t^{57}-33180077046549 t^{56}+54023978398206 t^{55}+258665762092742 t^{54}-730222984778512 t^{53}-1176650616223967 t^{52}+5133414926937896 t^{51}+3215949360267310 t^{50}-25314949455709487 t^{49}-3250693899453192 t^{48}+100061708321239907 t^{47}-11870420372952974 t^{46}-339238399437890710 t^{45}+42700750608722267 t^{44}+981140579622249464 t^{43}+47809016149678672 t^{42}-2319137418374010219 t^{41}-682985703690952563 t^{40}+4401167626609099247 t^{39}+2504161683767310832 t^{38}-6704021726456818544 t^{37}-6069927809279369084 t^{36}+7885305829432657964 t^{35}+11144426157491892942 t^{34}-6108049014149287836 t^{33}-15822874984064050435 t^{32}+592961921503389202 t^{31}+16946073056706643415 t^{30}+6606892911914138334 t^{29}-12684161541981207029 t^{28}-11259059461923513597 t^{27}+5036903151440891365 t^{26}+10624947395996892637 t^{25}+1424586785463416998 t^{24}-6104299620395167592 t^{23}-3676359822354936820 t^{22}+1603315866528990135 t^{21}+2577677964185523400 t^{20}+450228936822274355 t^{19}-876622720804139792 t^{18}-565429785256889630 t^{17}+57405874801933066 t^{16}+205346392780548932 t^{15}+71335249767114738 t^{14}-23642116814620626 t^{13}-26558820391655007 t^{12}-5853586493649205 t^{11}+2581739657652745 t^{10}+1948768447090684 t^9+376076662348253 t^8-92274450635835 t^7-68625199787767 t^6-15430313738600 t^5-680573141076 t^4+434985383145 t^3+108601906639 t^2+11002249559 t+431554920\right)-4096

==> polynomials/Q_51,69.tex <==
7 t^{60}-469 t^{59}+12243 t^{58}-179962 t^{57}+1710073 t^{56}-11146622 t^{55}+50436618 t^{54}-151059656 t^{53}+234052381 t^{52}+201754319 t^{51}-1997171213 t^{50}+4156174953 t^{49}-276368271 t^{48}-16121729292 t^{47}+28125989443 t^{46}+10114801856 t^{45}-91844072386 t^{44}+71207551873 t^{43}+144176744949 t^{42}-240946307269 t^{41}-143852139562 t^{40}+444155178380 t^{39}+211933500167 t^{38}-758631072892 t^{37}-566283660430 t^{36}+1572880442255 t^{35}+1147424840265 t^{34}-3278209064294 t^{33}-1468235705610 t^{32}+5658920692011 t^{31}+1086774068585 t^{30}-7779709012609 t^{29}-173590895819 t^{28}+8637279400530 t^{27}-607311827879 t^{26}-7893898126066 t^{25}+776534407543 t^{24}+6006819129143 t^{23}-440295413461 t^{22}-3807290297921 t^{21}+30374434426 t^{20}+1990583807321 t^{19}+168927986887 t^{18}-843536280849 t^{17}-167109688444 t^{16}+281979041986 t^{15}+95241032443 t^{14}-70193782028 t^{13}-37885749987 t^{12}+10723657559 t^{11}+10600264831 t^{10}+41488527 t^9-1838297880 t^8-421492833 t^7+126593931 t^6+69524854 t^5+6386776 t^4-2240824 t^3-705536 t^2-96320 t+d \left(14 t^{62}-112 t^{61}-8653 t^{60}+251509 t^{59}-3405735 t^{58}+28536707 t^{57}-159369712 t^{56}+588061194 t^{55}-1236420594 t^{54}+84721205 t^{53}+8290928658 t^{52}-24010330512 t^{51}+15135794859 t^{50}+78707265369 t^{49}-205501322323 t^{48}+40991092434 t^{47}+603210593909 t^{46}-819689345765 t^{45}-724121441401 t^{44}+2413006660911 t^{43}-28740416656 t^{42}-4239761193576 t^{41}+709915306165 t^{40}+6829889263231 t^{39}+1365425897361 t^{38}-14717740480593 t^{37}-6983306307439 t^{36}+34987738136370 t^{35}+11576041391816 t^{34}-70000866424696 t^{33}-8489516994784 t^{32}+111694142389678 t^{31}-2971317567696 t^{30}-144742237157656 t^{29}+14795440313585 t^{28}+155874104115376 t^{27}-17489061384543 t^{26}-141106977935576 t^{25}+9528669235781 t^{24}+107015537612358 t^{23}+1711314811558 t^{22}-66927432416958 t^{21}-8111700039703 t^{20}+33769181891403 t^{19}+7976236445175 t^{18}-13465139088159 t^{17}-4854558436185 t^{16}+4169947056833 t^{15}+2144686856608 t^{14}-957822362067 t^{13}-738264050967 t^{12}+121752788546 t^{11}+193491615501 t^{10}+15400690583 t^9-31288868924 t^8-10133225326 t^7+1311619620 t^6+1351085841 t^5+238697068 t^4-19875100 t^3-13562080 t^2-1986624 t-104576\right)+d^2 \left(-28 t^{64}+1034 t^{63}-13834 t^{62}+39994 t^{61}+1158831 t^{60}-18303607 t^{59}+137173836 t^{58}-598268566 t^{57}+1279850805 t^{56}+1298382935 t^{55}-17868069097 t^{54}+49645351321 t^{53}-20143548573 t^{52}-241626441639 t^{51}+616214340124 t^{50}-54243416908 t^{49}-2344850571287 t^{48}+3421681460134 t^{47}+3241444268129 t^{46}-12714924473667 t^{45}+2579119219807 t^{44}+26173214570193 t^{43}-17721863494633 t^{42}-40969855173165 t^{41}+31953259459065 t^{40}+72875140901554 t^{39}-31894718786607 t^{38}-168694368144229 t^{37}+28839102622073 t^{36}+378581459167824 t^{35}-63158084622075 t^{34}-702187632822618 t^{33}+159770531311494 t^{32}+1064477130423677 t^{31}-278337941891519 t^{30}-1346789516302497 t^{29}+326910935627434 t^{28}+1442324194591376 t^{27}-243636541793815 t^{26}-1303079623638383 t^{25}+67653830039712 t^{24}+972045043176630 t^{23}+86702292097024 t^{22}-578555328789356 t^{21}-137824665611022 t^{20}+264539943910979 t^{19}+103037578321796 t^{18}-90478293497289 t^{17}-49938150657471 t^{16}+23583534764979 t^{15}+17882927863677 t^{14}-4980113394972 t^{13}-5539502378841 t^{12}+581770502593 t^{11}+1505087993753 t^{10}+201861734591 t^9-247370151630 t^8-103770470739 t^7+2769472163 t^6+11566176606 t^5+2915155626 t^4+79969870 t^3-87498704 t^2-15969104 t-908528\right)+d^3 \left(8 t^{66}-440 t^{65}+9074 t^{64}-83639 t^{63}+118574 t^{62}+5209411 t^{61}-57237525 t^{60}+269792648 t^{59}-274422364 t^{58}-4034790559 t^{57}+25102997093 t^{56}-61020538284 t^{55}-8654337064 t^{54}+469168381296 t^{53}-1108381322272 t^{52}-168703592505 t^{51}+5555258868765 t^{50}-8154132079204 t^{49}-9388941945415 t^{48}+38069499504977 t^{47}-10411481298661 t^{46}-92183525765290 t^{45}+86900476961090 t^{44}+153078805790120 t^{43}-221986642164104 t^{42}-239328550134532 t^{41}+380353825536909 t^{40}+501896268819655 t^{39}-579565289651636 t^{38}-1216433835166746 t^{37}+972391554195222 t^{36}+2596646287285359 t^{35}-1732605707725583 t^{34}-4576870304386990 t^{33}+2767593473853165 t^{32}+6761564252629092 t^{31}-3562928766656821 t^{30}-8537382747361918 t^{29}+3439263328324272 t^{28}+9230411665408114 t^{27}-2145675451559399 t^{26}-8358508349932386 t^{25}+282349547081569 t^{24}+6061419134884375 t^{23}+1054992257737972 t^{22}-3300028329819819 t^{21}-1276561733894894 t^{20}+1234326489371531 t^{19}+779345280310074 t^{18}-278685262491399 t^{17}-282848018878122 t^{16}+37917947127056 t^{15}+67371543956273 t^{14}-11887305845686 t^{13}-18262744831201 t^{12}+3988811343050 t^{11}+6902604996549 t^{10}+807442300149 t^9-1355241728883 t^8-631267199012 t^7-27122442287 t^6+58522956268 t^5+19705420533 t^4+2141323715 t^3-162935136 t^2-59536592 t-4112144\right)+d^4 \left(24 t^{67}-888 t^{66}+9338 t^{65}+53468 t^{64}-2186519 t^{63}+22107824 t^{62}-94771324 t^{61}-95756743 t^{60}+3379827906 t^{59}-17871838352 t^{58}+35294429666 t^{57}+69531505739 t^{56}-580810705658 t^{55}+1155859455493 t^{54}+1005896309954 t^{53}-8913537007812 t^{52}+11649872785411 t^{51}+20934384058366 t^{50}-75730915604318 t^{49}+17479731015707 t^{48}+222318640347364 t^{47}-242281146922223 t^{46}-400214732841000 t^{45}+786383736524235 t^{44}+533038303054426 t^{43}-1670727784247552 t^{42}-843246045522090 t^{41}+2964170857524363 t^{40}+2149738213658004 t^{39}-5177531497438105 t^{38}-5633539575395402 t^{37}+9232312195774691 t^{36}+12097623921854880 t^{35}-15492714216457611 t^{34}-21348250660621202 t^{33}+22455360791449662 t^{32}+32051465749233693 t^{31}-26498885199406113 t^{30}-41688106406629939 t^{29}+23680155662963218 t^{28}+46471747235506072 t^{27}-13182778652664084 t^{26}-42573746608781866 t^{25}-191257859975745 t^{24}+29798027557514267 t^{23}+8637917354822607 t^{22}-14127034174858145 t^{21}-8691903434498946 t^{20}+3349352484933856 t^{19}+4320079028317955 t^{18}+345085801404047 t^{17}-970129192027117 t^{16}-358179005503942 t^{15}-10615197894829 t^{14}-15875373190179 t^{13}+8933585252491 t^{12}+41664040659557 t^{11}+24214904494254 t^{10}-1051623841941 t^9-6717709339773 t^8-2898489511115 t^7-261001418608 t^6+206221983281 t^5+89512291534 t^4+15750806038 t^3+1045933704 t^2-45696348 t-7680428\right)+d^5 \left(24 t^{68}-320 t^{67}-11846 t^{66}+342228 t^{65}-3270818 t^{64}+5571316 t^{63}+162526858 t^{62}-1670829432 t^{61}+7004637585 t^{60}-4443390810 t^{59}-96196282861 t^{58}+467809745984 t^{57}-683586031546 t^{56}-1884636981074 t^{55}+9738074973680 t^{54}-10013943772134 t^{53}-33148340294716 t^{52}+102710870420499 t^{51}-8227366137884 t^{50}-377102434240917 t^{49}+428575150231465 t^{48}+768473060645147 t^{47}-1757750233929441 t^{46}-891066605524842 t^{45}+4454719357897014 t^{44}+524848053312456 t^{43}-8968856490201673 t^{42}-753722311887135 t^{41}+16776546872515759 t^{40}+4592626481607104 t^{39}-31335212556107249 t^{38}-16115029231550322 t^{37}+56500886218610937 t^{36}+38733408814425473 t^{35}-91720369845098958 t^{34}-73850293401835326 t^{33}+127222637554594156 t^{32}+119453327099328943 t^{31}-144243116633240704 t^{30}-166877629290241217 t^{29}+123619582955321984 t^{28}+196948806338894668 t^{27}-62441880569151063 t^{26}-185164334672982606 t^{25}-11778185720396853 t^{24}+125195502162248801 t^{23}+54388326149472396 t^{22}-48958880954845838 t^{21}-47700493432076396 t^{20}+1064426119195868 t^{19}+19299583456557209 t^{18}+8885727366840455 t^{17}-1460673581139499 t^{16}-3341567410678401 t^{15}-1647532221096420 t^{14}-159067030544900 t^{13}+384632809541382 t^{12}+313185497262016 t^{11}+92426378133829 t^{10}-22706123130278 t^9-31582327854396 t^8-12193790217667 t^7-1540248842224 t^6+547355186768 t^5+308381923411 t^4+70296006176 t^3+8744355650 t^2+552799396 t+11888144\right)+d^{35} \left(-1680853902592 t^{69}+6280199841088 t^{68}+21011522522496 t^{67}-98119953826184 t^{66}-89904637498096 t^{65}+732786993816620 t^{64}-164100537337854 t^{63}-3360874524769542 t^{62}+5175186612035827 t^{61}+10188192266665066 t^{60}-43772270819857190 t^{59}-21955437598080907 t^{58}+245493843477236796 t^{57}+34983504981342271 t^{56}-1084671296012596862 t^{55}-169702141658578111 t^{54}+3726798465453121239 t^{53}+812673342240397424 t^{52}-11013845907873275588 t^{51}-4444986973088084551 t^{50}+25792751546335184478 t^{49}+14570138911033078519 t^{48}-52745125464051921452 t^{47}-41162767479379992795 t^{46}+91381776128386459464 t^{45}+106008020557152670407 t^{44}-96014265888591785305 t^{43}-142523626064993086769 t^{42}+168635185418863659590 t^{41}+321010490505478528126 t^{40}-76021194162711369361 t^{39}-439215014175238189862 t^{38}-140341916585373897483 t^{37}+322559281128978381842 t^{36}+139427514482345147227 t^{35}-405342046039622574766 t^{34}-439873704938794421272 t^{33}+44376698209316468594 t^{32}+293003106031970613179 t^{31}+48293739661690376988 t^{30}-195343413516118727554 t^{29}-84435940606352790547 t^{28}+150927093534827939789 t^{27}+184260807020212120352 t^{26}+39313058589532307962 t^{25}-68425931501711196338 t^{24}-54699560581255745992 t^{23}+3395859265347565787 t^{22}+26982187742719441876 t^{21}+13915516715335273477 t^{20}-3030251895291796963 t^{19}-7374726800140452912 t^{18}-3593048420861193253 t^{17}+185193964462555775 t^{16}+1300896791996054149 t^{15}+888536947067298915 t^{14}+318813519764330827 t^{13}+40851703184185343 t^{12}-24811724711300070 t^{11}-19580428753571784 t^{10}-7870143424853399 t^9-2223887649113949 t^8-474645140260969 t^7-77923786339241 t^6-9783011113233 t^5-916088490487 t^4-60916941539 t^3-2624083566 t^2-60260268 t-400718\right)+d^{34} \left(-1497803963776 t^{69}+4851709567936 t^{68}+18045470770416 t^{67}-64318934029360 t^{66}-56587612872604 t^{65}+230533264466826 t^{64}-360228456000230 t^{63}+1707476626998639 t^{62}+5449307530215860 t^{61}-26631254185076218 t^{60}-39047442102447620 t^{59}+183672699072962251 t^{58}+205412850176334307 t^{57}-879491665258714503 t^{56}-900327465459073992 t^{55}+3201395753909839284 t^{54}+3228173377569856902 t^{53}-9632464576798607881 t^{52}-10395683448727592708 t^{51}+23242738794675754548 t^{50}+27332045599691282682 t^{49}-49460865167659692970 t^{48}-67198141511994837342 t^{47}+83549809209093089388 t^{46}+139260013387851035268 t^{45}-112914751032806275547 t^{44}-233384015079371711531 t^{43}+176828066851112179074 t^{42}+494945620096339603414 t^{41}+32887251463716493044 t^{40}-499404823407957940047 t^{39}-92536516017774177986 t^{38}+592827892102937470038 t^{37}+245087222598635801113 t^{36}-714122307433473302552 t^{35}-792220542343832115032 t^{34}+20788612323634859757 t^{33}+344355033490870016954 t^{32}-233625510197902729718 t^{31}-663052058638304418445 t^{30}-265312277430909352699 t^{29}+362027863508972758108 t^{28}+458900197686142349498 t^{27}+114240358696729166946 t^{26}-135037761889954358750 t^{25}-91025609822191584799 t^{24}+44639004393805633027 t^{23}+81094315308769360935 t^{22}+29868455691867445486 t^{21}-17120164277217169145 t^{20}-22847694856104210933 t^{19}-7851807116901109414 t^{18}+3096928343163685455 t^{17}+4632825232981364294 t^{16}+2167088288384377700 t^{15}+195353512596797547 t^{14}-405218739860625247 t^{13}-323499984185622315 t^{12}-144559757638668869 t^{11}-44786261494058098 t^{10}-9834703249292647 t^9-1378928839193895 t^8-46574347718462 t^7+33322894129737 t^6+10180625434177 t^5+1697611284639 t^4+187789751586 t^3+13855189081 t^2+626330236 t+13277360\right)+d^{36} \left(-1274682843648 t^{69}+4150247626848 t^{68}+20690686241016 t^{67}-67012765888272 t^{66}-164565468675286 t^{65}+569106729484238 t^{64}+870139852671645 t^{63}-3396116033099679 t^{62}-3157290961615192 t^{61}+16441277714318632 t^{60}+5698717614628870 t^{59}-73557940503521401 t^{58}+5676584191547625 t^{57}+292451146304214870 t^{56}-112721028966107049 t^{55}-1115924032616087807 t^{54}+355658068948386147 t^{53}+3476916923779051797 t^{52}-904148234423330859 t^{51}-9957781370609394489 t^{50}+99852058504745155 t^{49}+23089980944995623873 t^{48}+5366349468728352330 t^{47}-43881726482945846259 t^{46}-17069161138169363293 t^{45}+84296720643106332172 t^{44}+74816199753312737369 t^{43}-77202579176290571465 t^{42}-102892631848931992349 t^{41}+87867865736818221843 t^{40}+148025934560524635213 t^{39}-106753204135150345575 t^{38}-283088285166742420223 t^{37}-57242257975026228074 t^{36}+225890895838351291590 t^{35}+118423623883035750456 t^{34}-187404307531962124049 t^{33}-212197495229165791180 t^{32}+43984977938846204643 t^{31}+187205162734564260268 t^{30}+71498207406091965591 t^{29}-72692617267887616702 t^{28}-59087013310413272575 t^{27}+34091603199977387139 t^{26}+62805237554825310465 t^{25}+17357780128756396888 t^{24}-24397598016618178661 t^{23}-23772074700520264075 t^{22}-3184849585318562605 t^{21}+8193835382681822785 t^{20}+6170855416196767210 t^{19}+688449959126311747 t^{18}-1712339489113542062 t^{17}-1272720881948984641 t^{16}-267973088409295982 t^{15}+207136165938601038 t^{14}+227032977413951408 t^{13}+118594393466007984 t^{12}+40859027465363303 t^{11}+9412797814961448 t^{10}+1120261733724636 t^9-131940218022006 t^8-105429574573975 t^7-29656246294783 t^6-5461283761748 t^5-718411933586 t^4-67757065752 t^3-4394014054 t^2-176470511 t-3317745\right)+d^{37} \left(-665731091616 t^{69}+1724153320520 t^{68}+14071910694200 t^{67}-23461309180354 t^{66}-147143273395840 t^{65}+174023261449892 t^{64}+1067487034103657 t^{63}-917658179183536 t^{62}-5979258821153655 t^{61}+3803447635304310 t^{60}+26134004539849970 t^{59}-17589949129700940 t^{58}-102502591971809842 t^{57}+65786872670629754 t^{56}+333632756157276120 t^{55}-274493490379020505 t^{54}-1104068650174987732 t^{53}+716375027549156834 t^{52}+3045874745832505740 t^{51}-1695980827941685722 t^{50}-7920597461038203525 t^{49}+2555704782465138392 t^{48}+18534378505732229479 t^{47}+1629884707010039559 t^{46}-30000425710866927392 t^{45}-3156511086606918160 t^{44}+61539892356718679188 t^{43}+38273580845446514726 t^{42}-71522633720271437462 t^{41}-88744436908523652746 t^{40}+31709972736386125988 t^{39}+82852406463158753608 t^{38}-36124322643712452261 t^{37}-118982870041762919422 t^{36}-8342526754382646988 t^{35}+121929180072045048370 t^{34}+63545476203354566493 t^{33}-84347290623349446332 t^{32}-98722935592348560059 t^{31}+18837976107337364503 t^{30}+89223660070581634466 t^{29}+41192846748924621101 t^{28}-29302215805834690268 t^{27}-35402895178642232888 t^{26}+820069170882825061 t^{25}+20253972301724347779 t^{24}+9977318642652827069 t^{23}-5111251538965612482 t^{22}-7935286152757764339 t^{21}-2512534293392644826 t^{20}+1752901805878459905 t^{19}+2047840648195625603 t^{18}+650926603304384601 t^{17}-276013050644372609 t^{16}-392801562019912116 t^{15}-193805433000491964 t^{14}-37115695594259248 t^{13}+15539544712616725 t^{12}+16509663513329591 t^{11}+7841549456798416 t^{10}+2550463244906467 t^9+618044758233731 t^8+113714225333284 t^7+15668753656699 t^6+1534345240487 t^5+91333575515 t^4+968844644 t^3-340043953 t^2-27835263 t-774000\right)+d^{33} \left(-557232074944 t^{69}-3074573599120 t^{68}+25225363529208 t^{67}+52008113980340 t^{66}-331399733313722 t^{65}-701894619524678 t^{64}+2795414026098093 t^{63}+7325068224123566 t^{62}-18458215892358669 t^{61}-54849819611946828 t^{60}+100485488280488128 t^{59}+305439804948419135 t^{58}-452865692275604135 t^{57}-1331284955023564143 t^{56}+1685077173979302665 t^{55}+4704576023405372071 t^{54}-5309834032844729884 t^{53}-14165208384282586279 t^{52}+13837515773202570300 t^{51}+36312023384732616622 t^{50}-31949474787913951584 t^{49}-85325419276197784404 t^{48}+57593941384507214244 t^{47}+172856106734054686821 t^{46}-92124412112920859672 t^{45}-329404610221512823340 t^{44}+103620593073179419838 t^{43}+595729950612035112723 t^{42}+91583585050694115740 t^{41}-644842368449753619947 t^{40}-44198780237695851035 t^{39}+1121957406654735844693 t^{38}+697441302135868658831 t^{37}-891514456245204394998 t^{36}-1107794721432833949053 t^{35}+266112611847516969771 t^{34}+727701875034499663478 t^{33}-654385010787432708079 t^{32}-1816349280613467060193 t^{31}-1151643617325607930787 t^{30}+266934213123836434358 t^{29}+723632894925098953644 t^{28}+197255086086224700066 t^{27}-232057668051400967581 t^{26}-100037368313259738445 t^{25}+185643193219297732107 t^{24}+223581343622186977385 t^{23}+68845112381239564198 t^{22}-50047989425707177682 t^{21}-54515456397239845334 t^{20}-10436162948165634948 t^{19}+15503826198748429568 t^{18}+14164067917265203877 t^{17}+4294214387070058390 t^{16}-1471752087645281299 t^{15}-2274574606270567027 t^{14}-1268069976067921444 t^{13}-416107562578356848 t^{12}-64181059621328942 t^{11}+14349683591428185 t^{10}+13628765725814907 t^9+5251296689456305 t^8+1379260200442969 t^7+270891104707985 t^6+40724706085231 t^5+4665120122512 t^4+396806943843 t^3+23742455609 t^2+894945521 t+16010198\right)+d^{25} \left(-317410102608 t^{69}+14882196190536 t^{68}-174019651797684 t^{67}+751047830219334 t^{66}+68377979701638 t^{65}-10990236895333014 t^{64}+24935412573535863 t^{63}+57324168721137546 t^{62}-280811487440627391 t^{61}-59392923796641399 t^{60}+1733436035006906375 t^{59}-1055497024605706956 t^{58}-7521772034116115110 t^{57}+8475343976104269243 t^{56}+25577287098671258497 t^{55}-38689981639961457574 t^{54}-73183539344914657077 t^{53}+130399800584582265054 t^{52}+186057931646500132203 t^{51}-351922696952461273342 t^{50}-436404742692171139666 t^{49}+786777698090140876603 t^{48}+958349198131991246145 t^{47}-1472333248024189393207 t^{46}-1954946067850501807331 t^{45}+2286058961867388737221 t^{44}+3631511365398608971430 t^{43}-2831491914692951261619 t^{42}-5997767444368026184128 t^{41}+2475391973131545233846 t^{40}+8589907055508808986740 t^{39}-791736147911545124263 t^{38}-10757192205881530376044 t^{37}-2601940032135846719015 t^{36}+11047995637569937163608 t^{35}+6440800485608273323535 t^{34}-9731593708509506822928 t^{33}-10330733733754970925938 t^{32}+8932513854398329094807 t^{31}+24086035102710552944155 t^{30}+18192208822537983814707 t^{29}+233245273458831802015 t^{28}-12435367406949968359791 t^{27}-14458399233711902759817 t^{26}-11261048175242689974117 t^{25}-7891919436968614000880 t^{24}-5125291490250600372995 t^{23}-2518602476925972169443 t^{22}-505674574669311269768 t^{21}+384097774111278718667 t^{20}+382925421600240304723 t^{19}+117593022660003423040 t^{18}-30449661481935448715 t^{17}-37024489954304486971 t^{16}-3299851177419267661 t^{15}+13243097450128026175 t^{14}+11457580169615978440 t^{13}+5181042279927783366 t^{12}+1309043724429897238 t^{11}+23815603718573058 t^{10}-144349187064111553 t^9-76047583885229760 t^8-24218644588226454 t^7-5567311765944703 t^6-964501622541021 t^5-126315426925221 t^4-12237236665153 t^3-833576896884 t^2-35892746558 t-740132620\right)+d^{26} \left(-228873202368 t^{69}+14963141294688 t^{68}-181109806457448 t^{67}+754505411712552 t^{66}+301009071378942 t^{65}-11350652577681558 t^{64}+20761502939644848 t^{63}+68956831366568217 t^{62}-247025011715708838 t^{61}-206072062156157685 t^{60}+1601227994136952957 t^{59}+28370505079736823 t^{58}-7430910334800684511 t^{57}+2877861060010366832 t^{56}+27490323786316488527 t^{55}-16408495163877647043 t^{54}-85964011864734832275 t^{53}+57618520093808723398 t^{52}+234964908569014814570 t^{51}-148597185449456245728 t^{50}-570319967048211954702 t^{49}+288922001106764135335 t^{48}+1232473018259900256415 t^{47}-393216657801785745619 t^{46}-2353871703126681016969 t^{45}+221331172026608731108 t^{44}+3919180339200451134139 t^{43}+609455542483271250221 t^{42}-5576355770783435080381 t^{41}-2445272067696687093124 t^{40}+6437853660827197529554 t^{39}+4864039187335183870665 t^{38}-6012960876907193911791 t^{37}-7328919050765258948374 t^{36}+3779660086802655738792 t^{35}+8440136415596584626868 t^{34}-98956811640434797201 t^{33}-4442377961967594488286 t^{32}+6423210264120930868262 t^{31}+18062215790987664188857 t^{30}+13047465825118795265498 t^{29}-4334019134045928102519 t^{28}-16696272350154649225849 t^{27}-16215271266867087609510 t^{26}-9178508540935253408265 t^{25}-3850274128504079564900 t^{24}-2093487428491133757383 t^{23}-1645445345562000931457 t^{22}-942518853501809302188 t^{21}-163812277531894781997 t^{20}+195151762085501624370 t^{19}+161692253468006932117 t^{18}+30026552870072291550 t^{17}-31358548893025112614 t^{16}-26375542653897065952 t^{15}-6601150750243190892 t^{14}+3221669993642033896 t^{13}+3978930256217392432 t^{12}+2097462680316755498 t^{11}+714549948108438769 t^{10}+160444232843692023 t^9+17801296894269922 t^8-2597363759813781 t^7-1792193191285294 t^6-473627846938744 t^5-81211873331944 t^4-9672238229338 t^3-783354599442 t^2-39233329192 t-924211309\right)+d^{38} \left(-175079168472 t^{69}+484136091268 t^{68}+5887097684522 t^{67}-324153995593 t^{66}-72078176495627 t^{65}-52021052658713 t^{64}+559826568978815 t^{63}+631336374581244 t^{62}-3249138350278387 t^{61}-4797617461705332 t^{60}+13650286172986697 t^{59}+22884053506971507 t^{58}-52032985950601563 t^{57}-97559867090190849 t^{56}+149772944762936300 t^{55}+302729094177793195 t^{54}-445992493289296934 t^{53}-947375108374075688 t^{52}+1013276286738198155 t^{51}+2520277546412567000 t^{50}-1863122085272865778 t^{49}-5689120554737982889 t^{48}+3446402193646250608 t^{47}+13954562761466000214 t^{46}+681804283232668175 t^{45}-19649204122009454188 t^{44}-2597708025681598146 t^{43}+31616147518396180380 t^{42}+10109160674869164521 t^{41}-53422320915554073368 t^{40}-52120749028048574696 t^{39}+30091481715144569683 t^{38}+69403301674305864668 t^{37}+5104653383349429908 t^{36}-56122796202489964597 t^{35}-21529710818296951030 t^{34}+40860870638735237335 t^{33}+30250893702949963230 t^{32}-26292049282276117491 t^{31}-37985044584381479152 t^{30}+4003503443642835338 t^{29}+33615905476924102508 t^{28}+18569177414370752250 t^{27}-9310637832569199903 t^{26}-15459604820797454255 t^{25}-3461338604559357472 t^{24}+5810901953303955817 t^{23}+4697062547335423737 t^{22}-167148301426194345 t^{21}-2236601887759884735 t^{20}-1326277060027798769 t^{19}-2974452989650459 t^{18}+426388477424325199 t^{17}+235773814373325235 t^{16}-2867228128750131 t^{15}-83464401893986305 t^{14}-63593756934801052 t^{13}-28079687358549220 t^{12}-8045767728918153 t^{11}-1245839184474372 t^{10}+101240666961329 t^9+130619930981492 t^8+45310430803340 t^7+10153346576259 t^6+1641589084856 t^5+195366790048 t^4+16833579291 t^3+999525258 t^2+36792135 t+637682\right)+d^{24} \left(-149329926896 t^{69}+9121548778504 t^{68}-116302379250068 t^{67}+545458506035670 t^{66}-116800884840444 t^{65}-7947566438532896 t^{64}+21415487204962684 t^{63}+35649517128015181 t^{62}-233915237528043606 t^{61}+52692548450594731 t^{60}+1389829317992137932 t^{59}-1530623387376992360 t^{58}-5634586755317671480 t^{57}+10176839204575951546 t^{56}+17224787375066051743 t^{55}-43963670188697245383 t^{54}-42622062475069306046 t^{53}+145319680071059142215 t^{52}+92178266465535595913 t^{51}-393113879947593003901 t^{50}-191631335882307320135 t^{49}+900736080156185491007 t^{48}+413721843236786880153 t^{47}-1776956391056125958417 t^{46}-923830174974550840514 t^{45}+3027405216899296657195 t^{44}+1994036453441831286371 t^{43}-4405454624727848422465 t^{42}-3897664588628550716390 t^{41}+5316891657784066609031 t^{40}+6668926402084325160343 t^{39}-4923956950855775635740 t^{38}-9929592781768130438532 t^{37}+2173613507383099831466 t^{36}+12173957026351602693481 t^{35}+2794725072547129485740 t^{34}-12399634381289052650192 t^{33}-10859885708338849042515 t^{32}+6130025883931928251198 t^{31}+19447544343205835612921 t^{30}+18678911555316272213959 t^{29}+8824710728486201572754 t^{28}-1953710464712426562823 t^{27}-9889536706578647882951 t^{26}-13579035258376607092263 t^{25}-12347517525919961556783 t^{24}-7623104557168377626730 t^{23}-2647030542246965077816 t^{22}+178448248846747278040 t^{21}+778666645647634601462 t^{20}+405456009070508206038 t^{19}+56504708020984328858 t^{18}-28768265214319496017 t^{17}+5075987255674186735 t^{16}+29103923672714616396 t^{15}+22871296064409074012 t^{14}+8817295512969254418 t^{13}+754077865895555900 t^{12}-1263235943398907248 t^{11}-929631323566114585 t^{10}-383009333212618431 t^9-110611386964945093 t^8-23371437805135268 t^7-3534651857282629 t^6-340789283236185 t^5-10065701034942 t^4+2529100376285 t^3+431549109075 t^2+30828189363 t+909132602\right)+d^{16} \left(-1556747848 t^{69}+36777508412 t^{68}-377900700466 t^{67}+2217525185417 t^{66}-8133606038813 t^{65}+16506886317509 t^{64}+20340010160700 t^{63}-343951224408699 t^{62}+1257114055216026 t^{61}-449214066360445 t^{60}-11101444954418949 t^{59}+27971200329270138 t^{58}+31349312856418413 t^{57}-220262591292167594 t^{56}+76586401777729098 t^{55}+1016270053357867001 t^{54}-1077495220907870390 t^{53}-3441602863005006347 t^{52}+5349478588592992927 t^{51}+9785069747741151226 t^{50}-17904611777393458731 t^{49}-26118090643121375613 t^{48}+45330044441475288290 t^{47}+69246010101933905173 t^{46}-86907683539585815673 t^{45}-176959943340535232881 t^{44}+107444906385511100696 t^{43}+403368672953490758306 t^{42}+11867706045176741357 t^{41}-751735093944025188934 t^{40}-497826478872324069000 t^{39}+1003515164172900552956 t^{38}+1534117211949916105844 t^{37}-562098443622290149476 t^{36}-2779806913660091975644 t^{35}-1227005788873937422389 t^{34}+2891524031502197138780 t^{33}+3836069456070494267566 t^{32}-374014063856780932566 t^{31}-4552164498198799395096 t^{30}-3469628064142156758516 t^{29}+1214512011591007587727 t^{28}+3907441368798737202823 t^{27}+2435105132591983245783 t^{26}-449148865043466211873 t^{25}-1588046856926859135399 t^{24}-784510179458787062703 t^{23}+269575555763592074270 t^{22}+496490634293491417103 t^{21}+133267232521832546572 t^{20}-182849628180567995130 t^{19}-209138895015390167389 t^{18}-84668503926022866253 t^{17}+13403497330841680932 t^{16}+37139582835060270929 t^{15}+22311115810818875131 t^{14}+5917854356751023182 t^{13}-920078251164925730 t^{12}-1631400107973554430 t^{11}-795977206404504561 t^{10}-219303053150810292 t^9-25809006837136121 t^8+6707313477037591 t^7+4479625234766940 t^6+1305428122063930 t^5+250284348853915 t^4+33523849938666 t^3+3070523373491 t^2+175023346571 t+4723351408\right)+d^{17} \left(-1080582256 t^{69}+20998635984 t^{68}-186167039536 t^{67}+1401931308572 t^{66}-11786039389229 t^{65}+74173361661222 t^{64}-226445964965425 t^{63}-184659690058593 t^{62}+3627536720825823 t^{61}-7982150944714239 t^{60}-14843400657363618 t^{59}+86931621944354789 t^{58}-27630835295454733 t^{57}-471277022818207762 t^{56}+596443014895643068 t^{55}+1706727007897353469 t^{54}-3535173021863833029 t^{53}-4737115218086480399 t^{52}+13814014311815504497 t^{51}+11627004962563704986 t^{50}-41551559965843364904 t^{49}-29865983963227930641 t^{48}+101675774327319270790 t^{47}+85348620319217204142 t^{46}-202631830837600596748 t^{45}-243799549591862380389 t^{44}+305514716058957379017 t^{43}+614142328075036699933 t^{42}-239360521769703637435 t^{41}-1257597217021266482159 t^{40}-370874864821371880184 t^{39}+1915715570285148928931 t^{38}+1936108135844730063237 t^{37}-1678046098283900444512 t^{36}-4180092024776154474690 t^{35}-737820553745997887255 t^{34}+5142668262122686609513 t^{33}+5132993481693125275674 t^{32}-1872672174505629024313 t^{31}-7409105555102059490732 t^{30}-4766474443508128590269 t^{29}+2599097356483750802152 t^{28}+6537972969668846477536 t^{27}+4215234507203888984837 t^{26}-377903876028384967701 t^{25}-2620526756689789522502 t^{24}-1833903539248155563006 t^{23}-173561068491142371184 t^{22}+598128797596513856073 t^{21}+397424072081373283298 t^{20}-34265870647444397056 t^{19}-212966979048854240874 t^{18}-149355466203489421340 t^{17}-34763315915828351670 t^{16}+22887605688421277411 t^{15}+26407248346571255120 t^{14}+12591301492300049946 t^{13}+2669336302185909061 t^{12}-627536075325098153 t^{11}-783992812830558337 t^{10}-354159116744936855 t^9-99961144070000632 t^8-17594671825444944 t^7-1111532586552604 t^6+376355971052216 t^5+141107671456256 t^4+25061467346687 t^3+2708615731695 t^2+171603579180 t+4944966389\right)+d^{15} \left(-800320872 t^{69}+19391269100 t^{68}-198393115070 t^{67}+1052592887581 t^{66}-2395907178002 t^{65}-5065916636746 t^{64}+58049195993768 t^{63}-193210004064133 t^{62}+145398926059407 t^{61}+1375483318696029 t^{60}-5453716131326426 t^{59}+2663503528698364 t^{58}+34021258465040559 t^{57}-75285056421248338 t^{56}-91494199994834721 t^{55}+489541425441354324 t^{54}-14884466106093480 t^{53}-2027599847952277860 t^{52}+1136674917386113983 t^{51}+6533529292637050276 t^{50}-5211728888930878544 t^{49}-18272629996065433196 t^{48}+14202976948987282417 t^{47}+47100752311190255097 t^{46}-24064556801071751799 t^{45}-112155817184204096113 t^{44}+8647077767308255324 t^{43}+235064051663186517041 t^{42}+105038611424826161162 t^{41}-396972750840279328867 t^{40}-437545045238557932142 t^{39}+445558323654974488901 t^{38}+1048291849506158402636 t^{37}-41263545882334868406 t^{36}-1662175166061100301651 t^{35}-1092837857558017290268 t^{34}+1496359005485818905627 t^{33}+2480354297114081959144 t^{32}+90272389132063572659 t^{31}-2611661503384398024269 t^{30}-2100053768280356629021 t^{29}+701162019747838153695 t^{28}+2198413437665865619819 t^{27}+1127424292049916312804 t^{26}-550322240027700790714 t^{25}-906499773445238256553 t^{24}-161581401919983204301 t^{23}+425688087370689421248 t^{22}+333048088465316789470 t^{21}-38465456278845146839 t^{20}-218262146833559719715 t^{19}-151884044207310825238 t^{18}-24595784965199329406 t^{17}+36935494292725461062 t^{16}+33841471629074089769 t^{15}+12700602181155960024 t^{14}+57773024495365074 t^{13}-2639262384026518487 t^{12}-1572229852272371500 t^{11}-470766085707703847 t^{10}-41300990258247259 t^9+31805364327832195 t^8+18677251389868197 t^7+5745951633983340 t^6+1200125856802063 t^5+178729478516949 t^4+18864186889062 t^3+1352193671026 t^2+59718774445 t+1250052034\right)+d^{14} \left(-273280808 t^{69}+6539468116 t^{68}-63203286410 t^{67}+271854891287 t^{66}+47947414299 t^{65}-6512552711538 t^{64}+32291530449302 t^{63}-53594833764640 t^{62}-152637885780480 t^{61}+1007585402414368 t^{60}-1603018188837926 t^{59}-3698367218962089 t^{58}+19114319505667015 t^{57}-11719737285948197 t^{56}-90935427985443851 t^{55}+175718822414115694 t^{54}+243072477061909006 t^{53}-946264950212350975 t^{52}-326829694730088354 t^{51}+3494225249125605568 t^{50}-120736717515574899 t^{49}-10387333085184800657 t^{48}+1151703504945822610 t^{47}+26789712332856711682 t^{46}+1089766060005771966 t^{45}-61179665551371299869 t^{44}-22814432616361913277 t^{43}+119822841031687184825 t^{42}+103452285158016558447 t^{41}-183054487606385591869 t^{40}-299583729214186360590 t^{39}+161457349895371474679 t^{38}+620291068531763678752 t^{37}+113900383002723308212 t^{36}-893501050017284046975 t^{35}-739444315643238590385 t^{34}+725065157009475988884 t^{33}+1412686553582552908529 t^{32}+123014449939585147239 t^{31}-1410718315045162641102 t^{30}-1089348825762822157948 t^{29}+485661985709446143449 t^{28}+1168014199797739787684 t^{27}+386270340157019329802 t^{26}-513844078254474040336 t^{25}-477827082564754935673 t^{24}+104508398770397434191 t^{23}+383528965083893382779 t^{22}+181871451241930912605 t^{21}-104845884272138252718 t^{20}-179471757939847860524 t^{19}-86307511542875724666 t^{18}+10085691682840269134 t^{17}+37897275056446015088 t^{16}+22535619090835459751 t^{15}+4248907105245997880 t^{14}-2800192178933158662 t^{13}-2593275677893336082 t^{12}-982364513839369689 t^{11}-128265567019907314 t^{10}+67373912825601735 t^9+48877555345072630 t^8+16770659241852846 t^7+3681319889821703 t^6+512839377710316 t^5+33582816151308 t^4-2331725413651 t^3-754461144289 t^2-69978290935 t-2499431936\right)+d^{13} \left(-67112392 t^{69}+1515290908 t^{68}-12512984418 t^{67}+23908524877 t^{66}+344830355833 t^{65}-2992015585363 t^{64}+9418949254925 t^{63}+2643680896529 t^{62}-124912684853327 t^{61}+388095538391763 t^{60}-15559181532008 t^{59}-3006810817876263 t^{58}+6718925954672940 t^{57}+6317774361590988 t^{56}-48762290931704559 t^{55}+33661371761613604 t^{54}+192482138579355219 t^{53}-323907650954480729 t^{52}-516316896246808997 t^{51}+1463170813667470023 t^{50}+1088891149480462491 t^{49}-4767162853899269461 t^{48}-2348092223109508604 t^{47}+12619861865431472554 t^{46}+6810761042850349631 t^{45}-28229339965780756773 t^{44}-22963779578594217060 t^{43}+52210857130991994602 t^{42}+69435346303464323995 t^{41}-71304472065184000783 t^{40}-169649948914512667069 t^{39}+40594963841049526092 t^{38}+319437239907205669442 t^{37}+113645422880986838265 t^{36}-430386726742053724271 t^{35}-418221115126210308775 t^{34}+329083202620669847156 t^{33}+720606672626894118957 t^{32}+64167805841759411259 t^{31}-717947854231181653091 t^{30}-497526627948686488989 t^{29}+333260940768558316094 t^{28}+586663467604762579695 t^{27}+66631004709505213020 t^{26}-379457150855347745813 t^{25}-229974024338328388376 t^{24}+155555584127639998750 t^{23}+264481146042333785990 t^{22}+79927243973472536415 t^{21}-100977328106651796644 t^{20}-117101161405773746578 t^{19}-38284970084001335091 t^{18}+20542145121344549983 t^{17}+27594428504607199543 t^{16}+11573389495655379303 t^{15}-388009627264988215 t^{14}-3085957636648534614 t^{13}-1732262643418038928 t^{12}-399219994664945994 t^{11}+65945439425628500 t^{10}+90483739916893409 t^9+37300708834833538 t^8+8772637243002522 t^7+982313772231122 t^6-103566185625893 t^5-68033321625976 t^4-14484785445448 t^3-1775415313461 t^2-125057332162 t-3970055160\right)+d^{12} \left(-11598176 t^{69}+223223000 t^{68}-1033793240 t^{67}-9753010494 t^{66}+146565851270 t^{65}-724199224803 t^{64}+731002783237 t^{63}+9402905058974 t^{62}-49275794692460 t^{61}+67677179883555 t^{60}+267372592167990 t^{59}-1279589536612585 t^{58}+1003660669177940 t^{57}+6393648576142470 t^{56}-17042645875425149 t^{55}-8947152272912269 t^{54}+93979811501817240 t^{53}-58339823008953527 t^{52}-329454617215081102 t^{51}+438241860936282271 t^{50}+888661365261941626 t^{49}-1696321689115558045 t^{48}-2162254197118535365 t^{47}+4784104909302860567 t^{46}+5460476396444090057 t^{45}-10680765615407745794 t^{44}-14564912443026303277 t^{43}+18641004569739011104 t^{42}+37126781213327026802 t^{41}-21564933331240210849 t^{40}-81646202848452871094 t^{39}-117212844839774595 t^{38}+143633532508689232213 t^{37}+74703049595445356470 t^{36}-184669488248878976002 t^{35}-207534423052580901905 t^{34}+137399821038422026004 t^{33}+334487692189516792683 t^{32}+24037306556096645818 t^{31}-342716645605238113996 t^{30}-206996524382259021168 t^{29}+203043035342410756799 t^{28}+278648716793378091914 t^{27}-26362841146239693462 t^{26}-232073702542409106803 t^{25}-100962548646735972868 t^{24}+118927367178103997471 t^{23}+151092790371491393963 t^{22}+26783335920669815659 t^{21}-69952321426069019038 t^{20}-63737595534715671496 t^{19}-12265523825620665182 t^{18}+17614637112719321060 t^{17}+15973331415965287220 t^{16}+4491578650110581535 t^{15}-1784743517458346742 t^{14}-2192168467860868401 t^{13}-865550798719727337 t^{12}-56526959195107674 t^{11}+114431029578617618 t^{10}+66476272187118238 t^9+18564267853589420 t^8+1949978509260342 t^7-621131874604305 t^6-350183756283295 t^5-88919168473732 t^4-14350754264628 t^3-1518374090968 t^2-97630893961 t-2931304593\right)+d^{11} \left(-1214688 t^{69}+11781568 t^{68}+197170496 t^{67}-4181894152 t^{66}+28119614734 t^{65}-40247091992 t^{64}-582054283510 t^{63}+4057513078671 t^{62}-9160402828267 t^{61}-16561786568223 t^{60}+152795307786070 t^{59}-295963893588471 t^{58}-439000478654732 t^{57}+2990895159841886 t^{56}-3009702956882089 t^{55}-11523408091544643 t^{54}+31148130393588635 t^{53}+15315800500212011 t^{52}-143631098762036790 t^{51}+57233826115639436 t^{50}+460420028375629458 t^{49}-401807421787902692 t^{48}-1216669108615894476 t^{47}+1335879057712829095 t^{46}+2988951292019873904 t^{45}-3063246592612213005 t^{44}-7215298653778513062 t^{43}+4894942813016957458 t^{42}+16598622356301593041 t^{41}-3598181986921469504 t^{40}-33794624178068165137 t^{39}-8329761714242637509 t^{38}+56336565704545329462 t^{37}+40470574396760383226 t^{36}-69835724860309101384 t^{35}-93149344033434431550 t^{34}+50959859827669518165 t^{33}+143147418714658899478 t^{32}+9059644739316443472 t^{31}-152271325255553695768 t^{30}-81947270617792684294 t^{29}+106730914763365287741 t^{28}+124953804556574506862 t^{27}-32079400064809649395 t^{26}-121184192555178477555 t^{25}-40727140694592036412 t^{24}+69001977373206377615 t^{23}+74050948187645782747 t^{22}+5439749808378307938 t^{21}-39278490326798219429 t^{20}-29630479706454395442 t^{19}-1768636603553906870 t^{18}+11008229302507699098 t^{17}+7647998913321374299 t^{16}+1124478198120531905 t^{15}-1554060676262702119 t^{14}-1195089853480816170 t^{13}-319083247701234996 t^{12}+64610377739030194 t^{11}+88713902103368250 t^{10}+34715327861630430 t^9+5387182854722046 t^8-1206768561869428 t^7-976662310320069 t^6-305728430564458 t^5-60366314576052 t^4-8064349249095 t^3-716928363768 t^2-38764128988 t-971741540\right)+d^{10} \left(-15072 t^{69}-2972272 t^{68}+75294836 t^{67}-622538164 t^{66}+206904749 t^{65}+32905957580 t^{64}-251703561979 t^{63}+694108540973 t^{62}+1221523621347 t^{61}-15452122406094 t^{60}+43188713310165 t^{59}+9544803355638 t^{58}-372577769137857 t^{57}+811696922534143 t^{56}+643125451244694 t^{55}-5656884610415930 t^{54}+5503716565015993 t^{53}+18508499462885494 t^{52}-43615345263191446 t^{51}-29752826222259195 t^{50}+174721133871189808 t^{49}-8563264214093111 t^{48}-513368039076091764 t^{47}+178180195578258364 t^{46}+1281494439061791802 t^{45}-482275815211893723 t^{44}-2943609379914917911 t^{43}+536180128302112448 t^{42}+6300280306935643682 t^{41}+955315051176293791 t^{40}-12030580638143758290 t^{39}-6568746204123305882 t^{38}+19096173435497573910 t^{37}+19185891726148574523 t^{36}-22787567363496960667 t^{35}-38450339037807088082 t^{34}+15830000113614808360 t^{33}+56869550844596543242 t^{32}+4887249809266409689 t^{31}-62380529210328342386 t^{30}-32124677121760815114 t^{29}+48388756069406646401 t^{28}+52621315299024648151 t^{27}-18641082233751969978 t^{26}-55075623093828687573 t^{25}-15233377780316084649 t^{24}+33191170360102906352 t^{23}+31703259269670621511 t^{22}-616269697563033264 t^{21}-18670943822365119825 t^{20}-11894531491074884174 t^{19}+982162487538383318 t^{18}+5564445923600832711 t^{17}+3070708462462087861 t^{16}-9779503590768374 t^{15}-923730537018466534 t^{14}-524767012168086097 t^{13}-72960283722009112 t^{12}+69534020384554940 t^{11}+48939274891708106 t^{10}+13313408978130988 t^9-265032338352805 t^8-1648818977543275 t^7-701901624858092 t^6-168945674922591 t^5-25706628462131 t^4-2327600088324 t^3-86790081353 t^2+3443292331 t+338745665\right)+d^6 \left(8 t^{69}+404 t^{68}-17214 t^{67}+138083 t^{66}+1799785 t^{65}-42900503 t^{64}+333791169 t^{63}-807667057 t^{62}-5930149851 t^{61}+58944089379 t^{60}-204208549816 t^{59}+73210325615 t^{58}+2010449581501 t^{57}-7016354406240 t^{56}+3484679966427 t^{55}+38125332026308 t^{54}-96564585526924 t^{53}-24342090431707 t^{52}+469882232730948 t^{51}-514806794207549 t^{50}-1121568077192829 t^{49}+2748116735927266 t^{48}+1149459296961307 t^{47}-8189356742313805 t^{46}+1266500501672576 t^{45}+18348888603238066 t^{44}-6945075002914233 t^{43}-36570251748724306 t^{42}+12830815654568090 t^{41}+72227425537864890 t^{40}-10723914689726378 t^{39}-141808007249052927 t^{38}-12080574242839077 t^{37}+259452371368310429 t^{36}+71993491714599933 t^{35}-417453922068647692 t^{34}-186350247279446225 t^{33}+569823492340424235 t^{32}+362204541892649192 t^{31}-635899543385737382 t^{30}-572941310465772333 t^{29}+534185963878768138 t^{28}+732946959806649112 t^{27}-250639427601266467 t^{26}-715549286287678350 t^{25}-89954709567469577 t^{24}+470491805624405324 t^{23}+273160365640200549 t^{22}-144188576105929586 t^{21}-216997004901281614 t^{20}-43355610737728327 t^{19}+71626865341608904 t^{18}+56846078552692070 t^{17}+5775707035381229 t^{16}-16099952005480818 t^{15}-11255773611523257 t^{14}-1806485221424792 t^{13}+2055075418137861 t^{12}+1625024059478322 t^{11}+430384469255785 t^{10}-98007518131938 t^9-126645566581330 t^8-48908557552011 t^7-8116608449364 t^6+868331889266 t^5+837475531165 t^4+225002793093 t^3+33788437351 t^2+2872505945 t+109029511\right)+d^7 \left(248 t^{69}-908 t^{68}-174714 t^{67}+3371219 t^{66}-18700405 t^{65}-122087880 t^{64}+2448043114 t^{63}-15095845116 t^{62}+31044285638 t^{61}+145768053680 t^{60}-1192373211378 t^{59}+2958993495055 t^{58}+1903882694724 t^{57}-29873187726963 t^{56}+59748605044387 t^{55}+56458313158589 t^{54}-426161876504121 t^{53}+411113536967282 t^{52}+1259255466898726 t^{51}-3097757250004089 t^{50}-1252001506168792 t^{49}+10983600956970945 t^{48}-4145211854986909 t^{47}-27187412813489726 t^{46}+21963563998260064 t^{45}+56453724313568636 t^{44}-57155279727028534 t^{43}-114724143895070822 t^{42}+107254651699606946 t^{41}+243185369512542649 t^{40}-157085511735388681 t^{39}-507560196911005782 t^{38}+167202998292134672 t^{37}+959943269189961829 t^{36}-58437476818678790 t^{35}-1565809328324833683 t^{34}-277196662748595114 t^{33}+2144652887215672187 t^{32}+907000505475727811 t^{31}-2390306288524371796 t^{30}-1744770563558737386 t^{29}+1996873987483480255 t^{28}+2452383153011997194 t^{27}-898260466666426838 t^{26}-2495689873780195796 t^{25}-436270062585403914 t^{24}+1608615508319122273 t^{23}+1128045707285667584 t^{22}-369326780838850027 t^{21}-830745772085515016 t^{20}-283990937445944888 t^{19}+220167794190719474 t^{18}+246495339295283383 t^{17}+57379345168221509 t^{16}-53772717452397792 t^{15}-48970024088007261 t^{14}-11779001020521528 t^{13}+6405772208337351 t^{12}+6229128823941968 t^{11}+1926130670767982 t^{10}-169382430496271 t^9-397885443212423 t^8-171956686518163 t^7-36418756224808 t^6-1298855519492 t^5+1613724017440 t^4+532670896103 t^3+87057028685 t^2+7857999933 t+316272243\right)+d^{51} \left(2752 t^{69}+47488 t^{68}+374992 t^{67}+1669392 t^{66}+3816132 t^{65}-1114688 t^{64}-39399557 t^{63}-130397867 t^{62}-151955601 t^{61}+310433533 t^{60}+1546008368 t^{59}+2226275938 t^{58}-1267426570 t^{57}-10091188775 t^{56}-14138962467 t^{55}+4146016035 t^{54}+40849103668 t^{53}+49595532737 t^{52}-13440723157 t^{51}-104971347617 t^{50}-105042712755 t^{49}+31318665672 t^{48}+171674803010 t^{47}+142589868349 t^{46}-41252057541 t^{45}-178869903821 t^{44}-130142727537 t^{43}+26394392035 t^{42}+117526605231 t^{41}+81515157330 t^{40}-3469313698 t^{39}-46432196970 t^{38}-33772852220 t^{37}-4880811365 t^{36}+9524518322 t^{35}+8196287214 t^{34}+2525254255 t^{33}-567779822 t^{32}-908083395 t^{31}-391064622 t^{30}-47566407 t^{29}+35547117 t^{28}+22978200 t^{27}+6219386 t^{26}+398986 t^{25}-352109 t^{24}-161608 t^{23}-38537 t^{22}-5931 t^{21}-596 t^{20}-36 t^{19}-t^{18}\right)+d^8 \left(3176 t^{69}-75500 t^{68}-209322 t^{67}+22424815 t^{66}-271373152 t^{65}+1119445727 t^{64}+4377444768 t^{63}-73753471479 t^{62}+353224283971 t^{61}-490133678993 t^{60}-2762477666047 t^{59}+15328300186910 t^{58}-22038799926013 t^{57}-59144288410080 t^{56}+280131884556474 t^{55}-211276414455358 t^{54}-1078737854124417 t^{53}+2592254368900353 t^{52}+1136628355787841 t^{51}-11095482948023897 t^{50}+6552160273470502 t^{49}+30076156965467164 t^{48}-38278061302954761 t^{47}-62442970271060820 t^{46}+118247646560048842 t^{45}+120688448970471113 t^{44}-274306515041070800 t^{43}-262336669267484932 t^{42}+532628488036501006 t^{41}+635446143936489965 t^{40}-888948604546332380 t^{39}-1477976026666080273 t^{38}+1219941903545114827 t^{37}+2991070297936689660 t^{36}-1177200838267273731 t^{35}-5068732073583352678 t^{34}+249849540417767662 t^{33}+7062846470949729884 t^{32}+1870430462663121851 t^{31}-7895498773594160583 t^{30}-4837821445244115456 t^{29}+6569232063432601878 t^{28}+7444299969424060579 t^{27}-2885025553044402297 t^{26}-7843493320896407459 t^{25}-1643121516940498209 t^{24}+4976083774708147690 t^{23}+3944592031616719926 t^{22}-801948923590048444 t^{21}-2714592059083845954 t^{20}-1210548936328480710 t^{19}+546251007642261812 t^{18}+837977403355534194 t^{17}+281506711364294759 t^{16}-129223179487780152 t^{15}-161997218422832278 t^{14}-53629025825368650 t^{13}+11839032884134210 t^{12}+18358870487148543 t^{11}+7110110194949051 t^{10}+347105736195345 t^9-922018481902831 t^8-489824393271500 t^7-128727196818452 t^6-15808747265178 t^5+1129585009422 t^4+837406497638 t^3+156166860741 t^2+14509435577 t+572476349\right)+d^9 \left(18504 t^{69}-785124 t^{68}+8826666 t^{67}+18773325 t^{66}-1210662889 t^{65}+10847867786 t^{64}-35445740670 t^{63}-90511574436 t^{62}+1299965802350 t^{61}-4768902407573 t^{60}+2934172663365 t^{59}+37661357871701 t^{58}-132173723518455 t^{57}+55656747679117 t^{56}+714442095400309 t^{55}-1654465157211877 t^{54}-886140215746230 t^{53}+8790538305177304 t^{52}-7069986790830770 t^{51}-25946931072739263 t^{50}+47016265468481214 t^{49}+49818391116129948 t^{48}-166051490940412177 t^{47}-68904961073554661 t^{46}+440797022907915500 t^{45}+104838835042317987 t^{44}-996956995008121974 t^{43}-323311247492631423 t^{42}+2020428344381845566 t^{41}+1188090895922394618 t^{40}-3628698388877610716 t^{39}-3509057934876251464 t^{38}+5448014530024634814 t^{37}+8069860585064735442 t^{36}-6117750204546691774 t^{35}-14626030736057574549 t^{34}+3591831747494144864 t^{33}+20932199973551944951 t^{32}+3187749932367657333 t^{31}-23333928792480667451 t^{30}-12610927997848789487 t^{29}+19051185839360812020 t^{28}+20624337437890088847 t^{27}-8067921611929164328 t^{26}-22052444662429626942 t^{25}-5271765282815234509 t^{24}+13722018893446177557 t^{23}+11941259501003019490 t^{22}-1291828110245524799 t^{21}-7650295344052389138 t^{20}-4121704560876322601 t^{19}+1012053742943640173 t^{18}+2354028876814371675 t^{17}+1030541393628144698 t^{16}-197489923346216079 t^{15}-429944971266112025 t^{14}-187404565663309465 t^{13}+2480405359083371 t^{12}+41756488370338796 t^{11}+20945526029774073 t^{10}+3454757978684729 t^9-1366275380508482 t^8-1071442965805525 t^7-347955692214039 t^6-64437082093697 t^5-5502875878326 t^4+369586984078 t^3+157665617711 t^2+17211643906 t+704272531\right)+d^{50} \left(91072 t^{69}+1440576 t^{68}+10239056 t^{67}+39247904 t^{66}+63270228 t^{65}-137341724 t^{64}-1034988437 t^{63}-2368461484 t^{62}-592209681 t^{61}+10607729109 t^{60}+26415782469 t^{59}+11188418086 t^{58}-71612729081 t^{57}-147409409443 t^{56}-7118447650 t^{55}+365365579739 t^{54}+424388182058 t^{53}-382900688430 t^{52}-1277867166856 t^{51}-409095769854 t^{50}+2152396680434 t^{49}+2851676778012 t^{48}-983115819754 t^{47}-5626322523617 t^{46}-4144346819928 t^{45}+3582442290536 t^{44}+8682641130572 t^{43}+4305645815312 t^{42}-4921793570828 t^{41}-8640165705090 t^{40}-3610304157958 t^{39}+3585800559294 t^{38}+5708441210721 t^{37}+2504154330898 t^{36}-1326458950389 t^{35}-2435906976771 t^{34}-1272107172635 t^{33}+110892758386 t^{32}+599999251930 t^{31}+397962684096 t^{30}+84496589150 t^{29}-59523545372 t^{28}-61750478196 t^{27}-25520247544 t^{26}-2900467015 t^{25}+2912240024 t^{24}+2072898710 t^{23}+691581048 t^{22}+97756503 t^{21}-25574227 t^{20}-20543452 t^{19}-7011175 t^{18}-1595240 t^{17}-260807 t^{16}-30691 t^{15}-2493 t^{14}-126 t^{13}-3 t^{12}\right)+d^{49} \left(1449584 t^{69}+20855264 t^{68}+131514152 t^{67}+417658120 t^{66}+325565031 t^{65}-2703800056 t^{64}-11442295776 t^{63}-15798464459 t^{62}+21515375114 t^{61}+119156547076 t^{60}+136564294597 t^{59}-211389502025 t^{58}-753217374007 t^{57}-264595130579 t^{56}+1986838342989 t^{55}+2912999248096 t^{54}-2465502532388 t^{53}-10244278395402 t^{52}-4795937152927 t^{51}+17555665797623 t^{50}+26745858282497 t^{49}-6644593382080 t^{48}-49522847773490 t^{47}-30295489171738 t^{46}+46531701216817 t^{45}+73596430273066 t^{44}-9638447025662 t^{43}-100338402949230 t^{42}-60238336236082 t^{41}+75594914300622 t^{40}+130619238933922 t^{39}+27897852415900 t^{38}-107574727044308 t^{37}-120194356974278 t^{36}-13668153532986 t^{35}+82350618372564 t^{34}+81346711880526 t^{33}+15467106228070 t^{32}-36099719531951 t^{31}-38574034035656 t^{30}-13165745523912 t^{29}+7381826295501 t^{28}+11381736643879 t^{27}+5863835943739 t^{26}+363389937398 t^{25}-1626235507406 t^{24}-1266954752130 t^{23}-447887693515 t^{22}+2035961664 t^{21}+98597660248 t^{20}+62635407690 t^{19}+21696432152 t^{18}+3393599903 t^{17}-938745615 t^{16}-897099899 t^{15}-370079595 t^{14}-105884201 t^{13}-22948797 t^{12}-3850932 t^{11}-497494 t^{10}-48161 t^9-3306 t^8-144 t^7-3 t^6\right)+d^{48} \left(14754136 t^{69}+191277388 t^{68}+1049703334 t^{67}+2583000789 t^{66}-1000353613 t^{65}-25781491593 t^{64}-68511644200 t^{63}-24149311370 t^{62}+278331194526 t^{61}+593079453588 t^{60}-205209853333 t^{59}-2499353161526 t^{58}-2245762976999 t^{57}+6315915851578 t^{56}+14959555705451 t^{55}-2412733207628 t^{54}-44544715391154 t^{53}-39956730092264 t^{52}+63224754358622 t^{51}+138102321053467 t^{50}-12880332979654 t^{49}-264744056845870 t^{48}-167760301484414 t^{47}+335215890089041 t^{46}+530953370758931 t^{45}-106603884586516 t^{44}-853872206471525 t^{43}-546381605569384 t^{42}+597937729491568 t^{41}+1055928968010901 t^{40}+169232444106102 t^{39}-850021646289065 t^{38}-667377312398120 t^{37}+324647657045018 t^{36}+724364075415324 t^{35}+110745884535769 t^{34}-584516173729245 t^{33}-504624420119475 t^{32}+119695658983969 t^{31}+508554423274216 t^{30}+341745683487812 t^{29}-55598321865878 t^{28}-262487901379684 t^{27}-192057339479615 t^{26}-23821698115311 t^{25}+72784223684067 t^{24}+69846128372265 t^{23}+26309769729232 t^{22}-5407276662965 t^{21}-13142033008126 t^{20}-8154719966417 t^{19}-2186217488768 t^{18}+595555917410 t^{17}+952045065566 t^{16}+522293387869 t^{15}+157083323501 t^{14}+5814408382 t^{13}-23247889394 t^{12}-15824298146 t^{11}-6692193112 t^{10}-2139102999 t^9-546177808 t^8-113475557 t^7-19222256 t^6-2630654 t^5-285052 t^4-23617 t^3-1409 t^2-54 t-1\right)+d^{47} \left(107647608 t^{69}+1243485116 t^{68}+5778952410 t^{67}+9555868585 t^{66}-23927194374 t^{65}-147275695912 t^{64}-219363334057 t^{63}+306210354061 t^{62}+1494732158107 t^{61}+753160976026 t^{60}-5403461014459 t^{59}-9774675059404 t^{58}+9375019944805 t^{57}+47065919572986 t^{56}+24463587031515 t^{55}-110055941548327 t^{54}-168837507651653 t^{53}+122660593256451 t^{52}+481488365786785 t^{51}+82829512682245 t^{50}-967923107961643 t^{49}-913920784988581 t^{48}+1102148924926849 t^{47}+2452491086648551 t^{46}+176389200421665 t^{45}-3346244286842214 t^{44}-2504968802644408 t^{43}+2499100145601599 t^{42}+4347008405216366 t^{41}-531444907235517 t^{40}-5442133826734108 t^{39}-2839677215002142 t^{38}+4218935533046334 t^{37}+6325526939302268 t^{36}+963445627236265 t^{35}-4851783853021541 t^{34}-4754660000515256 t^{33}-379537203500279 t^{32}+2670446637138765 t^{31}+2156509792312797 t^{30}+227779512926235 t^{29}-658828495909886 t^{28}-332981508046222 t^{27}+100583935904104 t^{26}+71671664361710 t^{25}-155201087241822 t^{24}-213773029936059 t^{23}-84145202066692 t^{22}+54546130382595 t^{21}+94339881583991 t^{20}+58506353246548 t^{19}+12206174378878 t^{18}-10675869943206 t^{17}-12419304713424 t^{16}-6629718900827 t^{15}-1847396545607 t^{14}+160018365992 t^{13}+496666117065 t^{12}+319686285689 t^{11}+137635237864 t^{10}+45550579067 t^9+12105865134 t^8+2621716355 t^7+462842050 t^6+65952570 t^5+7431226 t^4+639253 t^3+39534 t^2+1568 t+30\right)+d^{46} \left(597824760 t^{69}+6068366116 t^{68}+22916094366 t^{67}+15676503299 t^{66}-164065181065 t^{65}-531740148480 t^{64}-152440012608 t^{63}+2332807004597 t^{62}+3632109492388 t^{61}-6729384129151 t^{60}-25058776025265 t^{59}-3161551790535 t^{58}+90841499246941 t^{57}+112456003986478 t^{56}-159025810350986 t^{55}-440647311986863 t^{54}+89790340318904 t^{53}+1193415158425986 t^{52}+665873148782066 t^{51}-2231788802610203 t^{50}-3150306987528765 t^{49}+1790573004116334 t^{48}+6546327505288634 t^{47}+1317896565289892 t^{46}-8800686735868300 t^{45}-6289175831488124 t^{44}+9591767807957253 t^{43}+14761952962197188 t^{42}-3454053542368891 t^{41}-21414599961737338 t^{40}-12352457581052035 t^{39}+11901863652482734 t^{38}+18768729834124129 t^{37}+3421917775459257 t^{36}-8626624323964534 t^{35}-3111451865520202 t^{34}+5587578388944748 t^{33}+1768920002848873 t^{32}-8412227675414738 t^{31}-9794318057121714 t^{30}-653589290827035 t^{29}+7749808217025000 t^{28}+7556759889066549 t^{27}+1779362957407139 t^{26}-2625474415658031 t^{25}-2942111916003791 t^{24}-1134675276657292 t^{23}+244419890102746 t^{22}+489862222308181 t^{21}+202849404735306 t^{20}-16780164696449 t^{19}-43553410549639 t^{18}+2485959069347 t^{17}+27167249541728 t^{16}+21112572614230 t^{15}+7039567502409 t^{14}-1200472715078 t^{13}-3009042438604 t^{12}-2103949709982 t^{11}-987000074658 t^{10}-353685279064 t^9-101086772785 t^8-23398339328 t^7-4391243727 t^6-662042445 t^5-78595545 t^4-7096992 t^3-459176 t^2-18995 t-378\right)+d^{45} \left(2616588792 t^{69}+22935910492 t^{68}+65648413230 t^{67}-40668989027 t^{66}-669237454695 t^{65}-1119669409193 t^{64}+1847087855946 t^{63}+7643924510843 t^{62}-1579250379138 t^{61}-40335348900148 t^{60}-42760120162258 t^{59}+106449257360420 t^{58}+251837543072450 t^{57}-112991909065460 t^{56}-806139434497489 t^{55}-185389391128298 t^{54}+2148268889234755 t^{53}+2077972852692352 t^{52}-3447648292448453 t^{51}-6573692967338846 t^{50}+2545673439727663 t^{49}+12412833057134554 t^{48}+207863923601632 t^{47}-22232016007747418 t^{46}-11773108182248598 t^{45}+29635447928981304 t^{44}+36563861056396950 t^{43}-14315542344385544 t^{42}-46429851241825432 t^{41}-3349077208684957 t^{40}+43347202440453345 t^{39}+4877487684533577 t^{38}-66253712332484590 t^{37}-48377121451659168 t^{36}+52933500584015775 t^{35}+104446824631613871 t^{34}+39134575829160505 t^{33}-57684216651566327 t^{32}-78159900658673551 t^{31}-24481299407995296 t^{30}+25390762923562606 t^{29}+28099817427198539 t^{28}+5832156228538332 t^{27}-6303387469186605 t^{26}-2297723271082539 t^{25}+3912195768037282 t^{24}+3624341914589009 t^{23}-330918116911941 t^{22}-2629234889594444 t^{21}-2092686743559495 t^{20}-586687062559187 t^{19}+307639029054676 t^{18}+411648193717332 t^{17}+205481995678689 t^{16}+41569709754647 t^{15}-12467335500308 t^{14}-11274744183192 t^{13}-1818080242248 t^{12}+2009669373497 t^{11}+1878596012278 t^{10}+930816297545 t^9+328078198294 t^8+88628199198 t^7+18797163157 t^6+3135800834 t^5+405830413 t^4+39506807 t^3+2731916 t^2+119949 t+2519\right)+d^{18} \left(5249873088 t^{69}-134780545664 t^{68}+1459042368288 t^{67}-7432459820816 t^{66}+4234367537472 t^{65}+163433190908566 t^{64}-847514627222247 t^{63}+840678633628427 t^{62}+7032632792423859 t^{61}-24362612905635118 t^{60}-9386262865060374 t^{59}+183624199892222483 t^{58}-182162658236281540 t^{57}-796140516350128419 t^{56}+1579275198541750687 t^{55}+2342050250136342438 t^{54}-7545353453008535717 t^{53}-5147724658090759224 t^{52}+26417959464956079957 t^{51}+10114951949171930418 t^{50}-74809615445855928956 t^{49}-25379204225165721051 t^{48}+178751568229848417532 t^{47}+86989048268905213416 t^{46}-361099883890961736301 t^{45}-294759607060279695512 t^{44}+587018321395493400462 t^{43}+829113935726668124207 t^{42}-639025454237038138038 t^{41}-1844153211695589940181 t^{40}-20649371322374156638 t^{39}+3097138273913407773812 t^{38}+2110064982272410204461 t^{37}-3397254443458703096498 t^{36}-5618302848926372958454 t^{35}+673598528661392819296 t^{34}+8180872173777061566296 t^{33}+5802706704556037330202 t^{32}-4970028812396017257690 t^{31}-11059210054247835529211 t^{30}-5152961461277396648470 t^{29}+5671237082885817220554 t^{28}+10214561856323464436513 t^{27}+5987651322399279550234 t^{26}-835649792026208163482 t^{25}-4157400973652415459375 t^{24}-3230601930907863255347 t^{23}-855907917013354441236 t^{22}+574318287288935695120 t^{21}+671827932292639712149 t^{20}+209485746722116109052 t^{19}-126532297706452842128 t^{18}-177380740000816083262 t^{17}-89725967783019475961 t^{16}-10514314828140733678 t^{15}+17801454061817247883 t^{14}+15190820212297195104 t^{13}+6427363902549360302 t^{12}+1319181565004930164 t^{11}-206082121025462543 t^{10}-288413971952878081 t^9-129292644482804166 t^8-37555129204066306 t^7-7755110169109965 t^6-1135634948366454 t^5-109536755022691 t^4-5216581354820 t^3+149651416386 t^2+35015845711 t+1451668067\right)+d^{44} \left(9205866272 t^{69}+68133582744 t^{68}+128516271560 t^{67}-363219265966 t^{66}-1783313974298 t^{65}-555851168037 t^{64}+8923982685497 t^{63}+10429309252371 t^{62}-38622364067760 t^{61}-94247329279146 t^{60}+55220071665598 t^{59}+367889073802796 t^{58}+52146763191793 t^{57}-1132910992922915 t^{56}-743622168425460 t^{55}+3004000049542327 t^{54}+3991590920130297 t^{53}-4652604960433708 t^{52}-10189910479883214 t^{51}+7115072924135094 t^{50}+24535491671291480 t^{49}-6757175305763179 t^{48}-56417408810162576 t^{47}-21575967699461975 t^{46}+78843806963495252 t^{45}+66231953533276761 t^{44}-88850630321542671 t^{43}-122919020481252056 t^{42}+102474284044856445 t^{41}+266154550799013618 t^{40}+37545310023570051 t^{39}-332850658804406415 t^{38}-323681132738395079 t^{37}+70048575631788743 t^{36}+332387534405690859 t^{35}+187614454321327986 t^{34}-77487639319204794 t^{33}-119825305345256961 t^{32}+7227123267543735 t^{31}+55603619485626674 t^{30}-26141647154040314 t^{29}-91370877843995057 t^{28}-52283744021913914 t^{27}+27093013202909111 t^{26}+57382334369490107 t^{25}+31559364587287102 t^{24}-2456209802287631 t^{23}-13611804543307863 t^{22}-7230875300834205 t^{21}+214389696299360 t^{20}+1951034111252824 t^{19}+459321692292100 t^{18}-742900533957762 t^{17}-773440741114033 t^{16}-320261991537586 t^{15}+4982632092809 t^{14}+94905957354301 t^{13}+70215048179942 t^{12}+31559780718044 t^{11}+9963862150481 t^{10}+2188062736872 t^9+270971454629 t^8-15042046352 t^7-17056712574 t^6-4696854798 t^5-809575570 t^4-95925316 t^3-7690413 t^2-379864 t-8794\right)+d^{19} \left(25410706752 t^{69}-580785331136 t^{68}+5779084359600 t^{67}-30064404592336 t^{66}+58995814941332 t^{65}+235874750703018 t^{64}-1792776396000978 t^{63}+3094140576114971 t^{62}+9532685939377555 t^{61}-47248479409524046 t^{60}+14851742413116218 t^{59}+284807736529699941 t^{58}-436850251918321779 t^{57}-1018834542684120265 t^{56}+2859142677193297921 t^{55}+2337661765153334046 t^{54}-12049832212149238215 t^{53}-3268995449034512531 t^{52}+39092045292640950672 t^{51}+2530242868804951193 t^{50}-105674892066333213733 t^{49}-7533372336637605836 t^{48}+246974872127590025757 t^{47}+62051094853408934333 t^{46}-499548362878046694381 t^{45}-294673036846993205522 t^{44}+838742153679584840208 t^{43}+949346996701763589826 t^{42}-1025243789699850773330 t^{41}-2277304406278619941398 t^{40}+410244672369953898976 t^{39}+4116017249886277233498 t^{38}+1997091924710772994795 t^{37}-5171284325824722605742 t^{36}-6607409500572570280458 t^{35}+2744477483603016892994 t^{34}+11204205387190008943712 t^{33}+5301854256712000883897 t^{32}-9460914000158960487949 t^{31}-14686081726401850215180 t^{30}-3709777799909682848100 t^{29}+10895715226965476009048 t^{28}+14660861915744874900895 t^{27}+6973997448574804567800 t^{26}-2505820252998685529093 t^{25}-6383799904306743674971 t^{24}-4770174412102893483200 t^{23}-1556711468498692438699 t^{22}+449299664554669814808 t^{21}+846270092534850147501 t^{20}+454360797057108021896 t^{19}+36156132606167608230 t^{18}-133893048835379740946 t^{17}-116970910436008043809 t^{16}-48683754278869222379 t^{15}-3759162598779052218 t^{14}+9394297922302411468 t^{13}+7312119721942229660 t^{12}+3040911463858981210 t^{11}+723757549019584280 t^{10}+20328249120259597 t^9-64580114932004962 t^8-32098600417592848 t^7-9408652042976062 t^6-1950779640663294 t^5-297069808122416 t^4-32956189074664 t^3-2548911271036 t^2-124000882230 t-2876443576\right)+d^{43} \left(26243598368 t^{69}+159195316736 t^{68}+130472055968 t^{67}-1269729874936 t^{66}-2937574808138 t^{65}+4454640679106 t^{64}+19295269568013 t^{63}-13093636068843 t^{62}-114850820719821 t^{61}-47981018313838 t^{60}+371887272188066 t^{59}+270305114856708 t^{58}-1289259232622107 t^{57}-1480655406456632 t^{56}+3550149431418853 t^{55}+6008040631113517 t^{54}-7047642164575274 t^{53}-16424133741512954 t^{52}+16859190309456784 t^{51}+53717097637658195 t^{50}-10516066495886797 t^{49}-121121154002693672 t^{48}-43301277943297947 t^{47}+191197916960320612 t^{46}+138321959126906472 t^{45}-300276057438612825 t^{44}-423249066341124463 t^{43}+211043776657710838 t^{42}+781617315251775980 t^{41}+332103740908155501 t^{40}-570682459411261371 t^{39}-627419813747046905 t^{38}+96698739867999107 t^{37}+347764185611004741 t^{36}-190640990689249203 t^{35}-464656021645220357 t^{34}+109870907368458591 t^{33}+726326181951589010 t^{32}+519268410378898777 t^{31}-195267714028706673 t^{30}-541004141822558485 t^{29}-288683433222886797 t^{28}+82133342469374313 t^{27}+171437316311844320 t^{26}+46143373335108136 t^{25}-49850880572689452 t^{24}-33896721403331526 t^{23}+17771820073333480 t^{22}+34012121352535965 t^{21}+16667312624870118 t^{20}-2418449651050930 t^{19}-8061182808299155 t^{18}-4900965020580836 t^{17}-1086960803229432 t^{16}+394847103276248 t^{15}+352415904772197 t^{14}+34461753743671 t^{13}-98023046917859 t^{12}-86047668261603 t^{11}-43028524081906 t^{10}-15397003482978 t^9-4193776958967 t^8-883810838754 t^7-142926057307 t^6-17151250163 t^5-1407762399 t^4-61126108 t^3+892333 t^2+260459 t+10072\right)+d^{23} \left(35352261616 t^{69}+2853975605448 t^{68}-49291729601476 t^{67}+261691028810894 t^{66}-68576605768518 t^{65}-4326602900377178 t^{64}+12605493272049925 t^{63}+19274389876276010 t^{62}-144823680356024184 t^{61}+60453693244712223 t^{60}+870351654986861987 t^{59}-1198467024655511936 t^{58}-3421505502910808116 t^{57}+7776263102152473260 t^{56}+9561190091168837812 t^{55}-33392665636095594054 t^{54}-19629111179187437961 t^{53}+110021580158986335802 t^{52}+30053209332101904773 t^{51}-297340963403468645732 t^{50}-37699101649150753785 t^{49}+683961342684848416975 t^{48}+63359495664814670515 t^{47}-1365681419225973493920 t^{46}-197824410097902257307 t^{45}+2381591127088917489632 t^{44}+642139113754977711690 t^{43}-3600666518813207191027 t^{42}-1671015208933814702973 t^{41}+4606777409976103424137 t^{40}+3471177248017859186816 t^{39}-4650009517816402042483 t^{38}-5834484093633271728902 t^{37}+2725773462625250495010 t^{36}+7525815868532298141981 t^{35}+1456841272409457408318 t^{34}-6723202190117125507923 t^{33}-7764343041103024514501 t^{32}-1856925017389493646682 t^{31}+7241278167197813269069 t^{30}+15842395882303742926477 t^{29}+18107343832820365580407 t^{28}+9843056523609915759888 t^{27}-4518113011322468925691 t^{26}-14704945940342280374568 t^{25}-15032302497598278027894 t^{24}-8721444613542815868922 t^{23}-2376226757442947098356 t^{22}+597964691830496552313 t^{21}+884844328639154419676 t^{20}+380932315327546784141 t^{19}+83538304629475846615 t^{18}+39331960574385109575 t^{17}+49465770381875004526 t^{16}+33836392486729385804 t^{15}+9084838308799806593 t^{14}-3953829504570824200 t^{13}-5479204161795929901 t^{12}-3068795748240798047 t^{11}-1093336446873066282 t^{10}-250816633833380533 t^9-25160954872025040 t^8+6517623703457379 t^7+3851810487497881 t^6+1027223462707558 t^5+181437835468615 t^4+22405711427302 t^3+1886810444363 t^2+98359584331 t+2410502066\right)+d^{42} \left(60302580384 t^{69}+288087852944 t^{68}-108210341996 t^{67}-2718530737748 t^{66}-1860071268899 t^{65}+14818879258082 t^{64}+14514944835875 t^{63}-79753691696458 t^{62}-120811625887437 t^{61}+253990901707431 t^{60}+405400963659962 t^{59}-1232775498938141 t^{58}-2188145370668496 t^{57}+3745426877315369 t^{56}+8413703856896719 t^{55}-10229885261340975 t^{54}-29323627340481162 t^{53}+22943708011707024 t^{52}+100625159513497866 t^{51}+5116316094264615 t^{50}-209803885574401038 t^{49}-86555999044495760 t^{48}+394595417881294811 t^{47}+338777186890246603 t^{46}-586342788737892485 t^{45}-971255421588562213 t^{44}+201512807503962868 t^{43}+1244446295964329363 t^{42}+276210837299828520 t^{41}-1080008492839357857 t^{40}-116188139797590699 t^{39}+1832565279727712304 t^{38}+1087400396726843422 t^{37}-1982425153366755983 t^{36}-2998242027149815866 t^{35}-369550783362901378 t^{34}+2351992767986690991 t^{33}+1966554851649570696 t^{32}-193632242416304252 t^{31}-1096332849237251654 t^{30}-283355000254766301 t^{29}+492269378730638392 t^{28}+251587721472306616 t^{27}-337499714483537025 t^{26}-441901459563251928 t^{25}-110585041987103180 t^{24}+161670835662251597 t^{23}+164867731751675582 t^{22}+43721797079830629 t^{21}-29064595855323920 t^{20}-25941425993791819 t^{19}-490710315068029 t^{18}+10528341308783491 t^{17}+7192071019090814 t^{16}+1299786151248905 t^{15}-1377952301170156 t^{14}-1402503994680869 t^{13}-706610608619236 t^{12}-226381198805320 t^{11}-41044451832413 t^{10}+1368240741656 t^9+3871712559223 t^8+1520089762668 t^7+373801037874 t^6+65700561153 t^5+8441937366 t^4+777554242 t^3+48460604 t^2+1807549 t+29577\right)+d^{20} \left(64525585152 t^{69}-1313165351968 t^{68}+11765089701360 t^{67}-58178701622792 t^{66}+138258909699900 t^{65}+166913131222742 t^{64}-2381959894036534 t^{63}+6099571536378283 t^{62}+5832382649824852 t^{61}-63043286582933453 t^{60}+72299686219597872 t^{59}+292047429679891745 t^{58}-758424617516063523 t^{57}-712569519733271093 t^{56}+3963821683055117607 t^{55}+364309869333807378 t^{54}-14678524597032168441 t^{53}+4197684296508614735 t^{52}+43590416513906310036 t^{51}-18355110503260659669 t^{50}-111239908774527918535 t^{49}+39434067626773862876 t^{48}+252487181584668305804 t^{47}-26539025835391074070 t^{46}-508588942015528352343 t^{45}-152112258634549189983 t^{44}+870703192852074102109 t^{43}+758077394835315518711 t^{42}-1130759331387505237292 t^{41}-2096424656573679053320 t^{40}+671845919257359666486 t^{39}+4140423985366913826128 t^{38}+1560854947523352661196 t^{37}-5815609271934899461256 t^{36}-6377513336912195316508 t^{35}+4418659280954663954726 t^{34}+12453549507826248167748 t^{33}+3420942454945777484834 t^{32}-13652919682750332345021 t^{31}-16488163274507120751514 t^{30}-45142841815667325626 t^{29}+17440418271144902743449 t^{28}+18821389875998079765282 t^{27}+6463702424485779043317 t^{26}-5723891404705022561565 t^{25}-9331900424955564287756 t^{24}-6251045535073343058055 t^{23}-2011184878100604348599 t^{22}+357337679856966400118 t^{21}+876769277468533029333 t^{20}+580945104995698150638 t^{19}+194642655259005538946 t^{18}-29229024905320393244 t^{17}-89940305499429872094 t^{16}-65850575993459781057 t^{15}-26735681939693167298 t^{14}-3455102649889307293 t^{13}+3451171596837020535 t^{12}+2966001317383299963 t^{11}+1311357893911350236 t^{10}+376175877362255575 t^9+64171416975802891 t^8+817462656825555 t^7-3308936730837989 t^6-1161854119237242 t^5-235845406735764 t^4-32151839043649 t^3-2935080943843 t^2-164184053362 t-4291410666\right)+d^{39} \left(78361109272 t^{69}+258981860996 t^{68}+662106847390 t^{67}+2470090239087 t^{66}-12942979582141 t^{65}-65962208568918 t^{64}+84920649292117 t^{63}+619803278259890 t^{62}-342004056828350 t^{61}-4188670528714107 t^{60}-629082204666001 t^{59}+18282396036664781 t^{58}+7475916837684908 t^{57}-70969722504257197 t^{56}-56252543934671075 t^{55}+196788263319547963 t^{54}+201257126836627814 t^{53}-506926690429048674 t^{52}-641430006847405017 t^{51}+1122106246305946107 t^{50}+1881923084838152073 t^{49}-1641742227082890444 t^{48}-3695590917216541916 t^{47}+3152239616197101414 t^{46}+9229023645328444445 t^{45}-825297872312621926 t^{44}-14670043469501317158 t^{43}-5996816017215491827 t^{42}+13381282449676099656 t^{41}+5499994740871308521 t^{40}-21296983914280582499 t^{39}-16011730091176029047 t^{38}+23809218727226170090 t^{37}+36922560128148963768 t^{36}-1537424682842725578 t^{35}-36446237013918446493 t^{34}-20845235782653965301 t^{33}+15317785394604805610 t^{32}+20953077138439679364 t^{31}-1152017657167349769 t^{30}-13090219050196697466 t^{29}-2815480316771225658 t^{28}+9038658596151051628 t^{27}+7161736012051037385 t^{26}-1544607649676399120 t^{25}-5125789966815326718 t^{24}-2340493810653572345 t^{23}+976628447697135969 t^{22}+1491568379751324863 t^{21}+345633661701833046 t^{20}-468761928355987811 t^{19}-457574567777724625 t^{18}-140127622715844180 t^{17}+50164126436586376 t^{16}+68771309140860579 t^{15}+28033925699291152 t^{14}-134290497745391 t^{13}-6954542052925362 t^{12}-4782242731284415 t^{11}-2000764041914215 t^{10}-602092154062552 t^9-135619940450357 t^8-22699377555805 t^7-2665232904444 t^6-177442973303 t^5+2595507432 t^4+2021919396 t^3+219854570 t^2+11562315 t+253852\right)+d^{41} \left(108585228232 t^{69}+388262784892 t^{68}-659427279206 t^{67}-3478695001963 t^{66}+3314978757987 t^{65}+18229072055844 t^{64}-28298214733525 t^{63}-105022110220534 t^{62}+142492545733221 t^{61}+404932451409760 t^{60}-1119828030249924 t^{59}-2784215591654877 t^{58}+3616890467146181 t^{57}+11730985674861052 t^{56}-11235842427391122 t^{55}-47846442614234455 t^{54}+14608124725725083 t^{53}+150487916055940968 t^{52}+42521023464539865 t^{51}-316462681598854349 t^{50}-170395114500675382 t^{49}+679246090271140945 t^{48}+707677753688760254 t^{47}-874240615450456458 t^{46}-1545769720133598537 t^{45}+619538521934034288 t^{44}+2037441899062242600 t^{43}-1042629595171617936 t^{42}-4110248604644528713 t^{41}-375280617260043501 t^{40}+6204954071248349962 t^{39}+5238571963089573202 t^{38}-2916187868453580049 t^{37}-6750101521277157608 t^{36}-1748716800922945565 t^{35}+3400722035004938908 t^{34}+1675966749902501015 t^{33}-2304803662183494752 t^{32}-1642107553737815323 t^{31}+2167144403491703384 t^{30}+3265070982581616012 t^{29}+623721881573636869 t^{28}-1860370382545387325 t^{27}-1681851964838228000 t^{26}-137399986094636977 t^{25}+651504548770652309 t^{24}+347770939480166866 t^{23}-145755484671424846 t^{22}-243534467834464832 t^{21}-70973094766954396 t^{20}+67337910194096050 t^{19}+77705933024234684 t^{18}+31487175625396193 t^{17}-1147377612738282 t^{16}-7718919969004383 t^{15}-3368469908365770 t^{14}+360003140652392 t^{13}+1259917604423850 t^{12}+851115418208235 t^{11}+363642956429157 t^{10}+112977365398455 t^9+26427023499235 t^8+4614949675212 t^7+567993645465 t^6+39868803746 t^5-601691674 t^4-509141826 t^3-59440540 t^2-3384698 t-81415\right)+d^{21} \left(110052187360 t^{69}-1810222166144 t^{68}+12697287935896 t^{67}-53783963792016 t^{66}+172007740127300 t^{65}-316044174155970 t^{64}-1052613660178633 t^{63}+8823798847818022 t^{62}-14304143129614917 t^{61}-49550259341166171 t^{60}+195666222135448060 t^{59}+56423750000000305 t^{58}-1174321460132839286 t^{57}+772199436617691264 t^{56}+4632572315436218834 t^{55}-5769666140054454369 t^{54}-13793249115870552178 t^{53}+23521243729926404292 t^{52}+34004847566016132543 t^{51}-68636543995585658468 t^{50}-75458994913810397290 t^{49}+153765425761021255555 t^{48}+160169715475800926018 t^{47}-263476261840128599138 t^{46}-325775140521137549972 t^{45}+306350163991738014024 t^{44}+596455187337195904514 t^{43}-68944139213467682129 t^{42}-878417487167070462090 t^{41}-751443075926960513184 t^{40}+784241054128487178522 t^{39}+2324520721749932407592 t^{38}+501934900229008851348 t^{37}-4172343131106745078370 t^{36}-3999524927441603797597 t^{35}+4451076540479429514035 t^{34}+9816306185093049979038 t^{33}+346585563070581348419 t^{32}-14659424586496127710112 t^{31}-14026020171096547183181 t^{30}+5283870328597896639318 t^{29}+22718934139117399585804 t^{28}+20715748235412377768455 t^{27}+4194134374927716919740 t^{26}-9873004219108521152539 t^{25}-12546752573724365269958 t^{24}-7553810448916685416998 t^{23}-2147287413129493013762 t^{22}+428420817626364928126 t^{21}+838865266163837248172 t^{20}+546142107327908126688 t^{19}+252266490789885351333 t^{18}+71577672880056161391 t^{17}-19993416147631052905 t^{16}-45398169015023297919 t^{15}-33807053650098099762 t^{14}-14842810104615057397 t^{13}-3195029614670524631 t^{12}+677728337183687687 t^{11}+940720355219435478 t^{10}+461737756036508363 t^9+148834794423217218 t^8+34385934765818734 t^7+5654692545828868 t^6+599772405138588 t^5+23400472976722 t^4-4015645024220 t^3-786656250512 t^2-60211658842 t-1873779098\right)+d^{22} \left(119236397648 t^{69}-853590766744 t^{68}-4142427571660 t^{67}+42551238295270 t^{66}+88571395171506 t^{65}-1677497186139472 t^{64}+3951340741027248 t^{63}+11838667372000681 t^{62}-63564027489388378 t^{61}+2683784302373461 t^{60}+445938699128313611 t^{59}-502564173497330054 t^{58}-1930093338163684758 t^{57}+3849544883711824877 t^{56}+5768647735344747421 t^{55}-17762943503650157051 t^{54}-12439822589232885366 t^{53}+60584638536485355323 t^{52}+19624622741527490475 t^{51}-165563554089866840535 t^{50}-23928305725367166167 t^{49}+377899000895544144023 t^{48}+33970747286348580435 t^{47}-734979378261970470279 t^{46}-95203918599235686629 t^{45}+1220283975244511644776 t^{44}+303093237306310989631 t^{43}-1695011409904916728096 t^{42}-755590103716421407824 t^{41}+1849893943729179986176 t^{40}+1414398610721900843887 t^{39}-1237136236829741367357 t^{38}-1860172804908616032298 t^{37}-488330498675652018231 t^{36}+1008267177242945618267 t^{35}+2808013626723041294201 t^{34}+2564684940651639344833 t^{33}-3563904306435438436906 t^{32}-10348902967486545155492 t^{31}-5673752538149006688240 t^{30}+11012021490103224954387 t^{29}+23446682696789481544894 t^{28}+18057582941781394433183 t^{27}+386678949955469130806 t^{26}-13383834145528455966228 t^{25}-14904737891311401472198 t^{24}-8515127249783897625509 t^{23}-2181403118949232722033 t^{22}+602400025399282933544 t^{21}+845699281278280074667 t^{20}+435551743646125321900 t^{19}+186393516726371234866 t^{18}+96799215081781038076 t^{17}+42382856987705498758 t^{16}+12670071564422519 t^{15}-17580930125373442994 t^{14}-15271893522816436509 t^{13}-7432775593005366975 t^{12}-2166211037835950109 t^{11}-194552118872438247 t^{10}+163416352904853815 t^9+105283526903010035 t^8+36663352943442955 t^7+8971519349329573 t^6+1633624460733654 t^5+222956151165572 t^4+22349694803347 t^3+1565138870165 t^2+68900898253 t+1448278747\right)+d^{40} \left(139695087368 t^{69}+363828047140 t^{68}-942224327490 t^{67}-1484612581109 t^{66}+6305022825028 t^{65}-10340853843271 t^{64}-63624120950812 t^{63}+125923563131222 t^{62}+460745189351467 t^{61}-965846404871646 t^{60}-3571779440639461 t^{59}+2593602416351214 t^{58}+15962219593195681 t^{57}-6142671905001506 t^{56}-65538188426261405 t^{55}-12343455786654695 t^{54}+188819218921245119 t^{53}+104122990881852144 t^{52}-435273695934821734 t^{51}-346681752883003030 t^{50}+973019455858133297 t^{49}+1235587445419989425 t^{48}-1238940800682464198 t^{47}-2305820154769234633 t^{46}+1889034427563235684 t^{45}+4706940861699212932 t^{44}-2007287519099391169 t^{43}-9852057948737956005 t^{42}-3932364290078163487 t^{41}+9247522009749279412 t^{40}+8795040639734393400 t^{39}-4303573581110238095 t^{38}-7124377462801564200 t^{37}+5045313653874199585 t^{36}+9810188061124643868 t^{35}-3300855814761105556 t^{34}-14672321248070615776 t^{33}-7088311234621202785 t^{32}+8155044572517774085 t^{31}+11191843851027757756 t^{30}+1905224436916565714 t^{29}-5212211490074410997 t^{28}-3411304067030694212 t^{27}+1298528455794259480 t^{26}+2351832027495987623 t^{25}+259820755946071606 t^{24}-1297717115244350431 t^{23}-1001302236946349236 t^{22}-60566360854909899 t^{21}+355119990846928607 t^{20}+218464930117341452 t^{19}-5860830664866473 t^{18}-77958395425002060 t^{17}-42212230018892215 t^{16}+1007159420393508 t^{15}+15375073666141789 t^{14}+11544277769548439 t^{13}+4984469555527206 t^{12}+1344042185389183 t^{11}+153874642783771 t^{10}-50389932766530 t^9-34373568725870 t^8-10940109585528 t^7-2369750071098 t^6-374089048578 t^5-43249695104 t^4-3557168078 t^3-194615693 t^2-6163993 t-79439\right)+d^{27} \left(327557338560 t^{69}+5696044150080 t^{68}-118726366963680 t^{67}+570155107886400 t^{66}+153021675664140 t^{65}-8229958985314098 t^{64}+12995162548241589 t^{63}+55355775315764676 t^{62}-151201766155757376 t^{61}-244724301092180279 t^{60}+994295803373908828 t^{59}+839440995196586931 t^{58}-4810651569387532633 t^{57}-2576823280405302586 t^{56}+18817373699503992944 t^{55}+8079742682917207852 t^{54}-61953814702949210021 t^{53}-27079786894456385599 t^{52}+174352773148353730200 t^{51}+90844524078557787603 t^{50}-420214527224141822159 t^{49}-279808616898918586864 t^{48}+861011918193373197643 t^{47}+752376667054786051139 t^{46}-1471509864429877679180 t^{45}-1724991842441803391396 t^{44}+2010366880870540657359 t^{43}+3317806180564095497204 t^{42}-2002170868575916301296 t^{41}-5401019316752093392552 t^{40}+655459115274241879536 t^{39}+6864227911078771913140 t^{38}+1854365439547262101857 t^{37}-6672283220777186288716 t^{36}-4352508128726338923005 t^{35}+5447108394509981741718 t^{34}+8743488521601129236597 t^{33}+4541611279481748987700 t^{32}+3040742742741850441256 t^{31}+5738166310600889521755 t^{30}+3825542893416542228335 t^{29}-5462417463871975343328 t^{28}-13770593176963479546307 t^{27}-13696668461842697450908 t^{26}-7448156603298575725534 t^{25}-1810261269366709005618 t^{24}+49922058667830085052 t^{23}-360632369933017317662 t^{22}-755678308953372499812 t^{21}-503089147915160171828 t^{20}-87725528076613996199 t^{19}+96754683585577991867 t^{18}+74852799143594847716 t^{17}+9836773791819878651 t^{16}-18215236472924757424 t^{15}-15253564405869851021 t^{14}-5737874852030078345 t^{13}-492893562140663541 t^{12}+746950956971385809 t^{11}+537114336750280352 t^{10}+216976678197173570 t^9+62176659024590551 t^8+13323268837475147 t^7+2138035249633552 t^6+247651756876088 t^5+18542458512939 t^4+544982764089 t^3-45466036858 t^2-5449170619 t-182023047\right)+d^{32} \left(870113432688 t^{69}-16703630718408 t^{68}+54472822488076 t^{67}+192726540957394 t^{66}-1022043395347710 t^{65}-1047990324896180 t^{64}+9298364155941484 t^{63}+3719774143807129 t^{62}-58923660434244432 t^{61}-9585523188277530 t^{60}+294237643226018887 t^{59}+12402573997977125 t^{58}-1216298141457454424 t^{57}+60234672848078783 t^{56}+4267199879857726733 t^{55}-591893336379810155 t^{54}-13005508090793840464 t^{53}+2746576069498441822 t^{52}+34886408421279382848 t^{51}-9348864887250221452 t^{50}-85380052412482765536 t^{49}+20344892214881653070 t^{48}+185669292711442568462 t^{47}-34113739082338828355 t^{46}-379409977938580761942 t^{45}-5440901892170612849 t^{44}+658541385016882666282 t^{43}+165115374847423641627 t^{42}-923804230069248546789 t^{41}-325840095317662830325 t^{40}+1518048708783184530503 t^{39}+1405178979780935741350 t^{38}-836328620426203009323 t^{37}-1420436182699431090531 t^{36}+810048538798351425815 t^{35}+2051678935809277486231 t^{34}-101498336930208555741 t^{33}-2776213054221232482791 t^{32}-2650158948748916479732 t^{31}-717839090398200945507 t^{30}+160148331015797159435 t^{29}-413620043437423167957 t^{28}-775781166744011820697 t^{27}-192255706530703284736 t^{26}+506171259404062886073 t^{25}+557190057803254770305 t^{24}+166017635643526895700 t^{23}-115976726952049271612 t^{22}-114089548058710478646 t^{21}-2384488755474102074 t^{20}+53307466946112148807 t^{19}+38480926949986255949 t^{18}+7498274455291620887 t^{17}-7226016907034526348 t^{16}-7065778440704115299 t^{15}-2891076880124297578 t^{14}-305008874020155596 t^{13}+382321130276825804 t^{12}+297640838103493183 t^{11}+127323984984684979 t^{10}+38464580000406757 t^9+8657883186258990 t^8+1443979217761802 t^7+166911896050501 t^6+10034412020012 t^5-510210145994 t^4-189909508775 t^3-20939467109 t^2-1197985286 t-29956777\right)+d^{28} \left(1302148710720 t^{69}-11059496633520 t^{68}-12822957485040 t^{67}+349862457956988 t^{66}-587377793396940 t^{65}-3344360455846776 t^{64}+8882984604408306 t^{63}+19989953709997139 t^{62}-63550256348323684 t^{61}-112217452888187725 t^{60}+318381811694860628 t^{59}+663092792005667781 t^{58}-1321036991021700237 t^{57}-3578610243190841039 t^{56}+4819745776548761325 t^{55}+16077567698466942302 t^{54}-15152282979833197757 t^{53}-59463213878176362109 t^{52}+38751772851617713280 t^{51}+183495793611663614635 t^{50}-73098965011010361368 t^{49}-478060510747431701456 t^{48}+72146089406801503595 t^{47}+1055481448580386631680 t^{46}+108575723201160385487 t^{45}-1968283097387607074063 t^{44}-751033600566145523716 t^{43}+3007486951647526169386 t^{42}+2063753452847716078728 t^{41}-3788026779744043548095 t^{40}-4267494776288729928152 t^{39}+3315161818543116484254 t^{38}+6710266637443809154667 t^{37}-589758798340025036474 t^{36}-6629414501556105454443 t^{35}-482946176923655476218 t^{34}+9755374956793392769467 t^{33}+10464651834055342684352 t^{32}+2401983776591931215012 t^{31}-4122526198311973269007 t^{30}-5459498451894332745023 t^{29}-5866926005542892666907 t^{28}-7544125097731601692521 t^{27}-7879488865582506196218 t^{26}-5164183564267922515549 t^{25}-1460163074058546088763 t^{24}+537610585573500085939 t^{23}+515113063089566909827 t^{22}-145864544886678947977 t^{21}-411151560014942925396 t^{20}-252249070936410243422 t^{19}-35570867868972683512 t^{18}+49508274878993617278 t^{17}+36371543648122620503 t^{16}+6175235126299844220 t^{15}-6928564791256577520 t^{14}-6575579442412998327 t^{13}-3048887868907810054 t^{12}-835402328136239661 t^{11}-77855012102476265 t^{10}+48617425242316922 t^9+30319011196181725 t^8+9984601177201859 t^7+2313140149708856 t^6+400833569551082 t^5+52404687239067 t^4+5068445552505 t^3+344857230991 t^2+14831605261 t+305062633\right)+d^{31} \left(2151998827248 t^{69}-30055805151336 t^{68}+96543240083076 t^{67}+266119430419818 t^{66}-1803443292313840 t^{65}-148380924153238 t^{64}+14984114705007229 t^{63}-11317194227896552 t^{62}-81240305158396666 t^{61}+103681806981301109 t^{60}+327012432691765589 t^{59}-574252033181919020 t^{58}-1028503150072505456 t^{57}+2434536138429811756 t^{56}+2565610023248541042 t^{55}-8618487827666343503 t^{54}-5078389617733680951 t^{53}+26563600963805740711 t^{52}+8119481178046242078 t^{51}-73023634485593457479 t^{50}-13733316423653325397 t^{49}+177366725991564384413 t^{48}+33546661302969472236 t^{47}-386138754042466518000 t^{46}-126708572935157612548 t^{45}+701292607299977103681 t^{44}+353186980005367737798 t^{43}-1116968327151616428428 t^{42}-859024274546105420817 t^{41}+1503815535381396267241 t^{40}+1978283291523092192414 t^{39}-770158457435737761363 t^{38}-2009097968212584989762 t^{37}+1014597460352501439955 t^{36}+3677733780708875032995 t^{35}+1601409851543523439677 t^{34}-2156239405803717244907 t^{33}-2662759188316150514367 t^{32}-873065166746534194029 t^{31}-810999439761725789831 t^{30}-2660876270139644060452 t^{29}-3270199956061165143451 t^{28}-1501615969052484683057 t^{27}+576845256977103320196 t^{26}+1085035784854394189653 t^{25}+383882323941133661670 t^{24}-223684643662301703985 t^{23}-229162265457037901164 t^{22}+19172681407347569034 t^{21}+137065887465308026972 t^{20}+88646209024346687872 t^{19}+8634115397464554442 t^{18}-24056489640687046955 t^{17}-18074644897445141197 t^{16}-4666617916465161384 t^{15}+1869658854005574465 t^{14}+2481218507217177934 t^{13}+1324036266422091961 t^{12}+446721997567042222 t^{11}+93417401703067093 t^{10}+5366646990216221 t^9-4446581981577733 t^8-2101882606743268 t^7-552860849689262 t^6-102184694487989 t^5-13882682549917 t^4-1375481297897 t^3-94874129307 t^2-4093515290 t-83397747\right)+d^{29} \left(2281034785680 t^{69}-27574064890200 t^{68}+80314954988964 t^{67}+241101327349422 t^{66}-1559658506400042 t^{65}+279527428327868 t^{64}+11188671961843541 t^{63}-13499640859304716 t^{62}-39237981603673979 t^{61}+83143106529542517 t^{60}+21741624528422086 t^{59}-206552531438840277 t^{58}+556763601855080634 t^{57}-340654143607205656 t^{56}-3854641460942361112 t^{55}+5372771201401417312 t^{54}+16801120074017875382 t^{53}-26680682865101343233 t^{52}-58379547602750918660 t^{51}+88724396031197285265 t^{50}+173575117698943731634 t^{49}-222058335461537717305 t^{48}-451206579192787839840 t^{47}+424287727127037917732 t^{46}+1016564568283592326541 t^{45}-599249516055004621305 t^{44}-1995500251823750593696 t^{43}+420132128164961632930 t^{42}+3196437007886508486016 t^{41}+327902515781041666299 t^{40}-4310983195312325411602 t^{39}-1765538650004979731004 t^{38}+5119772545207256072415 t^{37}+4908732759097951358198 t^{36}-2160193141293759933822 t^{35}-3628227126131582277109 t^{34}+3922247277386294282690 t^{33}+8891731219610751984425 t^{32}+3214627739554881632458 t^{31}-6326200748752237675504 t^{30}-9669114415433553206717 t^{29}-6497982149290901815104 t^{28}-2983770216115782596514 t^{27}-2123323519478705428603 t^{26}-2153629649627506078233 t^{25}-1290121780451637393720 t^{24}-31263859837930377329 t^{23}+524585782657588401368 t^{22}+306243873823432064155 t^{21}-62570016195416706922 t^{20}-185359759708125608080 t^{19}-109319682262806206472 t^{18}-13727456324716815552 t^{17}+22733299389290632636 t^{16}+17707562056608465420 t^{15}+5203483295979817660 t^{14}-960696311062121844 t^{13}-1803689699543410584 t^{12}-1019764525725108354 t^{11}-370128193070468020 t^{10}-94402557837158674 t^9-16193365767095904 t^8-1291352647845059 t^7+209173112555792 t^6+97853373460293 t^5+19245315123054 t^4+2401460560730 t^3+196499074866 t^2+9748600199 t+224550572\right)+d^{30} \left(2680665889200 t^{69}-35062292639736 t^{68}+116810825896140 t^{67}+251090348945894 t^{66}-2081969366818082 t^{65}+1008064781921522 t^{64}+15317555148922426 t^{63}-23468751182044297 t^{62}-64314889879641212 t^{61}+170487793849079835 t^{60}+141322355586869115 t^{59}-790093878602447116 t^{58}+125356662684717296 t^{57}+2729197680115963371 t^{56}-2680243990398427023 t^{55}-7651096982413920339 t^{54}+14151432940782525730 t^{53}+18954123450553532805 t^{52}-51564588424263311050 t^{51}-45925877960457320761 t^{50}+147857635615631669182 t^{49}+115150148065250737139 t^{48}-349006066315592806282 t^{47}-296062444325722835376 t^{46}+669024019404581610748 t^{45}+687473605720717805107 t^{44}-1069374055260633425444 t^{43}-1473657646980035124479 t^{42}+1216892113250240926501 t^{41}+2560846788194465196421 t^{40}-677599888599514946912 t^{39}-3174509616323238910588 t^{38}+346792968932511908078 t^{37}+4839344371714017364945 t^{36}+3075525875680050524034 t^{35}-1682654649102037740630 t^{34}-1556237621274211245709 t^{33}+2292724103287173437911 t^{32}+2124861932103857833592 t^{31}-3352435898296312034400 t^{30}-7454987413627432446220 t^{29}-5881362266851827786487 t^{28}-1628021484205488433621 t^{27}+664384197366710912407 t^{26}+326683464028930975175 t^{25}-486213234092143664130 t^{24}-447145268895145223435 t^{23}+48263735092808619484 t^{22}+284765161611834505811 t^{21}+171197808207725304248 t^{20}-6495636447732598887 t^{19}-70571082534813398383 t^{18}-44735619665125037344 t^{17}-7046057516125411575 t^{16}+8555317059965650153 t^{15}+7765061492101907815 t^{14}+3284506781473112687 t^{13}+623257264898671201 t^{12}-153880639920004486 t^{11}-176142594194751286 t^{10}-79494629833477610 t^9-24380442428677380 t^8-5598687685277382 t^7-987855028216235 t^6-133633154923837 t^5-13556022635331 t^4-985347186554 t^3-47156357940 t^2-1249787156 t-11356853\right)-7232

==> polynomials/Q_54,78.tex <==
127 t^{69}-7069 t^{68}+182500 t^{67}-2894920 t^{66}+31407619 t^{65}-244397401 t^{64}+1379970226 t^{63}-5487141994 t^{62}+13388239355 t^{61}-5281774277 t^{60}-102884928875 t^{59}+415630479031 t^{58}-567739982533 t^{57}-1155228414191 t^{56}+6360903519247 t^{55}-8141005088522 t^{54}-15255941678559 t^{53}+65626904704826 t^{52}-44774082985884 t^{51}-188623583412573 t^{50}+418044462452533 t^{49}+114855226537662 t^{48}-1420054822267765 t^{47}+1095212849648072 t^{46}+2795228487559632 t^{45}-4988426566005245 t^{44}-2808556771463526 t^{43}+12544807691313289 t^{42}-1666045006821479 t^{41}-22513872319097488 t^{40}+13077009555227407 t^{39}+31218799594937208 t^{38}-30335914871587276 t^{37}-34865517408112665 t^{36}+48042410214715733 t^{35}+32501287926128359 t^{34}-59194142219280721 t^{33}-26551067238716063 t^{32}+59419581779378021 t^{31}+20373528987664120 t^{30}-49393752720579887 t^{29}-15563407168009307 t^{28}+33939191599924145 t^{27}+11668833266356123 t^{26}-18934421362848823 t^{25}-7909292597273326 t^{24}+8275592946111816 t^{23}+4436231697704315 t^{22}-2664045667471645 t^{21}-1926301857375517 t^{20}+560469617063347 t^{19}+617183770918247 t^{18}-51590232976097 t^{17}-142171647177282 t^{16}-7742548046709 t^{15}+24186343454730 t^{14}+3905820437683 t^{13}-3252416739626 t^{12}-996730880147 t^{11}+266252621362 t^{10}+168880233926 t^9+12103451491 t^8-10002840926 t^7-3008924023 t^6-251364588 t^5+31147201 t^4+8836320 t^3+776604 t^2+27124 t+d \left(-364 t^{71}+20838 t^{70}-556406 t^{69}+9153287 t^{68}-103028459 t^{67}+830038609 t^{66}-4823413249 t^{65}+19431216522 t^{64}-45232966967 t^{63}-10869816480 t^{62}+536263143612 t^{61}-1977378937350 t^{60}+2244877119648 t^{59}+8159029777932 t^{58}-37635788730643 t^{57}+41418014891147 t^{56}+121800462024509 t^{55}-455971471400494 t^{54}+238295008359192 t^{53}+1606787888762141 t^{52}-3311792880062148 t^{51}-1607696646115317 t^{50}+13355644626284191 t^{49}-9260160550292177 t^{48}-30743261573496676 t^{47}+52516159925686947 t^{46}+38066734331596400 t^{45}-152810502800013418 t^{44}+9977350357682997 t^{43}+313798127265802139 t^{42}-171510238902646492 t^{41}-498753962921571307 t^{40}+473038771087060657 t^{39}+644417408479801458 t^{38}-867049536460790073 t^{37}-706096873401885475 t^{36}+1234047249639181476 t^{35}+691372704531839801 t^{34}-1437526704158833073 t^{33}-644153350562983278 t^{32}+1396551297266536959 t^{31}+594725015614239024 t^{30}-1129815704143561763 t^{29}-532141756507512496 t^{28}+746044114102830640 t^{27}+429823140800279263 t^{26}-384811061490175545 t^{25}-290659611052218815 t^{24}+141520287574736822 t^{23}+154485770710303924 t^{22}-28235246790575127 t^{21}-60875186699119122 t^{20}-2651986623972871 t^{19}+16682107921919878 t^{18}+3690668595223626 t^{17}-2978662448287866 t^{16}-1136288609372710 t^{15}+355613163820268 t^{14}+204379901584280 t^{13}-38610192985234 t^{12}-34330814141106 t^{11}+1301782444266 t^{10}+4995726500927 t^9+1053365624657 t^8-169665688986 t^7-111186195464 t^6-18380093416 t^5-492326976 t^4+238388242 t^3+33923565 t^2+1765024 t+28671\right)+d^2 \left(329 t^{73}-19985 t^{72}+562119 t^{71}-9658309 t^{70}+112244451 t^{69}-916790326 t^{68}+5213270823 t^{67}-18670365700 t^{66}+20445344546 t^{65}+198790637607 t^{64}-1326662380603 t^{63}+3613887312252 t^{62}-616094293634 t^{61}-30349720404205 t^{60}+98129282911085 t^{59}-51324599254933 t^{58}-509672050129325 t^{57}+1427055025328778 t^{56}-98272765414749 t^{55}-6852955363133210 t^{54}+11546693034795165 t^{53}+11730373485071621 t^{52}-60102505330808209 t^{51}+29735188603100661 t^{50}+167636219702311826 t^{49}-254033128627682882 t^{48}-261193721014521596 t^{47}+883403723522924295 t^{46}+41204327083917783 t^{45}-2086243668104953360 t^{44}+1037615626924703232 t^{43}+3759986578105860710 t^{42}-3512915135834471079 t^{41}-5471196672656840259 t^{40}+7458759776325927692 t^{39}+6723928110977401410 t^{38}-12161341706989352588 t^{37}-7370269368312629832 t^{36}+16236125950009946420 t^{35}+7717715891095826672 t^{34}-18186682141054825670 t^{33}-8129320953039048587 t^{32}+17129834397107731950 t^{31}+8492123876914253077 t^{30}-13331399538741252219 t^{29}-8191969212585681931 t^{28}+8210205247774959632 t^{27}+6747861925795707936 t^{26}-3631602573679228056 t^{25}-4447918724698604780 t^{24}+828803303617645464 t^{23}+2204925943997493083 t^{22}+193718376481260003 t^{21}-757033444358906723 t^{20}-250705576214534817 t^{19}+154016535930396018 t^{18}+98678213933756418 t^{17}-10466630183189522 t^{16}-19565148576173932 t^{15}-1617256073993942 t^{14}+2175729879245927 t^{13}+171134250185478 t^{12}-330034145851697 t^{11}-35245504388319 t^{10}+56973196468186 t^9+21244626359382 t^8+262762274976 t^7-1525582215225 t^6-408477809772 t^5-40511189179 t^4+694094780 t^3+501873066 t^2+39417556 t+960235\right)+d^3 \left(-91 t^{75}+6405 t^{74}-199780 t^{73}+3660298 t^{72}-43310336 t^{71}+333473564 t^{70}-1455218642 t^{69}-50842920 t^{68}+50893327667 t^{67}-389322941879 t^{66}+1519134528547 t^{65}-2296714497076 t^{64}-8452732578317 t^{63}+58416909101437 t^{62}-125638155111639 t^{61}-96509524427009 t^{60}+1208626115833916 t^{59}-2360245054991990 t^{58}-2117210260262857 t^{57}+17448532837784471 t^{56}-20894446420348027 t^{55}-47730236487327502 t^{54}+161286247670529934 t^{53}-24527599144140415 t^{52}-569156524341474788 t^{51}+703129079842586309 t^{50}+1137563884668865121 t^{49}-3095783805598788795 t^{48}-745817044492770791 t^{47}+8568793258464630064 t^{46}-3461731017570417960 t^{45}-17604668603295409919 t^{44}+15654684982156677549 t^{43}+28714661566855773126 t^{42}-39106118503719832629 t^{41}-38948868564387799237 t^{40}+73155400606028329364 t^{39}+46340260930508618226 t^{38}-111451639918778391076 t^{37}-52148247305584280625 t^{36}+142972565963046109158 t^{35}+59913980062343974687 t^{34}-155804709368363008044 t^{33}-71037859844322029917 t^{32}+142655084360773096804 t^{31}+80940512074445146739 t^{30}-106014689010133821302 t^{29}-81012149097282401367 t^{28}+59157021017575067888 t^{27}+66365615984237686199 t^{26}-19677334185912198794 t^{25}-41860907841643477598 t^{24}-1531033463107992117 t^{23}+18788300708593242990 t^{22}+6208423836373569166 t^{21}-5104141202237470282 t^{20}-3625184617178511181 t^{19}+366958361111293346 t^{18}+1027419787090677897 t^{17}+227287624975853849 t^{16}-117348676827877081 t^{15}-62032300382878199 t^{14}-2273844002994304 t^{13}+2467406042686202 t^{12}-712115103034933 t^{11}-80538739615369 t^{10}+433168553547440 t^9+214156430601187 t^8+25282490368253 t^7-10316885749001 t^6-4507619328961 t^5-726099486970 t^4-43535625072 t^3+2018416436 t^2+393872734 t+14100865\right)+d^4 \left(-273 t^{76}+14231 t^{75}-306180 t^{74}+3066408 t^{73}-1099635 t^{72}-386904766 t^{71}+5675136189 t^{70}-45028863598 t^{69}+214365433994 t^{68}-451960040139 t^{67}-1496216583219 t^{66}+15840201012872 t^{65}-55505979222603 t^{64}+47952101202469 t^{63}+379986457566788 t^{62}-1644577475381714 t^{61}+1726563858452399 t^{60}+7183342856333110 t^{59}-27527579975196868 t^{58}+15106463823951890 t^{57}+118282340366836813 t^{56}-272410863144254440 t^{55}-119522014006871183 t^{54}+1296380760378471808 t^{53}-1137273288807695291 t^{52}-3376453312670812717 t^{51}+7151443697683860681 t^{50}+4085895607152607824 t^{49}-23959047615494750231 t^{48}+5926167486636022744 t^{47}+56906479962336364700 t^{46}-45303667223811041618 t^{45}-104654255941705139556 t^{44}+137260348333092605420 t^{43}+156485734282149768477 t^{42}-296617963952533696450 t^{41}-199587616049763187577 t^{40}+514752266145065239285 t^{39}+233784148002837278051 t^{38}-751449134761960275728 t^{37}-279050704341219941432 t^{36}+939263745091512727593 t^{35}+360812073015752245728 t^{34}-1002769765720065774352 t^{33}-477007617304772553438 t^{32}+893332785320927920720 t^{31}+577021485451976313390 t^{30}-628753678414367576730 t^{29}-586358524169919078256 t^{28}+305280263255095598992 t^{27}+471018063450754416986 t^{26}-49953266136050099863 t^{25}-280021246980532864407 t^{24}-65123014066346731145 t^{23}+109238485060084780224 t^{22}+65883475611476068195 t^{21}-18173554131533531533 t^{20}-29216536106049441213 t^{19}-5303273471427926833 t^{18}+5811176286973488030 t^{17}+3394075583137063302 t^{16}+124605459873102417 t^{15}-505851393197159520 t^{14}-205577806230194834 t^{13}-29617668272943511 t^{12}+2866971735897414 t^{11}+5005691222520601 t^{10}+3766653657540700 t^9+1581822104783390 t^8+281033422921460 t^7-35957175706452 t^6-30018188050314 t^5-6755626328641 t^4-722547509184 t^3-26783079107 t^2+1283032669 t+100536449\right)+d^5 \left(-273 t^{77}+7063 t^{76}+63805 t^{75}-5316568 t^{74}+103629890 t^{73}-1063646272 t^{72}+5580387630 t^{71}+2045814139 t^{70}-280425932953 t^{69}+2347949457937 t^{68}-10065091412178 t^{67}+17121935305896 t^{66}+61278289563889 t^{65}-475983142407501 t^{64}+1151615043032992 t^{63}+581914947154549 t^{62}-11235632629300717 t^{61}+25450000133885389 t^{60}+14651168673025172 t^{59}-185639104315359233 t^{58}+275095772162735678 t^{57}+467446403217796026 t^{56}-2016158414869276736 t^{55}+816875786480454244 t^{54}+7032069001951717614 t^{53}-11059710336150137708 t^{52}-12968342421957169241 t^{51}+47540822106209018757 t^{50}+30138909373483116 t^{49}-133706945955731661525 t^{48}+86010634458968531983 t^{47}+281185567073831767033 t^{46}-337104945397049994292 t^{45}-468077869426156809326 t^{44}+854788478777606613700 t^{43}+642703125946878969537 t^{42}-1693304589059606286102 t^{41}-772363363344379373443 t^{40}+2799213896142939489974 t^{39}+909754585297658832463 t^{38}-3974529509392730723059 t^{37}-1202614168343605819797 t^{36}+4882749124807238935090 t^{35}+1785114953594164915541 t^{34}-5128186888336561924534 t^{33}-2590573897029870542844 t^{32}+4443083752529571962413 t^{31}+3257994820093594773014 t^{30}-2931522616284983361632 t^{29}-3316096332567786823095 t^{28}+1156553083870244995410 t^{27}+2588086571777831203816 t^{26}+148376435877201585794 t^{25}-1428637072013284568569 t^{24}-607708444508792628983 t^{23}+453093197874686638648 t^{22}+447063662905171695482 t^{21}+2874846298751024017 t^{20}-159020006846065618173 t^{19}-68391524596595823684 t^{18}+16145546197437291159 t^{17}+24285729181693247725 t^{16}+6987734667021929536 t^{15}-1640917799823229143 t^{14}-1905835293574686851 t^{13}-624511593724324189 t^{12}-45605846491455561 t^{11}+53023036615678670 t^{10}+33125725324754614 t^9+11333570746090336 t^8+2153613751740824 t^7-13909269545620 t^6-136765295426227 t^5-40027663387382 t^4-5794303605201 t^3-424197895605 t^2-10412752774 t+211703083\right)+d^{29} \left(-1450530509064 t^{78}+30161482106886 t^{77}-265458864846786 t^{76}+1174345848100308 t^{75}-1708980071411160 t^{74}-8441972029709320 t^{73}+47705993146219498 t^{72}-59232593827524636 t^{71}-242075536926917170 t^{70}+955992768491777298 t^{69}-288421833613487596 t^{68}-4924521440355715230 t^{67}+8634115915362552959 t^{66}+11364749219105218742 t^{65}-47633240255034338184 t^{64}+3447990548291682551 t^{63}+153693902216653418497 t^{62}-114165011680911173741 t^{61}-337694828797909204551 t^{60}+410293426177590885544 t^{59}+527085666089023986048 t^{58}-759362207252383513078 t^{57}-570402045265489736397 t^{56}+232984446933093875099 t^{55}+269749978863955394089 t^{54}+3857864337414265211914 t^{53}+1090458058630174838207 t^{52}-17084761020374607410381 t^{51}-6947079692138986467159 t^{50}+47877278951079027882254 t^{49}+28405179483430114004557 t^{48}-102883907988335103874317 t^{47}-89916412211000776065448 t^{46}+172578152666272893881832 t^{45}+225324135236082858925393 t^{44}-209853888101707673545654 t^{43}-449977100081173458234806 t^{42}+120188753906386652928043 t^{41}+699053356067623929711092 t^{40}+181433167575126210752207 t^{39}-797006261957739001128526 t^{38}-653755274146032125927431 t^{37}+530561644844969800992751 t^{36}+1024387745896040040087452 t^{35}+126328834466767167494068 t^{34}-851456314245151131457648 t^{33}-614433184323916973413302 t^{32}+445449293041641074081145 t^{31}+1109050159343284905026853 t^{30}+914725293384984411056627 t^{29}+328732015749353437104882 t^{28}-109739304017490003356314 t^{27}-275059540094865012049180 t^{26}-283790090644831234844746 t^{25}-233708237480118901174427 t^{24}-160740567156102613146403 t^{23}-88197382620081619224019 t^{22}-36559597009193327082609 t^{21}-10250261359534558248561 t^{20}-540943299787504152212 t^{19}+1994811920786528139250 t^{18}+2071961371263120330455 t^{17}+1336501069892591858797 t^{16}+526164026141028071638 t^{15}+21146667935839527246 t^{14}-147268732341318143525 t^{13}-132037742076544837272 t^{12}-73070644184764009844 t^{11}-30233679945320629639 t^{10}-9898283802249386218 t^9-2621405154794842944 t^8-566373873901260144 t^7-100027501568893199 t^6-14407198218212626 t^5-1678394815550185 t^4-154749431985163 t^3-10723742817278 t^2-497389719446 t-11479293791\right)+d^{30} \left(-1394577220140 t^{78}+25935094041792 t^{77}-187297597239012 t^{76}+491437101495770 t^{75}+1454224952106372 t^{74}-14535894180852670 t^{73}+35638734345854188 t^{72}+35036202788948170 t^{71}-384992103559481566 t^{70}+590421881852085652 t^{69}+1319336436016577562 t^{68}-5470809388405650838 t^{67}+952288370571899836 t^{66}+24183181228974687124 t^{65}-28927116831125289241 t^{64}-69340434730490061488 t^{63}+155323185645517675734 t^{62}+140197003182971829433 t^{61}-556105618928762848891 t^{60}-202470310768181316615 t^{59}+1593386824883341081400 t^{58}+219517887335765944013 t^{57}-3924594531486478879784 t^{56}-378305564137361852925 t^{55}+8537493057946153847599 t^{54}+1757063278533415201619 t^{53}-16349377129850180179817 t^{52}-7575113999397329717615 t^{51}+26578736618462898016353 t^{50}+24260623260793419556689 t^{49}-33096973746878380787132 t^{48}-59790211562560105754003 t^{47}+19360485681579386896182 t^{46}+114585339400861778927222 t^{45}+41258702446033934576826 t^{44}-165949036643675866155973 t^{43}-171086738023111543045091 t^{42}+154055862830923369458109 t^{41}+346124316028957948823830 t^{40}-10316283529620596635018 t^{39}-465388423907088922498786 t^{38}-266037212036333687135074 t^{37}+393492793929496765682537 t^{36}+562444890114484599448772 t^{35}-9820329792862188786299 t^{34}-487843972364842477003830 t^{33}-198352508783714617968258 t^{32}+478171363398616887942626 t^{31}+753061985557107507711112 t^{30}+430769788713000921131600 t^{29}-63369246359923873912723 t^{28}-325538513172737471434534 t^{27}-318124925097907540190153 t^{26}-205097757646704186957974 t^{25}-106918857535837463016424 t^{24}-47317437089931263206548 t^{23}-13377298255982045493596 t^{22}+4136947605914758549227 t^{21}+9748605266928186218584 t^{20}+8692118696753888774705 t^{19}+5811089627654310773553 t^{18}+3465954572237792578214 t^{17}+1988320727827170398878 t^{16}+1080484616807827786293 t^{15}+521524202927239593658 t^{14}+209065721704437893148 t^{13}+64551754063286437026 t^{12}+12877125906338175687 t^{11}+61145842276184261 t^{10}-1222713803520959258 t^9-604415034513570639 t^8-188578815200286636 t^7-43742569842032403 t^6-7832817610729498 t^5-1080660379405272 t^4-111724970556307 t^3-8166111905248 t^2-376086411204 t-8191281471\right)+d^{28} \left(-913941905016 t^{78}+20950358074152 t^{77}-216606671329842 t^{76}+1288151216828070 t^{75}-4455074823544542 t^{74}+6109302508769082 t^{73}+18433174799471640 t^{72}-105525612252471688 t^{71}+143780647915500240 t^{70}+354177372440244508 t^{69}-1535604856322442400 t^{68}+805169718121199914 t^{67}+6225659203467377980 t^{66}-12815673932288962825 t^{65}-8076833091011255727 t^{64}+61101364106009410900 t^{63}-51543978054915647866 t^{62}-153024387706235556238 t^{61}+385707850162679990922 t^{60}+69237066142568886735 t^{59}-1465014214375768680250 t^{58}+1207035463121948605202 t^{57}+3971787400610566277124 t^{56}-6491166235439015052923 t^{55}-8671235144149328379188 t^{54}+21580406695333722355509 t^{53}+17101321903203182601819 t^{52}-55840038197934005920399 t^{51}-34974315370550447856145 t^{50}+120150324099762424407209 t^{49}+79391956674421287754860 t^{48}-217802908311711168003382 t^{47}-185488666797959861003800 t^{46}+323260400851673523845842 t^{45}+396700275132912482985993 t^{44}-355282846189616282454723 t^{43}-717963978138675167439021 t^{42}+177547199941004314764446 t^{41}+1031364311864027581431856 t^{40}+305163478497812825807750 t^{39}-1069951624079108936256121 t^{38}-973187703241362551240607 t^{37}+560710521016091519437086 t^{36}+1367649777941004838846651 t^{35}+387250660612544832716600 t^{34}-984690187928112803752874 t^{33}-1059346478670551430522009 t^{32}+64095988331573231609723 t^{31}+1104941376186176427735605 t^{30}+1306552701797732321797714 t^{29}+901365795996650929466157 t^{28}+403486104783013512347339 t^{27}+51130439930967843275378 t^{26}-153467092908362402074627 t^{25}-244298434567633378320099 t^{24}-242452318383551462938335 t^{23}-183619104791405215949289 t^{22}-112386014452565321190820 t^{21}-57271714941880103123527 t^{20}-24853173037191611166314 t^{19}-9893246701552889246207 t^{18}-4756938382127474594943 t^{17}-3489117279098372176368 t^{16}-2884727596017471410821 t^{15}-2042153292555225262458 t^{14}-1158251924622240910793 t^{13}-524183170185548302868 t^{12}-189502350623974484545 t^{11}-54180048135035396296 t^{10}-11805742528530978790 t^9-1738129513174195002 t^8-76697335174482473 t^7+42919135758215724 t^6+14971550938647175 t^5+2782901894117898 t^4+340017243519883 t^3+27326877653557 t^2+1316682787610 t+28822603398\right)+d^{31} \left(-791856050856 t^{78}+12442373280558 t^{77}-56941356493152 t^{76}-151105950150568 t^{75}+2600050851740088 t^{74}-10106282709466758 t^{73}+6161596447726968 t^{72}+77932826150981468 t^{71}-239944429302932064 t^{70}-43537652920430260 t^{69}+1565716625684651384 t^{68}-2211229732137908622 t^{67}-5005536743554568271 t^{66}+16564657433478424013 t^{65}+4550054464897766457 t^{64}-72811149066889089284 t^{63}+41497270399895962107 t^{62}+236248212513673188452 t^{61}-284618792120152202890 t^{60}-615583482608813445328 t^{59}+1121955794643280331150 t^{58}+1366774499017652764767 t^{57}-3364558914105767220512 t^{56}-2781184743308518963570 t^{55}+8313373081954700643607 t^{54}+5678710875224923103194 t^{53}-17467369005734141205646 t^{52}-12314103458670905016184 t^{51}+31318256285931922468916 t^{50}+27350265889409152661306 t^{49}-46728676449061690252488 t^{48}-57350108517383819018791 t^{47}+52877358384406333875696 t^{46}+105123447385235276048461 t^{45}-30504981312500724050493 t^{44}-159783703357211441968605 t^{43}-41176563253382084492821 t^{42}+184886148311790922144901 t^{41}+158668162185921620864517 t^{40}-128969565066377760112556 t^{39}-264000256793859316858984 t^{38}-14917441460382320308034 t^{37}+293777711988113412654785 t^{36}+242005218774367714251123 t^{35}-75657724370528923441848 t^{34}-200588510722635647920159 t^{33}+39381230055296827353174 t^{32}+332839296318514744579544 t^{31}+334581626896870874394989 t^{30}+65889040596521939611570 t^{29}-199206248206732183196580 t^{28}-275809832962787950547658 t^{27}-194997509349585832107701 t^{26}-80536486248002093545057 t^{25}-8930476829370319060971 t^{24}+15681875702334740008766 t^{23}+17390235427017142462027 t^{22}+13595622213390184535397 t^{21}+9792765386121657783556 t^{20}+6515265444751190079706 t^{19}+3861790833874949778504 t^{18}+2053559823903382469335 t^{17}+1035990684799920471658 t^{16}+527915069684482479453 t^{15}+272073355005077328034 t^{14}+133222237377480299300 t^{13}+58026155675824966262 t^{12}+21596358980922820794 t^{11}+6722697622547372722 t^{10}+1724108477498918333 t^9+357967370056687806 t^8+58547097408049723 t^7+7178274952739847 t^6+590222557046056 t^5+20755972786057 t^4-1663110939057 t^3-265848020041 t^2-14095195292 t-264822151\right)+d^{20} \left(-215600997556 t^{78}+7726056685524 t^{77}-125415149613178 t^{76}+1199427321881465 t^{75}-7270965693810030 t^{74}+26934667543194596 t^{73}-42570783022907025 t^{72}-114128363559623732 t^{71}+784109537311595473 t^{70}-1308497112571641254 t^{69}-2686552150985642603 t^{68}+14973341560057701254 t^{67}-11772948143831046741 t^{66}-68281464724046888000 t^{65}+170186518895784899908 t^{64}+110030634937452553875 t^{63}-941628599694909055973 t^{62}+584248573590242411919 t^{61}+3249901013232723630207 t^{60}-5210042211956095037148 t^{59}-7257361183579656016504 t^{58}+22645006746289068719550 t^{57}+7770373937094618743127 t^{56}-70515423408579796434106 t^{55}+14331813366817709530685 t^{54}+175405497677542383574780 t^{53}-100462339489089028113129 t^{52}-370354107923840753879631 t^{51}+313410593041337445920480 t^{50}+695974353312917476623940 t^{49}-718156658210793706923727 t^{48}-1213079408202194763374694 t^{47}+1340744133635926172594783 t^{46}+2023155430039173484800897 t^{45}-2107055403236866771910485 t^{44}-3269792020055398614968869 t^{43}+2769266138331157588045586 t^{42}+5071184489272005375005522 t^{41}-2850979296989715427416998 t^{40}-7332529117372500373356521 t^{39}+1708219360640799928438336 t^{38}+9460495305733295077335181 t^{37}+1118488009481635653366683 t^{36}-10229448318807873370331567 t^{35}-5207992570453151823272203 t^{34}+8315494971443107070253185 t^{33}+8771044201786090239186731 t^{32}-3657162604415075527132113 t^{31}-9516340291530153203161777 t^{30}-1683132437808813728109953 t^{29}+6789642791015745455606833 t^{28}+4997603177606280733131059 t^{27}-2210298452178475851317825 t^{26}-5079124548356133631336973 t^{25}-2093692114274316498830024 t^{24}+1647549129012868652024674 t^{23}+2721280021026050493721538 t^{22}+1887944853706979261440633 t^{21}+1013682412344472489773226 t^{20}+684882392518419240844456 t^{19}+546702305745566763935135 t^{18}+333678758301076528022974 t^{17}+105539906723626563481969 t^{16}-24867985310485424256406 t^{15}-52209392412102171244563 t^{14}-33615289619849089715237 t^{13}-12992212615744435842486 t^{12}-2814703761818015444381 t^{11}+76842775688769772185 t^{10}+340655591015884405918 t^9+157242101899757393451 t^8+45306666865870869002 t^7+9417425622401285290 t^6+1464990013939874048 t^5+171781796849229584 t^4+15148947417864441 t^3+997641021986749 t^2+46896866460186 t+1231952394927\right)+d^{19} \left(-193427117780 t^{78}+7132522545607 t^{77}-119777110538676 t^{76}+1194538318794301 t^{75}-7659428230198106 t^{74}+31055489630186570 t^{73}-63613863681616550 t^{72}-63550940234939405 t^{71}+823522119391309374 t^{70}-1983709506770178411 t^{69}-903739208706352991 t^{68}+15356742448297727375 t^{67}-24859732408702531590 t^{66}-43667442409635802527 t^{65}+197640163177478374508 t^{64}-56124472920384900892 t^{63}-835937770168645731950 t^{62}+1152161794635577513074 t^{61}+2235895650357355511257 t^{60}-6319986575442849684930 t^{59}-2950695899450703807924 t^{58}+23198101363021555803468 t^{57}-5412424375394106563313 t^{56}-65571008435703065117879 t^{55}+47724832579975224347701 t^{54}+151385698427800792457616 t^{53}-175489304253820368123458 t^{52}-297479546934915563249549 t^{51}+468315696821383265990540 t^{50}+519326055067364957062803 t^{49}-1016153986300009610599038 t^{48}-848961641453090024296876 t^{47}+1876094545330312823858694 t^{46}+1372776453010413949298419 t^{45}-3002731183523396173367668 t^{44}-2258418686563126717357829 t^{43}+4158571441007332883674542 t^{42}+3702081826181874617277672 t^{41}-4842423480321892258658468 t^{40}-5725729961177842042347218 t^{39}+4350255127750438211962126 t^{38}+7859004985368104090268201 t^{37}-2142597003398544670396019 t^{36}-8992823538692252392174189 t^{35}-1484161877933030631508405 t^{34}+7883522947110275448647156 t^{33}+4987153248538837930003829 t^{32}-4339708745193275690692316 t^{31}-6330919803835582803944795 t^{30}-54236948144901400790800 t^{29}+4689856619060764290621324 t^{28}+2923670756331807514745450 t^{27}-1221829546128609359031017 t^{26}-2764979027587537148955720 t^{25}-1568382025283821744620257 t^{24}+14600112003217355758392 t^{23}+846283075151155370745987 t^{22}+1205317822347271816172638 t^{21}+1360360156054025099354820 t^{20}+1206622912251932350435802 t^{19}+749210746059583227411428 t^{18}+251898172711541666771770 t^{17}-46896914423569550336591 t^{16}-122549329169926342295189 t^{15}-85194127186133847849212 t^{14}-34641777288836326901150 t^{13}-7162719788503942501093 t^{12}+1061108627017621203507 t^{11}+1554777336774512820172 t^{10}+699835733937750840188 t^9+197137124791632372142 t^8+35986932055311023787 t^7+3191568403023063632 t^6-349695775409101035 t^5-179732684140730621 t^4-32738815221263209 t^3-3472062772690562 t^2-211904573374831 t-5804493778241\right)+d^{39} \left(-159527349852 t^{78}+724524759805 t^{77}+556264474704 t^{76}-19537473387323 t^{75}+68538924326179 t^{74}+44138522301360 t^{73}-854100904154121 t^{72}+1118953158212957 t^{71}+4991279058153203 t^{70}-13250817874379347 t^{69}-17268885105322026 t^{68}+82340716610198035 t^{67}+28063383963826301 t^{66}-365556604052271190 t^{65}+50633714953074853 t^{64}+1267285547471185331 t^{63}-544931266635100423 t^{62}-3674408910404582047 t^{61}+2140118975548510641 t^{60}+9147072706805203240 t^{59}-5902653340534506266 t^{58}-20341092013695101841 t^{57}+12218084373557836154 t^{56}+40634475048593435717 t^{55}-19245128548152834698 t^{54}-72901530617520837642 t^{53}+22048044614770928884 t^{52}+120545760738878267595 t^{51}-2492085745468800401 t^{50}-162456245282292088784 t^{49}-27390896719251613563 t^{48}+219845161181264610456 t^{47}+134492033393955779480 t^{46}-169420875272298584415 t^{45}-167726952629659845566 t^{44}+158041760440896513763 t^{43}+272565929077070960885 t^{42}-24101010721903636795 t^{41}-312325736134181887856 t^{40}-254780348349339677671 t^{39}-48555608563956537249 t^{38}-22819375123962779537 t^{37}-160284687908426358173 t^{36}-191048517903848733904 t^{35}+32567777736211350163 t^{34}+374068473300682682988 t^{33}+554587507476896365950 t^{32}+413642279743634403447 t^{31}+52638025391394898128 t^{30}-269509697318748278842 t^{29}-372513259259189039553 t^{28}-274559492396897452889 t^{27}-111545070659998711438 t^{26}+5662945433363091840 t^{25}+50085886659004962281 t^{24}+47882703418470927710 t^{23}+30717471876156545968 t^{22}+15346076311003905578 t^{21}+5945330790937823165 t^{20}+1458072453550660170 t^{19}-135908318551563689 t^{18}-416338000882220169 t^{17}-292097221648765381 t^{16}-142968068131489347 t^{15}-57287644973280548 t^{14}-20657671725164886 t^{13}-7238578417071121 t^{12}-2531312074968892 t^{11}-850208204792544 t^{10}-258042719412357 t^9-67554456453451 t^8-14826957277176 t^7-2675288247785 t^6-389364348124 t^5-44599029043 t^4-3874948908 t^3-240299648 t^2-9484821 t-179194\right)+d^{40} \left(-133057690156 t^{78}+183960376368 t^{77}+2788794093728 t^{76}-13035082415693 t^{75}+1335343051902 t^{74}+129153952963746 t^{73}-304394021950237 t^{72}-492212034598246 t^{71}+2994166401734028 t^{70}-856448128908153 t^{69}-16765644074210759 t^{68}+19742447452875536 t^{67}+63912775668241431 t^{66}-126189057700117772 t^{65}-185444977741701592 t^{64}+527217245905694186 t^{63}+421456644125756452 t^{62}-1722574010758425292 t^{61}-829796695821427861 t^{60}+4621377460815057205 t^{59}+1511044693919315565 t^{58}-10674733077938418937 t^{57}-2987132412864026941 t^{56}+21606094501470046480 t^{55}+6971423166803159176 t^{54}-37794805586025886861 t^{53}-14960459042947148959 t^{52}+60771677894375109543 t^{51}+35859940005772815284 t^{50}-76615137594400929173 t^{49}-58160623305533430222 t^{48}+96917777359036471112 t^{47}+108826847608633555184 t^{46}-72806007715922841410 t^{45}-133589189984841204225 t^{44}+40122827975043759436 t^{43}+140104661597333771322 t^{42}-18367596035970927663 t^{41}-186081868715077640278 t^{40}-122569306202666264701 t^{39}+38522451969619200233 t^{38}+69075886687716053927 t^{37}-1427772755559357762 t^{36}-1887470354715805882 t^{35}+96368545117188243385 t^{34}+168350850579743442012 t^{33}+122810965396197030097 t^{32}-4117461302296326082 t^{31}-114434138395586036169 t^{30}-145705542387198120514 t^{29}-104258198197348167144 t^{28}-36757381263969338962 t^{27}+13932883304964489853 t^{26}+32616845138813004549 t^{25}+27945152578124172859 t^{24}+15574726766466257855 t^{23}+5687579252557328693 t^{22}+784693370096089675 t^{21}-677601530207423161 t^{20}-707371238149469599 t^{19}-427761682984418687 t^{18}-205431811525736516 t^{17}-82643812732244235 t^{16}-26434233700461761 t^{15}-5234265610339119 t^{14}+565484453605509 t^{13}+1122484643730801 t^{12}+619637823393599 t^{11}+234597187355582 t^{10}+68714230819340 t^9+16157416811226 t^8+3085601228545 t^7+478211000312 t^6+59557721627 t^5+5845694924 t^4+437449662 t^3+23569744 t^2+818602 t+13841\right)+d^{18} \left(-129651849184 t^{78}+4920869509140 t^{77}-85268663255283 t^{76}+880707297102012 t^{75}-5885340989008363 t^{74}+25212891106911926 t^{73}-57570445706187680 t^{72}-28881823642269305 t^{71}+677341695923249399 t^{70}-1949528712740113491 t^{69}+269202506753886757 t^{68}+12743425391946988745 t^{67}-28733867885303189360 t^{66}-18966444883405663507 t^{65}+181495543552704481831 t^{64}-170924622667601799612 t^{63}-599122916607120012816 t^{62}+1400874393228666765546 t^{61}+952779679847450795682 t^{60}-6059593877924785594478 t^{59}+1507579611265188954011 t^{58}+18945930053659212283190 t^{57}-16695988414780513607606 t^{56}-46515067015088009317614 t^{55}+69702477463680271230831 t^{54}+92303459206293908818613 t^{53}-209328021090092094336431 t^{52}-149157662190344422900286 t^{51}+510195925724374938596222 t^{50}+196512321400448527182542 t^{49}-1060304781985010326983275 t^{48}-217442626670942931970186 t^{47}+1929140757268268076119702 t^{46}+242737266685713657317773 t^{45}-3114878771790531672601284 t^{44}-399506522194416310758062 t^{43}+4472842914385410243070497 t^{42}+901418195271006344765747 t^{41}-5649921910156354509054744 t^{40}-1908312889975620950234845 t^{39}+6110090620068939598085351 t^{38}+3270262083911889877888601 t^{37}-5381041672680633039600332 t^{36}-4374067870655793931517022 t^{35}+3513219995684173281382668 t^{34}+4437408178327317161523275 t^{33}-1353783643234507687389188 t^{32}-3249998399544439375277179 t^{31}+74441709103055231602004 t^{30}+1616979466002728480637179 t^{29}-138995955743192955709868 t^{28}-784300739205248544296284 t^{27}+779180126460655040720433 t^{26}+1309994629707376024820616 t^{25}-457562028687831077461638 t^{24}-2062439724406980308682737 t^{23}-1434685080463158768043725 t^{22}+551915122707498597648320 t^{21}+1854656151988616036027500 t^{20}+1706370870661016457585161 t^{19}+801172312326416091573025 t^{18}+48906989727175778803130 t^{17}-229391187530569677029203 t^{16}-195202628937644559231751 t^{15}-87383305705962176838185 t^{14}-18984930138165506283468 t^{13}+3577787995102574001652 t^{12}+5082706334424403857028 t^{11}+2379401778627685955331 t^{10}+677906608783286610689 t^9+108036101031595381322 t^8-2974606149530475864 t^7-7540850969614779099 t^6-2505536454549263722 t^5-506874492787377318 t^4-70084996138593750 t^3-6557869560042026 t^2-379002401460460 t-10298186395319\right)+d^{21} \left(-126153082860 t^{78}+4487911847452 t^{77}-71087504418696 t^{76}+647630244570314 t^{75}-3576945035995961 t^{74}+10591840076897953 t^{73}-273561987328534 t^{72}-131079139252825728 t^{71}+461780712711716050 t^{70}-129342230920525538 t^{69}-3687393916100896299 t^{68}+9905457026296224397 t^{67}+4568230051103061959 t^{66}-71504800387543849038 t^{65}+96607251283893402782 t^{64}+226063954656010870326 t^{63}-774029167033404656216 t^{62}-47480274291704431362 t^{61}+3203259197720472896760 t^{60}-2933673270993770609460 t^{59}-8694852742297870949404 t^{58}+16160528493613959835928 t^{57}+15764434645704478870977 t^{56}-55183217850416080956124 t^{55}-14799334268734925568059 t^{54}+145143132086099199869872 t^{53}-16184900022234474699092 t^{52}-320644892569103276320613 t^{51}+108613946555536470288949 t^{50}+626711783782191092550743 t^{49}-288819399814303469614426 t^{48}-1121990110989807698107142 t^{47}+552651160181953251942551 t^{46}+1878802400471479720705857 t^{45}-834208721571348927658643 t^{44}-2969249004230618613374584 t^{43}+972673237403343735748369 t^{42}+4423428128066720679910209 t^{41}-680338920890993690981522 t^{40}-6132046141087440332367171 t^{39}-451707028892802158956314 t^{38}+7660264416013533019381044 t^{37}+2768155610437318549391469 t^{36}-8074705878482311966950408 t^{35}-6005729211352265016960894 t^{34}+6244337163482256322898112 t^{33}+8696290042883421730439998 t^{32}-2068435198308653188857371 t^{31}-8767153516443692589782734 t^{30}-2437643612502623243299957 t^{29}+5844630542074830535200855 t^{28}+4737251612027553320200652 t^{27}-2060973159073129588772279 t^{26}-4833896309778452171426751 t^{25}-1579583019823115969487806 t^{24}+2510919485569131406371855 t^{23}+3547260232593843556218386 t^{22}+2227903535630427296269596 t^{21}+835648340153144264411023 t^{20}+316496217845195174156238 t^{19}+299019250797003340923381 t^{18}+286164069187355269947641 t^{17}+171115273556364052148643 t^{16}+51926795452053276851860 t^{15}-7651475871039377457642 t^{14}-18264304765456973134428 t^{13}-11219967019930678312210 t^{12}-4261860242278341089482 t^{11}-1040267142549049603432 t^{10}-107324977957953430797 t^9+36575077887450136694 t^8+23603692800135256099 t^7+7425691473612559292 t^6+1632869691775000002 t^5+267588543867907184 t^4+32575042336754184 t^3+2810063625433092 t^2+153807194640716 t+4013312673951\right)+d^{38} \left(-108752032477 t^{78}+1076772862176 t^{77}-5492523880579 t^{76}-2766043983130 t^{75}+129857023320003 t^{74}-342268281234947 t^{73}-715696023630137 t^{72}+4201112150442069 t^{71}-265160150532364 t^{70}-26031715536981901 t^{69}+23344293349580417 t^{68}+108782461872460102 t^{67}-161934468966066676 t^{66}-350850780293092735 t^{65}+697973229777363976 t^{64}+930742483432407382 t^{63}-2285090231661980525 t^{62}-2199757909684707031 t^{61}+5946933914990602137 t^{60}+4783896891768547467 t^{59}-12778116151403357171 t^{58}-10369095256942800693 t^{57}+21838383667592583183 t^{56}+21391060782624100523 t^{55}-28260447781404924802 t^{54}-41277660440937581381 t^{53}+19478975352781355642 t^{52}+71310278327087856263 t^{51}+31298931255576289149 t^{50}-82482346940010306943 t^{49}-111009969738117379421 t^{48}+99257060578803832496 t^{47}+317746644431090059001 t^{46}+99058157503374337018 t^{45}-325889145090237077591 t^{44}-139502321454701715247 t^{43}+577361999388295720156 t^{42}+648011761396850445618 t^{41}-247707335839254055762 t^{40}-853839120311850759978 t^{39}-373988095482757869826 t^{38}+213051317299041883440 t^{37}-202689881994291835344 t^{36}-1088649898458943799399 t^{35}-1105395693982933020668 t^{34}+18560217634801832071 t^{33}+1262508577859841206940 t^{32}+1617810510932079071986 t^{31}+1024036710452724418959 t^{30}+116887761203092615088 t^{29}-507415837631058270665 t^{28}-672039708664841517808 t^{27}-522233020674188035323 t^{26}-276734383787618968599 t^{25}-78625517650210581463 t^{24}+26970134180760531803 t^{23}+56738885625013991932 t^{22}+47273804121765036598 t^{21}+28140096624161529129 t^{20}+13358354716650873203 t^{19}+5312488668669422578 t^{18}+1811180216616927083 t^{17}+502934353353006335 t^{16}+71102041298107812 t^{15}-40361840783122853 t^{14}-45532811966886611 t^{13}-26886821116994799 t^{12}-11711966074393796 t^{11}-4043688238979169 t^{10}-1134286245292513 t^9-260744304879767 t^8-49128772280730 t^7-7540994016016 t^6-931329867651 t^5-90682059115 t^4-6737875325 t^3-361470940 t^2-12575053 t-215095\right)+d^{41} \left(-84023771972 t^{78}-123558119347 t^{77}+2323753029285 t^{76}-3222431441804 t^{75}-22169136673226 t^{74}+63588920469102 t^{73}+63189318112525 t^{72}-507040506783374 t^{71}+305854722916484 t^{70}+2185015134438709 t^{69}-4156089816034338 t^{68}-5557960970562974 t^{67}+22637936491387761 t^{66}+2882426648349691 t^{65}-87861143237719051 t^{64}+38786561017532789 t^{63}+265798948073597677 t^{62}-221315726746930797 t^{61}-694589776658995770 t^{60}+737529423204796308 t^{59}+1606557326912024824 t^{58}-1877924790232665347 t^{57}-3356982139664650075 t^{56}+4033651906926322504 t^{55}+6787267746600011080 t^{54}-6662093953109129202 t^{53}-11613748446007270632 t^{52}+10732416838902089590 t^{51}+21041101379310351429 t^{50}-10287761765555214579 t^{49}-28455304476538064653 t^{48}+10949017355872550724 t^{47}+40894135705051828923 t^{46}-2081791910438635527 t^{45}-48903894289586548172 t^{44}-17661605126226265093 t^{43}+33660138613062584483 t^{42}+11615403692767118831 t^{41}-46451692750068089417 t^{40}-42588315562352438367 t^{39}+18170612132960649500 t^{38}+51485928039798086901 t^{37}+31965276058953265430 t^{36}+10241658801976558444 t^{35}+16339401340429323549 t^{34}+22410236675799809661 t^{33}+453242163132145837 t^{32}-34242737604458599303 t^{31}-48839166451044502204 t^{30}-34192087088310650896 t^{29}-7777998090808435595 t^{28}+10656873399294327406 t^{27}+15217754547906207971 t^{26}+11114647497249139144 t^{25}+5265626551036062917 t^{24}+1260762823214313849 t^{23}-461001621635482568 t^{22}-760640401710897659 t^{21}-522529507470220315 t^{20}-241760253927426924 t^{19}-74456511378184060 t^{18}-8566663503913394 t^{17}+6462365219408632 t^{16}+5533976594498729 t^{15}+2715219324680542 t^{14}+1073243420104194 t^{13}+385552205998421 t^{12}+132146055883958 t^{11}+42671230874569 t^{10}+12433286213747 t^9+3138130052955 t^8+666603197970 t^7+116665709714 t^6+16483582628 t^5+1832876289 t^4+154515585 t^3+9290958 t^2+355334 t+6501\right)+d^{17} \left(-70421578188 t^{78}+2743870152127 t^{77}-48844525849353 t^{76}+518757685756987 t^{75}-3569058073848063 t^{74}+15770234161624205 t^{73}-37256234572698490 t^{72}-19123565892960925 t^{71}+474529538113037033 t^{70}-1465186265011474002 t^{69}+517484516430551093 t^{68}+9303627343203405189 t^{67}-24727648653554779875 t^{66}-5228956235066984503 t^{65}+143396861140415576156 t^{64}-201064281267127625047 t^{63}-377420176169356895454 t^{62}+1330313310838503266529 t^{61}+27651480500033554896 t^{60}-4985416654212289743661 t^{59}+4266584556284161348955 t^{58}+13104213659881791124199 t^{57}-22271924903930855712691 t^{56}-24928635712353052009300 t^{55}+75294843059137601701896 t^{54}+30137421750192730250797 t^{53}-200583094908602762581435 t^{52}+566638804927933886895 t^{51}+451373288660131392599270 t^{50}-120383209667432425479301 t^{49}-889574266154478542853800 t^{48}+394278880427543640326964 t^{47}+1570976195399690458414648 t^{46}-860233082341444754197315 t^{45}-2524131671633759725480473 t^{44}+1473235403657223913337040 t^{43}+3721464201988444417320094 t^{42}-2071039767138746917251896 t^{41}-5045497412617013554328720 t^{40}+2414374393702042799703935 t^{39}+6279869638417762146899630 t^{38}-2310877538464301205800268 t^{37}-7179515927844768894044072 t^{36}+1725755008500615474195698 t^{35}+7611942640630914631947181 t^{34}-730007192853805269164512 t^{33}-7600340166360635113467896 t^{32}-674289754672248992105380 t^{31}+7101760016574532608557954 t^{30}+2515467514483464679529886 t^{29}-5757917086414782955754558 t^{28}-4442282894064275696100507 t^{27}+3129663844285426889168182 t^{26}+5395424461098683744828611 t^{25}+517655434704498481786969 t^{24}-3962192389727636266895604 t^{23}-3266150229305423588689241 t^{22}+210516159126721283498019 t^{21}+2311090957844837302957376 t^{20}+1970925057273602433515059 t^{19}+667124358036878628967203 t^{18}-196444549604643869753184 t^{17}-364486140491989067168379 t^{16}-211000902973736873427746 t^{15}-58789600605715896052782 t^{14}+4801365293061330883414 t^{13}+13208971572961703445807 t^{12}+6875629041600873007764 t^{11}+2025375808400594449902 t^{10}+280508147130146993744 t^9-51314257905678547884 t^8-43456055790186123170 t^7-14352855815625201674 t^6-3153850961731445692 t^5-501612446021805735 t^4-58131000927518449 t^3-4731233125924127 t^2-245221830877788 t-6168215017783\right)+d^{27} \left(-64686955256 t^{78}+2011468094794 t^{77}-39628524077656 t^{76}+491408234400798 t^{75}-3754387861492352 t^{74}+17283975076628426 t^{73}-40093151025418846 t^{72}-20555443550446946 t^{71}+431168133635363500 t^{70}-1059344050755139436 t^{69}-387568219822568638 t^{68}+7239575946790926468 t^{67}-10890461594586452429 t^{66}-19348182911011203679 t^{65}+77221208906652393767 t^{64}-8672822831198162259 t^{63}-305179335314693976014 t^{62}+310474106199571949926 t^{61}+863735331088358849692 t^{60}-1648137778423874983390 t^{59}-1875716880183431063060 t^{58}+5991752748605131865890 t^{57}+3137211280108890715880 t^{56}-17597640881032383045363 t^{55}-3946381951315770354375 t^{54}+44213425060900055077138 t^{53}+4317281911497439115133 t^{52}-97364223008538629376210 t^{51}-9937611980066793892297 t^{50}+188936902172724490070286 t^{49}+41839745597842419648524 t^{48}-318544993606156917850407 t^{47}-143948398919801867371789 t^{46}+446715993298647396543180 t^{45}+367257754735092545419690 t^{44}-465180262145883264153177 t^{43}-705065676780337831751091 t^{42}+212144167471812249176488 t^{41}+991979584689213416624793 t^{40}+391088675666199613630822 t^{39}-894979863580668501495219 t^{38}-1118676179720721431337252 t^{37}+149482745042310526982852 t^{36}+1354747906765289103107675 t^{35}+940755365457335433984853 t^{34}-610169237352028123463203 t^{33}-1441697994218837442523531 t^{32}-690994215074241272756671 t^{31}+701102042742448596329180 t^{30}+1457835979821017651305625 t^{29}+1349458147093114707093427 t^{28}+927486988037006871632194 t^{27}+590441876468468067749198 t^{26}+328049548400811112278845 t^{25}+62184209449016462711368 t^{24}-150298842680318930573031 t^{23}-228314710162588112494995 t^{22}-187464074352073372968602 t^{21}-108263369779019244792778 t^{20}-50736723245397676037413 t^{19}-25483290639578062888717 t^{18}-17575260737296704345429 t^{17}-13513709166802010810559 t^{16}-8998284306167610729645 t^{15}-4776878854849492965711 t^{14}-1960639652177462384540 t^{13}-586583141919661470910 t^{12}-100473713448997387917 t^{11}+10585733693237000666 t^{10}+15701147590934861123 t^9+6892105064719860474 t^8+2053617765795860178 t^7+466661912323846323 t^6+83385659199133727 t^5+11684491007699164 t^4+1248046104209172 t^3+95674600807278 t^2+4676289484183 t+108979468467\right)+d^{42} \left(-43162327208 t^{78}-186718425868 t^{77}+1157822293277 t^{76}+1606225505937 t^{75}-16941477233628 t^{74}+762435326210 t^{73}+123511421661170 t^{72}-107264988222500 t^{71}-602007753106047 t^{70}+825681433047193 t^{69}+2013738020982923 t^{68}-4060508450742656 t^{67}-5255505803979330 t^{66}+14052807001709392 t^{65}+9430213982376131 t^{64}-39945500722142722 t^{63}-10739839871781109 t^{62}+91391584602903789 t^{61}-7352135508067654 t^{60}-176632330049126044 t^{59}+82969822302276552 t^{58}+311904183500403404 t^{57}-230014543887227875 t^{56}-400078587134433292 t^{55}+690470358214323435 t^{54}+744717026569557708 t^{53}-1024699926162592760 t^{52}-608916690933022244 t^{51}+2368695876235325847 t^{50}+1613176661570512059 t^{49}-2813881356960907000 t^{48}-2148189293336896562 t^{47}+3223861355075407664 t^{46}+1970601653497727833 t^{45}-6059660017466723804 t^{44}-7451113414959020652 t^{43}+130187673016806860 t^{42}+3509498550865935468 t^{41}-1439548131480643713 t^{40}-2636204864840130188 t^{39}+5885482322022942448 t^{38}+13475778938365807767 t^{37}+10479601620583903027 t^{36}+1567474902089616382 t^{35}-4333343910471886512 t^{34}-6371735702136375910 t^{33}-8170560171166764736 t^{32}-9429838712563419774 t^{31}-7098562876798262181 t^{30}-1408217787925770945 t^{29}+3717747672288231320 t^{28}+5271163947682076355 t^{27}+3723947646552923442 t^{26}+1394170120191959258 t^{25}-87749208764632798 t^{24}-517388859917654022 t^{23}-400765409094622716 t^{22}-189294339669496708 t^{21}-56039572027901057 t^{20}-2912964454550804 t^{19}+9225753973220804 t^{18}+7700420550604901 t^{17}+4070361862700385 t^{16}+1580150410035627 t^{15}+415767059757526 t^{14}+31688666440007 t^{13}-37811328548394 t^{12}-26410444615760 t^{11}-10809645174630 t^{10}-3298370437934 t^9-797613667303 t^8-155924953494 t^7-24708014172 t^6-3146931609 t^5-315988119 t^4-24179489 t^3-1329286 t^2-46888 t-799\right)+d^{16} \left(-31927341732 t^{78}+1272215256728 t^{77}-23139524426070 t^{76}+250671122062426 t^{75}-1752658893203771 t^{74}+7791078756258727 t^{73}-17649508850152315 t^{72}-19574820880899829 t^{71}+293341463968659874 t^{70}-889602166533207276 t^{69}+265210670499275532 t^{68}+6217857508350459241 t^{67}-17252056469783772564 t^{66}-1449967358180295859 t^{65}+101715410244664024599 t^{64}-168442837500777249911 t^{63}-230135979715276052813 t^{62}+1067075580232738493688 t^{61}-363169287907014254660 t^{60}-3706460372466490694322 t^{59}+4945381772488099230701 t^{58}+8169662509073439460078 t^{57}-22049100137296962926655 t^{56}-9155143613876626942496 t^{55}+67880797083420398573665 t^{54}-12269631125329834200324 t^{53}-166234274010557049818199 t^{52}+98674173567137062507630 t^{51}+344861949328371046192465 t^{50}-322227436076542875530500 t^{49}-630513906355707490831066 t^{48}+777857587804053021930196 t^{47}+1048461460466412493475043 t^{46}-1555633187016310877677325 t^{45}-1632059742020414957089234 t^{44}+2691598181797369817014579 t^{43}+2439930282818349787533921 t^{42}-4108767273924393625425439 t^{41}-3565424749660541918462399 t^{40}+5569873620599163328734292 t^{39}+5114867704806494920455854 t^{38}-6661067092064775464059465 t^{37}-7130751319019160337749822 t^{36}+6819163270022255924854420 t^{35}+9438007158644449531615993 t^{34}-5444902786753571304103645 t^{33}-11431133265932148825572716 t^{32}+2214845969801900400722670 t^{31}+11987524397230251511241113 t^{30}+2366288749235486207195478 t^{29}-9896932382041261440801675 t^{28}-6555900297843408918022265 t^{27}+4965340888538965177655226 t^{26}+7896236888230157021009651 t^{25}+897445582983096442084511 t^{24}-5076595112458171058860589 t^{23}-4070544001109823840151165 t^{22}+214485835365393021899610 t^{21}+2503796910916146944458584 t^{20}+1889879738354981089651098 t^{19}+408265050604175665546893 t^{18}-382925028968252837928499 t^{17}-402759632997820061276029 t^{16}-171387158937756863695513 t^{15}-16996031389893862433528 t^{14}+24180314515237875252927 t^{13}+17074707139242005217476 t^{12}+5807404002159771810974 t^{11}+845890820948657027337 t^{10}-211456942720463062059 t^9-172613102418915761176 t^8-57801481209094072373 t^7-12474198590318587330 t^6-1817446599596803531 t^5-163934067056361587 t^4-5241244440137939 t^3+665834375637808 t^2+88644301242801 t+3450722692622\right)+d^{43} \left(-18521594364 t^{78}-135445712155 t^{77}+347508805332 t^{76}+2156613480277 t^{75}-6662724406958 t^{74}-18302792141489 t^{73}+62948049752975 t^{72}+88382927472095 t^{71}-417196362637886 t^{70}-315237595902816 t^{69}+1991002696270797 t^{68}+714324963977830 t^{67}-7711275669867750 t^{66}-1118138616139762 t^{65}+24224158122048321 t^{64}+191146422024268 t^{63}-65131664243543986 t^{62}+3168592037354176 t^{61}+151818002201971057 t^{60}-4377810719790037 t^{59}-303192880281551387 t^{58}+2836624908198258 t^{57}+562878458297736164 t^{56}+83588741665613083 t^{55}-837242308186086954 t^{54}-174856400691534005 t^{53}+1257920550503472137 t^{52}+572651018438452751 t^{51}-1400008666213923030 t^{50}-953755823793555247 t^{49}+1344241712161215230 t^{48}+1173670662418444503 t^{47}-1523398436596582732 t^{46}-2257027480265054562 t^{45}-42593579274721962 t^{44}+1245995570011309481 t^{43}+12083325544413017 t^{42}-803972231990741951 t^{41}+711581434194771044 t^{40}+2596690710238632970 t^{39}+2592616187823588353 t^{38}+1062068874936293486 t^{37}-489320737686329171 t^{36}-1499682022578149925 t^{35}-2145332295487030016 t^{34}-2359670172298062081 t^{33}-1856102225034012971 t^{32}-714067593091683709 t^{31}+508502592505854462 t^{30}+1216991582811559257 t^{29}+1213863961516152904 t^{28}+742561840690574619 t^{27}+209585359809137813 t^{26}-113833838340543999 t^{25}-191729180292977364 t^{24}-132413485394830188 t^{23}-51674608137055473 t^{22}-3845067057756251 t^{21}+10262923348026535 t^{20}+8332077070563770 t^{19}+3675623897981535 t^{18}+919829069297152 t^{17}-8268691421993 t^{16}-135844554021932 t^{15}-79122999256082 t^{14}-30546556773970 t^{13}-9600556643091 t^{12}-2734770681773 t^{11}-752206452929 t^{10}-199503041026 t^9-48502481171 t^8-10222290323 t^7-1792717249 t^6-253800741 t^5-28162606 t^4-2356609 t^3-139891 t^2-5255 t-94\right)+d^{15} \left(-12218700116 t^{78}+495528869303 t^{77}-9147107024272 t^{76}+100069994873562 t^{75}-699390156714858 t^{74}+3021766212025331 t^{73}-5708463892963402 t^{72}-17840927324638676 t^{71}+160311087850480878 t^{70}-442549373216035328 t^{69}-17073274471149664 t^{68}+3807231650286890221 t^{67}-10032671353076632314 t^{66}-2005311567951002792 t^{65}+65493775188585911918 t^{64}-111690943873791195214 t^{63}-146354141814311096133 t^{62}+744252977486516439608 t^{61}-368365004199260384276 t^{60}-2555598602530199708398 t^{59}+4158923055097438431552 t^{58}+4938981254276672427543 t^{57}-18014538412663908879376 t^{56}-1317125526028820163039 t^{55}+53591491347057158334534 t^{54}-29248550736404323384282 t^{53}-124386829107539360760580 t^{52}+131723402508454727849550 t^{51}+238916562639399547475840 t^{50}-381001176190438239980612 t^{49}-395480664241656268675946 t^{48}+878528285766063656606213 t^{47}+588777021626234912462423 t^{46}-1735122970858658326048274 t^{45}-837957930894489548534809 t^{44}+3035310252829033805765492 t^{43}+1234947119902126352198851 t^{42}-4776262243249570634370138 t^{41}-1988854545405464908058916 t^{40}+6775438844436755730820378 t^{39}+3411161216889859556466717 t^{38}-8560861171569118030569935 t^{37}-5764991476778658021389731 t^{36}+9318331948265604621912268 t^{35}+8936026842638574242908629 t^{34}-8063729463459804410423589 t^{33}-12043479148779025877834148 t^{32}+4222526382168341440323209 t^{31}+13393753029350492899688669 t^{30}+1494594788799427958475746 t^{29}-11297449360705280983141551 t^{28}-6662112700050370917419969 t^{27}+5698067319434001700430439 t^{26}+8220621373999399021903953 t^{25}+698199367151800353901654 t^{24}-5141097608691971084082570 t^{23}-3812003767813211392412769 t^{22}+393293962807410529173316 t^{21}+2326230932489150154116582 t^{20}+1518909888129133796935387 t^{19}+138019541786445183796205 t^{18}-448943419875604674855729 t^{17}-347947725339741757671995 t^{16}-104588286586002992071685 t^{15}+17056376878481008723479 t^{14}+31550850982501238589379 t^{13}+14795274893784017959357 t^{12}+3119242312016345522326 t^{11}-344145314438773624606 t^{10}-506633334901598190540 t^9-194472431569318333762 t^8-42690040717105379052 t^7-4724257318028061894 t^6+277078880054196099 t^5+219243369313595643 t^4+44061678017701236 t^3+5005563575663957 t^2+326200576114095 t+9621963364213\right)+d^{44} \left(-6703423740 t^{78}-70604205308 t^{77}+18067117839 t^{76}+1252686697861 t^{75}-1023027055341 t^{74}-13371240606085 t^{73}+13271388132620 t^{72}+87387366888740 t^{71}-116202351768796 t^{70}-436535178523566 t^{69}+651181905682934 t^{68}+1673986266958005 t^{67}-2824913048500785 t^{66}-5433097893839092 t^{65}+9551094016577378 t^{64}+15138675910034363 t^{63}-26541346801821940 t^{62}-37354161473964681 t^{61}+62671552324065332 t^{60}+85729317082137016 t^{59}-120996615333848909 t^{58}-170839313477759569 t^{57}+210647867257701598 t^{56}+331721410591924776 t^{55}-278987210435964132 t^{54}-537189799720596003 t^{53}+327939409137208524 t^{52}+817346787155822001 t^{51}-264670393913455865 t^{50}-1114677916114408263 t^{49}-28416966181938231 t^{48}+1131293613987758396 t^{47}+179879501606460071 t^{46}-1258467606436007234 t^{45}-641656294105418195 t^{44}+987146498871587677 t^{43}+1055107809397812827 t^{42}-145742346842893029 t^{41}-455838608791310481 t^{40}+364997816129553171 t^{39}+694988272150212167 t^{38}-56132630421202205 t^{37}-831447095845355309 t^{36}-807850684336751579 t^{35}-327296153115557376 t^{34}+148933136280623 t^{33}+95886960910950369 t^{32}+164501093897383516 t^{31}+243263138002646865 t^{30}+232134499484421449 t^{29}+118139664558008363 t^{28}-4293633968534972 t^{27}-59784578637494800 t^{26}-52041621155982540 t^{25}-23289345527567103 t^{24}-2886610269015738 t^{23}+4123801430767284 t^{22}+3851983804627007 t^{21}+1925169807593565 t^{20}+579008622900031 t^{19}+16541945407544 t^{18}-108075131010668 t^{17}-81031497942483 t^{16}-36210652614632 t^{15}-10172344267127 t^{14}-755300026873 t^{13}+1019841676010 t^{12}+712743849924 t^{11}+293119978873 t^{10}+89797941273 t^9+21782471184 t^8+4267986097 t^7+677214491 t^6+86256973 t^5+8645740 t^4+658739 t^3+35941 t^2+1253 t+21\right)+d^{14} \left(-3954896162 t^{78}+162240716240 t^{77}-3012925587306 t^{76}+32836170202147 t^{75}-223777264282256 t^{74}+882408677843415 t^{73}-804826391836076 t^{72}-12269575849108793 t^{71}+75703558798780343 t^{70}-176936746430191262 t^{69}-139462973770065861 t^{68}+2083693700072375335 t^{67}-4846369118489439144 t^{66}-2777635224209668550 t^{65}+37862142356458951343 t^{64}-59938900066295901259 t^{63}-96289522972843967583 t^{62}+453655012994868727308 t^{61}-220284259922126460409 t^{60}-1637023662913895243484 t^{59}+2800309800483825297204 t^{58}+3066161525906446187942 t^{57}-12579168825601487775025 t^{56}+783266918050785831878 t^{55}+37749030610733809785090 t^{54}-27789465770220774305562 t^{53}-85947005989864496413065 t^{52}+116755603024112267566727 t^{51}+156225467782787767294815 t^{50}-332687095530934912410203 t^{49}-232698494842983455069124 t^{48}+765012341253719032965701 t^{47}+291609415930996446717689 t^{46}-1517110852948327082899861 t^{45}-333447470730375459992950 t^{44}+2683276949982679013734188 t^{43}+440924487229745966700149 t^{42}-4299738038077798558694571 t^{41}-838625906413894877463799 t^{40}+6249497969155691979903689 t^{39}+1891783473633180295049008 t^{38}-8124202761442421493001947 t^{37}-3950675239055529245090976 t^{36}+9129804659660596685397573 t^{35}+6986669993788246889016352 t^{34}-8242328205868494152261757 t^{33}-10160180552586427499150833 t^{32}+4819986331240294640973920 t^{31}+11774791903187096857857840 t^{30}+480693736907042788491510 t^{29}-10152574298597248679876864 t^{28}-5313488737568507689322447 t^{27}+5281673754933359887173110 t^{26}+6842350657224142174087375 t^{25}+243700914652215776098373 t^{24}-4335294888152783181857901 t^{23}-2889662392693059255594160 t^{22}+541400030825352204965177 t^{21}+1851592620988168791866380 t^{20}+1025343598969681492701406 t^{19}-51089588068981963568248 t^{18}-399920900074289538272420 t^{17}-243558053719132207053120 t^{16}-43000055325921499259288 t^{15}+32411158166859697131218 t^{14}+27658994161977439879684 t^{13}+9366410150552958273950 t^{12}+589222730069074151293 t^{11}-961328051689091057132 t^{10}-518802555219399249346 t^9-137535154486245479977 t^8-15997092037821816049 t^7+2535401921356982689 t^6+1623803086320853769 t^5+391390310233056378 t^4+58192456230434061 t^3+5581007035632148 t^2+320756890179115 t+8480892719613\right)+d^{45} \left(-2047600516 t^{78}-28878932241 t^{77}-47125667253 t^{76}+477280491480 t^{75}+473917663550 t^{74}-5531015206594 t^{73}-2979316137905 t^{72}+39137661968518 t^{71}+5479466440883 t^{70}-210588813191919 t^{69}+12199564153042 t^{68}+865703312894429 t^{67}-165051722689061 t^{66}-2942208028097200 t^{65}+695849892304318 t^{64}+8459575952659635 t^{63}-1785961392788228 t^{62}-20746584553510621 t^{61}+3473886018470147 t^{60}+45600841482553019 t^{59}-1603400483210682 t^{58}-84961313580204875 t^{57}-6131022878400233 t^{56}+144894134653568051 t^{55}+36787628542392397 t^{54}-209352149695551259 t^{53}-94672007950403570 t^{52}+256941958017186880 t^{51}+167643421070305716 t^{50}-290406387030535188 t^{49}-290874544236499852 t^{48}+215646429485477100 t^{47}+344528016788282319 t^{46}-113565292827973943 t^{45}-329993103322310234 t^{44}+57360150366250701 t^{43}+377268193327939646 t^{42}+153742467910287077 t^{41}-192568024037450983 t^{40}-184770087406778409 t^{39}+8175714088851312 t^{38}+27687011879174348 t^{37}-96749844208862912 t^{36}-124858950180798427 t^{35}-15239679743729518 t^{34}+85025251409036781 t^{33}+89241675749004780 t^{32}+41046275983702978 t^{31}+5037744516081715 t^{30}-5659332669530539 t^{29}-6837360312501909 t^{28}-7336758293714291 t^{27}-6155551212236803 t^{26}-2851046975700438 t^{25}+201063088184932 t^{24}+1333661435443188 t^{23}+985582821224063 t^{22}+322291495173418 t^{21}-39109771558031 t^{20}-101828848710792 t^{19}-55389482442088 t^{18}-13760870537810 t^{17}+1637101499271 t^{16}+3082038185404 t^{15}+1440906163753 t^{14}+361275694367 t^{13}+15997950033 t^{12}-30847139413 t^{11}-16941643971 t^{10}-5599447626 t^9-1374630055 t^8-265164865 t^7-40858860 t^6-5018310 t^5-483366 t^4-35346 t^3-1851 t^2-62 t-1\right)+d^{13} \left(-1077972532 t^{78}+44367880731 t^{77}-818758565689 t^{76}+8704315857100 t^{75}-55299897633102 t^{74}+168613995353058 t^{73}+356495539758863 t^{72}-6339840529371466 t^{71}+29696329120437471 t^{70}-52648256610887571 t^{69}-131649325180091318 t^{68}+986563715385879377 t^{67}-1881643825258242966 t^{66}-2542194780749771630 t^{65}+19236601003828334426 t^{64}-25507884370215086098 t^{63}-60943772196161634085 t^{62}+239779092673378191234 t^{61}-79986068078957025208 t^{60}-959458636687665297727 t^{59}+1547333270348388469176 t^{58}+1945102635655371220785 t^{57}-7582374708890271370462 t^{56}+387716883867955468084 t^{55}+23782190504604338148700 t^{54}-18584926523504408729581 t^{53}-55049952007443367607845 t^{52}+81071256733382642491673 t^{51}+98461455442231924500951 t^{50}-236614886439218435133172 t^{49}-136579501405378804528323 t^{48}+553247175962661825582005 t^{47}+141627379307419779051832 t^{46}-1111280893762001578347617 t^{45}-101750919244667651173230 t^{44}+1988861445044676628318677 t^{43}+71742540553561493432819 t^{42}-3228691158108606286654663 t^{41}-229147168345082271000375 t^{40}+4764526334874682340269170 t^{39}+882831842555690689963997 t^{38}-6303033404518387326701740 t^{37}-2352033414135301073969086 t^{36}+7230450114883653611689801 t^{35}+4665376870285446079283511 t^{34}-6721749191761400798237247 t^{33}-7195763836821092167965728 t^{32}+4231526919191410632510138 t^{31}+8613230812004223576237805 t^{30}-236318601545742789994584 t^{29}-7593125438786192772898843 t^{28}-3466554193460682128503610 t^{27}+4119588205142994844224756 t^{26}+4745118826512669951985137 t^{25}-141047609950119703904916 t^{24}-3111629163422848952521624 t^{23}-1817414051046673403089953 t^{22}+553734394438651335130982 t^{21}+1264177054806632012379206 t^{20}+577351206805547240837131 t^{19}-130466769352991920043334 t^{18}-288225094267993050480017 t^{17}-138993928229586506976052 t^{16}-4610222483415314190503 t^{15}+30984176841125880366775 t^{14}+18406333460283690204769 t^{13}+4205306614708140026087 t^{12}-778045928654361334162 t^{11}-961799129915008857927 t^{10}-357263675021988506443 t^9-62218785924949143539 t^8+3586232823080786675 t^7+5511510688170256802 t^6+1749380992333405215 t^5+334029859226639369 t^4+42485010531315966 t^3+3546031435629715 t^2+176173826170337 t+3921245279533\right)+d^{46} \left(-524831570 t^{78}-9550637648 t^{77}-32111463426 t^{76}+122586519259 t^{75}+408344961364 t^{74}-1450468796497 t^{73}-3438769535384 t^{72}+10282896829207 t^{71}+17873309591775 t^{70}-56212145376438 t^{69}-75471145498589 t^{68}+231271770911927 t^{67}+260756103516204 t^{66}-769065561260118 t^{65}-783613276672618 t^{64}+2139478902627431 t^{63}+2176273175825169 t^{62}-4872508010665717 t^{61}-5185018526613380 t^{60}+9767000899291935 t^{59}+11746168100526098 t^{58}-15740157916370127 t^{57}-22521908781110603 t^{56}+21678782916759735 t^{55}+38725004664147039 t^{54}-23822606104269591 t^{53}-59908322837264540 t^{52}+13889793311262872 t^{51}+73354240689896416 t^{50}-483937487108456 t^{49}-83397083073502770 t^{48}-23296044592199202 t^{47}+79720414726096748 t^{46}+55050599380179133 t^{45}-41693531270540469 t^{44}-48474937386115079 t^{43}+24497670985354503 t^{42}+44839535800089847 t^{41}-11436078223556746 t^{40}-51130225775423541 t^{39}-28657762454218961 t^{38}+8912579550366637 t^{37}+17134057782156381 t^{36}+6460016371013578 t^{35}+2082414103393457 t^{34}+5748463488045790 t^{33}+6490839592790365 t^{32}+1760977702238643 t^{31}-2736448870401660 t^{30}-3354047450791075 t^{29}-1523315092295630 t^{28}+93175445127591 t^{27}+555429808159468 t^{26}+347494207768948 t^{25}+83913732528014 t^{24}-25990882628165 t^{23}-32034423107031 t^{22}-13492345741481 t^{21}-2226656881422 t^{20}+765467044655 t^{19}+674877448792 t^{18}+243765686426 t^{17}+47234076921 t^{16}-31769619 t^{15}-3604635206 t^{14}-1479549214 t^{13}-377165303 t^{12}-70323024 t^{11}-9978967 t^{10}-1078753 t^9-86740 t^8-4917 t^7-176 t^6-3 t^5\right)+d^{12} \left(-244979916 t^{78}+10000119124 t^{77}-179909619741 t^{76}+1796747676109 t^{75}-9561801361133 t^{74}+6483215328867 t^{73}+305926074297132 t^{72}-2467547343066124 t^{71}+9122871900811148 t^{70}-8509060153050334 t^{69}-79311516982573854 t^{68}+390675408073638241 t^{67}-536861263358619787 t^{66}-1696671333777299455 t^{65}+8374319489902374649 t^{64}-7922812334429426227 t^{63}-34585359129587627402 t^{62}+108110909123799428679 t^{61}-3865691622496534358 t^{60}-502883743707782211727 t^{59}+697279615512726584141 t^{58}+1187336027257482930579 t^{57}-3935185900822809418754 t^{56}-318985322634145856739 t^{55}+13307086477962655617372 t^{54}-9477327854475250315916 t^{53}-32330309660354221322077 t^{52}+46103718836861024743972 t^{51}+59393340986375504816666 t^{50}-141550202304386421420466 t^{49}-82005551024483372382519 t^{48}+341335162844469727181180 t^{47}+77866144721280113920534 t^{46}-699519380711713701486476 t^{45}-31791884794691193264251 t^{44}+1269345737635203151699581 t^{43}-28477392969203916830187 t^{42}-2083023597711049487745965 t^{41}-9861359253018599468038 t^{40}+3105294738332579416611384 t^{39}+356294205095156245752636 t^{38}-4154298209073605798283113 t^{37}-1240149062573915463563004 t^{36}+4833515604672096494001746 t^{35}+2708041902378273808457423 t^{34}-4595905728861248339615946 t^{33}-4372823378027117134124349 t^{32}+3065473698836503048695754 t^{31}+5374212290711741297548214 t^{30}-529064348858601821551154 t^{29}-4844364813637497975911165 t^{28}-1871250855615704488835018 t^{27}+2755428268741401348796688 t^{26}+2789152282563237121445613 t^{25}-312920482537073518779669 t^{24}-1919606943553809980187077 t^{23}-951961038699404248940150 t^{22}+446230796918993081204875 t^{21}+740028271391504494063120 t^{20}+265477850198623692732694 t^{19}-127259410776403465410951 t^{18}-171825059238986910302608 t^{17}-63617353463946225569526 t^{16}+10306284062468457493275 t^{15}+21415148265317723131149 t^{14}+9559614162843103911063 t^{13}+1041117584906738345271 t^{12}-1030455065000110075047 t^{11}-647650574682122202206 t^{10}-176217870129223345123 t^9-11646350934356458029 t^8+10105620622467590421 t^7+4752450184018777226 t^6+1167198490211679129 t^5+187360970575447329 t^4+20113140410442445 t^3+1368967982105431 t^2+50776310886936 t+656469501825\right)+d^{47} \left(-111543748 t^{78}-2575692693 t^{77}-13013006608 t^{76}+17300957654 t^{75}+161093454378 t^{74}-199202149045 t^{73}-1384816465302 t^{72}+1257239916496 t^{71}+7610083092970 t^{70}-6656417465108 t^{69}-33141123726152 t^{68}+25365523360337 t^{67}+117054039001461 t^{66}-72376786138265 t^{65}-341845568067635 t^{64}+168895527779790 t^{63}+881244171703322 t^{62}-244702043531028 t^{61}-1887997065299954 t^{60}+215670526987442 t^{59}+3617036002078164 t^{58}+372296584307578 t^{57}-5882006213190492 t^{56}-1981918462170107 t^{55}+7910506027774991 t^{54}+4380758627170124 t^{53}-9537442566267330 t^{52}-8440541768636762 t^{51}+8282569412372410 t^{50}+11709444765355992 t^{49}-4383853226429754 t^{48}-11702396112117776 t^{47}+1746987640413522 t^{46}+12400445904308621 t^{45}+3871615248050581 t^{44}-8524633659787742 t^{43}-7543581287901736 t^{42}+791938482323295 t^{41}+3051237688191106 t^{40}-732739343903692 t^{39}-2383799652800591 t^{38}+222900383888336 t^{37}+2716392979684214 t^{36}+2281694093424707 t^{35}+343901889921323 t^{34}-830153272079863 t^{33}-769025101299375 t^{32}-257928512293241 t^{31}+60593488628529 t^{30}+108540384343255 t^{29}+52566410177851 t^{28}+8203385009912 t^{27}-5160142798152 t^{26}-4155989792666 t^{25}-1410158574887 t^{24}-168945359672 t^{23}+78626287175 t^{22}+52814008031 t^{21}+16529848209 t^{20}+3114077329 t^{19}+251691504 t^{18}-50285960 t^{17}-23456219 t^{16}-4877875 t^{15}-667426 t^{14}-63454 t^{13}-4088 t^{12}-162 t^{11}-3 t^{10}\right)+d^{11} \left(-45673036 t^{78}+1816460097 t^{77}-30805014844 t^{76}+265526685077 t^{75}-744450687018 t^{74}-8862719901617 t^{73}+121461830019367 t^{72}-707762978174301 t^{71}+1951362083174354 t^{70}+1585107404589044 t^{69}-35215901388622447 t^{68}+124082308087223110 t^{67}-78112258417792249 t^{66}-870685460075416051 t^{65}+3026893265017516492 t^{64}-1232935958903089961 t^{63}-16820114105475933796 t^{62}+40479132764939525834 t^{61}+18522900151933855795 t^{60}-229912300688780114281 t^{59}+246784916037261443021 t^{58}+654128247356736185464 t^{57}-1737990559013385997968 t^{56}-581312319059692550180 t^{55}+6530107939631386288481 t^{54}-3619958834448176587405 t^{53}-17086761123934426404772 t^{52}+21650191273412595488237 t^{51}+33353618503444075360303 t^{50}-71873465409247144623585 t^{49}-48707154575846603144142 t^{48}+181231022705575961421362 t^{47}+49230348510100586365058 t^{46}-381858699185427433113304 t^{45}-22484998276343892697277 t^{44}+704931253461638429562429 t^{43}-21400062724745680732424 t^{42}-1169245076944462766839465 t^{41}+23261254428581950151208 t^{40}+1756280058940019961533803 t^{39}+135063176760575957000643 t^{38}-2366752483592912551782600 t^{37}-589726464982137119197878 t^{36}+2781356800193166862277382 t^{35}+1380333596347368421757533 t^{34}-2693614316237641838269956 t^{33}-2305275075566059404205787 t^{32}+1886978714775126774556592 t^{31}+2895041655713194331037696 t^{30}-507845014908920911081819 t^{29}-2668122624016587408693503 t^{28}-829012376372828297322160 t^{27}+1594680784681670810070702 t^{26}+1397222417496618875377785 t^{25}-302632878854344858678384 t^{24}-1021027411751417598193628 t^{23}-409990870676092532354056 t^{22}+293464372521637488290816 t^{21}+370006876822420677568031 t^{20}+94477828730488883500713 t^{19}-87940448265846760895200 t^{18}-85126459626849899765461 t^{17}-22112266358706209896353 t^{16}+11021507286331937479662 t^{15}+11536261524301224419159 t^{14}+3818287527173623432485 t^{13}-202025670896627619031 t^{12}-731299852946465605166 t^{11}-322865871804976538407 t^{10}-59300536304702910260 t^9+7354444377135101443 t^8+8189831134849896772 t^7+2714184782531295893 t^6+546302445627887099 t^5+71816205683166934 t^4+5841097424583625 t^3+227097298760774 t^2-2229746519143 t-386947825819\right)+d^{48} \left(-19278420 t^{78}-564539816 t^{77}-3823644630 t^{76}-1143958786 t^{75}+41134312981 t^{74}+13510668919 t^{73}-335060004559 t^{72}-158712552381 t^{71}+1755577928050 t^{70}+886464350134 t^{69}-7163238630330 t^{68}-4013060833223 t^{67}+23681847854678 t^{66}+16349885880492 t^{65}-61708728111262 t^{64}-50193578501280 t^{63}+139654768423215 t^{62}+142811225587024 t^{61}-248223048915098 t^{60}-323761021010261 t^{59}+361685971820334 t^{58}+620232149064008 t^{57}-418055693617948 t^{56}-1055067306378318 t^{55}+220686905345484 t^{54}+1374861103296446 t^{53}+127679655954997 t^{52}-1521366748260990 t^{51}-581600437271956 t^{50}+1473433705849815 t^{49}+1267780050555136 t^{48}-683761383988831 t^{47}-1255373605962506 t^{46}-3909147020562 t^{45}+758886925718950 t^{44}+52637318419771 t^{43}-749758025975563 t^{42}-518582187075788 t^{41}+232284059756308 t^{40}+558278370054546 t^{39}+326254497386803 t^{38}-8749219721091 t^{37}-136849900704169 t^{36}-92855831078586 t^{35}-21081643175057 t^{34}+10698829842975 t^{33}+11205106927709 t^{32}+4307812761308 t^{31}+412933002816 t^{30}-438684539343 t^{29}-273844175625 t^{28}-80114958465 t^{27}-9321470810 t^{26}+2689254261 t^{25}+1729804935 t^{24}+494562750 t^{23}+91922025 t^{22}+11432440 t^{21}+821520 t^{20}+921 t^{19}-7119 t^{18}-816 t^{17}-44 t^{16}-t^{15}\right)+d^{10} \left(-6814952 t^{78}+256147780 t^{77}-3810619503 t^{76}+20948521513 t^{75}+150206290144 t^{74}-3655618917178 t^{73}+31089285383926 t^{72}-138378554449940 t^{71}+176121865979313 t^{70}+1736138660933609 t^{69}-11796847369484545 t^{68}+29262772765514256 t^{67}+19624057726877838 t^{66}-348677974987979710 t^{65}+864236194092783084 t^{64}+377698911799198835 t^{63}-6802434780508796365 t^{62}+11982530593648926695 t^{61}+15861352304572128386 t^{60}-89305050265096839210 t^{59}+61058116567049054232 t^{58}+311394655687056177510 t^{57}-638883316889064409997 t^{56}-477598111686279408796 t^{55}+2764510087583100793546 t^{54}-887774738035888274308 t^{53}-7960527437765122164744 t^{52}+8275863190673651973886 t^{51}+16880166391844490929062 t^{50}-30863012268249929134799 t^{49}-26955440256679645059350 t^{48}+82723137652001316272050 t^{47}+31218749437547659014328 t^{46}-180847147412983216765246 t^{45}-21879668072404888435658 t^{44}+341318585455186992340829 t^{43}+783616662451670896121 t^{42}-573209417425531530678541 t^{41}+6415731766792494013138 t^{40}+866904609099017811634149 t^{39}+56409837347718834123868 t^{38}-1174195650289234680826311 t^{37}-257388307705278122050080 t^{36}+1389967200973887401643377 t^{35}+621493184903250197105281 t^{34}-1367252180719544811847745 t^{33}-1059642887403857608334468 t^{32}+1000318376919037942673516 t^{31}+1353597538045843292912044 t^{30}-353141300449781730616876 t^{29}-1274973193341939697678438 t^{28}-291121197462549071083676 t^{27}+801103950179918245402511 t^{26}+595000635206385670751614 t^{25}-209854331863879826124799 t^{24}-467408271092695235592510 t^{23}-139652535971976994770835 t^{22}+160298057194720458889348 t^{21}+156646914870722228605627 t^{20}+21876553961810417604231 t^{19}-47665428300379872906072 t^{18}-34780979217668254884100 t^{17}-4825503760835564267191 t^{16}+6935895032480589333840 t^{15}+4927582762452844648982 t^{14}+1089327888532534352715 t^{13}-380621296671747493122 t^{12}-368091195923533777526 t^{11}-120355117561365656883 t^{10}-9756101070708955090 t^9+8240757890541003078 t^8+4285209527040172073 t^7+1119598128450859047 t^6+181631553515825548 t^5+17254381250467974 t^4+507165051603476 t^3-84531482501179 t^2-10540316846675 t-394049818125\right)+d^{49} \left(-2627548 t^{78}-99268749 t^{77}-852042037 t^{76}-1369663597 t^{75}+6922711233 t^{74}+13912883757 t^{73}-48656342014 t^{72}-103859806541 t^{71}+216584856501 t^{70}+516153645686 t^{69}-708388050685 t^{68}-1925474607449 t^{67}+1882311171724 t^{66}+6188505274435 t^{65}-3066452960086 t^{64}-15326913597851 t^{63}+3151968651316 t^{62}+32887018896943 t^{61}+3550248971773 t^{60}-58182445486265 t^{59}-25796625584199 t^{58}+78534018215083 t^{57}+58937005922189 t^{56}-90667840408300 t^{55}-109855848586005 t^{54}+68357509154517 t^{53}+155629959124534 t^{52}+3712086703487 t^{51}-133931967910300 t^{50}-45427113143361 t^{49}+101753020553910 t^{48}+75354143123794 t^{47}-64480522552042 t^{46}-115203659274872 t^{45}-37501814643548 t^{44}+49050359737668 t^{43}+61607087388884 t^{42}+24811373917200 t^{41}-6247303468199 t^{40}-12762745237735 t^{39}-6599346894422 t^{38}-929300212662 t^{37}+873151305382 t^{36}+662591124987 t^{35}+212344982885 t^{34}+15734262248 t^{33}-17519372001 t^{32}-9495415793 t^{31}-2581505361 t^{30}-379201759 t^{29}+54523 t^{28}+15129310 t^{27}+4178589 t^{26}+666771 t^{25}+70535 t^{24}+4921 t^{23}+207 t^{22}+4 t^{21}\right)+d^9 \left(-783476 t^{78}+26180873 t^{77}-273537407 t^{76}-1295061192 t^{75}+65335411378 t^{74}-796617819942 t^{73}+5056487315837 t^{72}-13368328742530 t^{71}-53552918355472 t^{70}+678154819183861 t^{69}-2882247303827426 t^{68}+4023989220136418 t^{67}+18280668541147928 t^{66}-107674445431607393 t^{65}+174463491935413843 t^{64}+381372223112681069 t^{63}-2223110383692387323 t^{62}+2490377820121844135 t^{61}+8246939211168709513 t^{60}-28556036080712316994 t^{59}+5259564940171375749 t^{58}+124528578720153526123 t^{57}-187670885103973477021 t^{56}-272404371216031576221 t^{55}+988795895300705865674 t^{54}-5526312809597044887 t^{53}-3202990765241260124394 t^{52}+2461177271540506319689 t^{51}+7485694651300009994602 t^{50}-11046051761442598028263 t^{49}-13230447813879397961211 t^{48}+32198874842855235029383 t^{47}+17652287109289734964291 t^{46}-73897961529204090287581 t^{45}-16835513470979075059857 t^{44}+143558158068241432374187 t^{43}+10076821364022723576327 t^{42}-244965479224557451161120 t^{41}-6392937953578204375284 t^{40}+373407117517728145605140 t^{39}+28226182869043783743054 t^{38}-508006877333362496034451 t^{37}-104496172283953651790929 t^{36}+604833418185401424477224 t^{35}+247902875365471752411401 t^{34}-603193507165986943313191 t^{33}-425165914240142982857060 t^{32}+459022928082203617613618 t^{31}+549729798661718020845102 t^{30}-196354448051051900700183 t^{29}-528750586008363075357284 t^{28}-72799732371588750810435 t^{27}+348974475100757582202520 t^{26}+213111808203575959969602 t^{25}-115045073018141971780533 t^{24}-182994144846472301944185 t^{23}-33579018043407739226987 t^{22}+73185906052920086259165 t^{21}+55255571351046563951828 t^{20}-21570341628543054635 t^{19}-20857214073564336856019 t^{18}-11462300002920367023075 t^{17}+131273394110357191387 t^{16}+3198981806173245746175 t^{15}+1649900862910648690954 t^{14}+160381561991913317201 t^{13}-231365640218918536939 t^{12}-138703991318038092504 t^{11}-32086354909547122602 t^{10}+2433177314899404899 t^9+4375113558648289973 t^8+1615181802371620375 t^7+338368327064134705 t^6+40415743455404801 t^5+1234644148285436 t^4-449474264737551 t^3-82906896595734 t^2-6529794086729 t-216653554412\right)+d^{50} \left(-268352 t^{78}-13678876 t^{77}-144245887 t^{76}-400075464 t^{75}+651775325 t^{74}+3465525232 t^{73}-2731704010 t^{72}-21327247371 t^{71}+3839778369 t^{70}+92867665263 t^{69}+27787094925 t^{68}-282613439633 t^{67}-163068736440 t^{66}+735153664455 t^{65}+705220476480 t^{64}-1369713521137 t^{63}-1960176959660 t^{62}+1848565614426 t^{61}+4038983098702 t^{60}-1734448376586 t^{59}-7212713618912 t^{58}-833393311362 t^{57}+8987577547070 t^{56}+5072786453352 t^{55}-7392120022814 t^{54}-7715577303726 t^{53}+5052770356083 t^{52}+10808681012528 t^{51}+1317874339091 t^{50}-9395952691541 t^{49}-8592519122887 t^{48}-385902841390 t^{47}+4823359340493 t^{46}+4031737627984 t^{45}+1067497881551 t^{44}-615385044324 t^{43}-711015325322 t^{42}-292361076884 t^{41}-24919127969 t^{40}+37073608215 t^{39}+22819459698 t^{38}+6526589692 t^{37}+640026044 t^{36}-273937591 t^{35}-150197622 t^{34}-39377301 t^{33}-6720037 t^{32}-778405 t^{31}-58840 t^{30}-2518 t^{29}-33 t^{28}+t^{27}\right)+d^8 \left(-65212 t^{78}+1648528 t^{77}+2708936 t^{76}-640865245 t^{75}+11498004314 t^{74}-100119265386 t^{73}+373850602295 t^{72}+1400423901574 t^{71}-26673494775020 t^{70}+160493822769827 t^{69}-451628287687635 t^{68}-219998571448916 t^{67}+6964084516308609 t^{66}-24527341101162185 t^{65}+15263664838174147 t^{64}+166080250833765105 t^{63}-563383065343809228 t^{62}+198895279862728582 t^{61}+3116277576930308559 t^{60}-7168111556135737392 t^{59}-3905805737938541311 t^{58}+40826079221117244681 t^{57}-40237773472314479066 t^{56}-118053238315940002523 t^{55}+290217369324346488707 t^{54}+125831597295424143896 t^{53}-1089131458045526488909 t^{52}+498030994285943361938 t^{51}+2841330871639801754447 t^{50}-3198238691384384059109 t^{49}-5577252543964561504664 t^{48}+10523300604763327337559 t^{47}+8445522480174997572236 t^{46}-25772702143712083059135 t^{45}-9851159605631614736101 t^{44}+52014114649883098041872 t^{43}+8933874757012671737564 t^{42}-90676147512513123070454 t^{41}-8120905078266575420224 t^{40}+139700923276176775003671 t^{39}+14876133915152625847176 t^{38}-191055562408344087181150 t^{37}-39589612464693784960161 t^{36}+228696073098659156459028 t^{35}+87624899760897751726208 t^{34}-230993426856930974199235 t^{33}-148602798063840022776910 t^{32}+182247653869232211611466 t^{31}+193355114849352087878189 t^{30}-90224452882497794240687 t^{29}-189619538680976062427388 t^{28}-7039195975620121607325 t^{27}+131205622725778857053322 t^{26}+62785929434628148054317 t^{25}-51520684505308609256553 t^{24}-60558963784839555075304 t^{23}-2926870976453149751568 t^{22}+27872762003200277611917 t^{21}+15764396681345903434931 t^{20}-3011181948863560668036 t^{19}-7385846219117926262994 t^{18}-2898379281981468277644 t^{17}+684918517568050877560 t^{16}+1129883946761479882051 t^{15}+414257098659520675338 t^{14}-30610702930646897571 t^{13}-91943402631988737321 t^{12}-38973624558552097769 t^{11}-5163291599519704795 t^{10}+2379617033316813292 t^9+1560716214310676953 t^8+450607573969868631 t^7+73634999385175175 t^6+4454502937846568 t^5-950898352065155 t^4-292907532436496 t^3-38179834563955 t^2-2681049095814 t-82289464354\right)+d^{51} \left(-18628 t^{78}-1421477 t^{77}-18108708 t^{76}-70216917 t^{75}-1938456 t^{74}+476887382 t^{73}+409133650 t^{72}-2135686937 t^{71}-2971256058 t^{70}+7180705721 t^{69}+15361604965 t^{68}-12025736851 t^{67}-45817261701 t^{66}+10106889740 t^{65}+110249471249 t^{64}+29355153053 t^{63}-205351045504 t^{62}-168022704834 t^{61}+226626972345 t^{60}+341846350080 t^{59}-147757809419 t^{58}-498260341906 t^{57}-45140569005 t^{56}+602098206846 t^{55}+484069172468 t^{54}-231453659456 t^{53}-618095931880 t^{52}-346181940962 t^{51}+101936405517 t^{50}+265582238000 t^{49}+163045048730 t^{48}+26053255353 t^{47}-28747173837 t^{46}-23960285821 t^{45}-8278942627 t^{44}-619395764 t^{43}+777098625 t^{42}+426200163 t^{41}+116238488 t^{40}+17402938 t^{39}+497711 t^{38}-394985 t^{37}-96473 t^{36}-11482 t^{35}-743 t^{34}-21 t^{33}\right)+d^7 \left(-3500 t^{78}+25305 t^{77}+2966480 t^{76}-85796507 t^{75}+1023855635 t^{74}-4462046396 t^{73}-36495744169 t^{72}+723623879981 t^{71}-5497596516053 t^{70}+21982688957013 t^{69}-20659722761258 t^{68}-281797999722993 t^{67}+1682605460619658 t^{66}-3633705741323193 t^{65}-4396182339171994 t^{64}+47868652157967253 t^{63}-101826985695916128 t^{62}-89981833343974303 t^{61}+882443821068543595 t^{60}-1280726666348535514 t^{59}-2481676069996581275 t^{58}+10635189845793306890 t^{57}-4475999474720689252 t^{56}-39785754720403413385 t^{55}+66604772561337885081 t^{54}+74765409370005006642 t^{53}-304748005274077055578 t^{52}+26576687587907075403 t^{51}+902568051776838435116 t^{50}-703061557389890516623 t^{49}-1974005196898686775077 t^{48}+2812996235592391008139 t^{47}+3347098485266436527779 t^{46}-7541397825968394112215 t^{45}-4502495316332288381995 t^{44}+16020313602529677145644 t^{43}+4966029640383195048023 t^{42}-28757723361358825939667 t^{41}-5153011409001571636478 t^{40}+44990993017790503407316 t^{39}+7071093497558427174238 t^{38}-62000092600041378177150 t^{37}-13844889020075629389618 t^{36}+74671256689547463639842 t^{35}+27370548220481067767470 t^{34}-76358980764290591569196 t^{33}-45016192727912313513643 t^{32}+62290971082847905770543 t^{31}+58516675481234120549307 t^{30}-34623147853533153647681 t^{29}-58364960005764219630617 t^{28}+4399299570571896579486 t^{27}+42218058238024345134145 t^{26}+14536009119093233026055 t^{25}-19032909869602718957052 t^{24}-16615775784163408027675 t^{23}+2009552781628574199774 t^{22}+8769092533270125071003 t^{21}+3420443567856808865451 t^{20}-1736671405605151347614 t^{19}-2084064160608193869450 t^{18}-490748636147949360480 t^{17}+354199121183461811283 t^{16}+303363170332129077367 t^{15}+68618720793746748260 t^{14}-28304106353135923339 t^{13}-25938748997332870854 t^{12}-7788557641811386942 t^{11}-46103465124658807 t^{10}+899780214088689893 t^9+399770607096698711 t^8+94037577478174564 t^7+11032045141875391 t^6-595742360847792 t^5-525894151179300 t^4-109178019575192 t^3-12462344040528 t^2-773259385977 t-19517145881\right)+d^{52} \left(-676 t^{78}-104476 t^{77}-1596776 t^{76}-7927797 t^{75}-9343282 t^{74}+35684232 t^{73}+99212049 t^{72}-50554360 t^{71}-401546061 t^{70}-46361002 t^{69}+1367850673 t^{68}+1231671900 t^{67}-2543697829 t^{66}-4558892705 t^{65}+1920987555 t^{64}+8934477269 t^{63}+1161171649 t^{62}-14392000965 t^{61}-11291233553 t^{60}+12785410537 t^{59}+25604193015 t^{58}+8124689420 t^{57}-17301828227 t^{56}-21783474818 t^{55}-7000938111 t^{54}+6500367652 t^{53}+8531416157 t^{52}+4101186375 t^{51}+394310565 t^{50}-685324985 t^{49}-466508418 t^{48}-146491972 t^{47}-17221180 t^{46}+5366315 t^{45}+3196698 t^{44}+820941 t^{43}+130340 t^{42}+13233 t^{41}+798 t^{40}+22 t^{39}\right)+d^6 \left(-91 t^{78}-4592 t^{77}+280343 t^{76}-4729218 t^{75}+14986203 t^{74}+644096367 t^{73}-12148328777 t^{72}+109307542183 t^{71}-540821666344 t^{70}+769806960125 t^{69}+9157341830999 t^{68}-74887660925542 t^{67}+255062236245224 t^{66}-172862277262557 t^{65}-2209426734953223 t^{64}+9440038376366396 t^{63}-9970301809609703 t^{62}-45924440638757048 t^{61}+182938799756979220 t^{60}-113328914413196708 t^{59}-831543469522205368 t^{58}+2088253781744803942 t^{57}+675510006960249743 t^{56}-10357170903424824128 t^{55}+10768572468556295191 t^{54}+27239421876227637649 t^{53}-67505095379978754076 t^{52}-26977489720655954264 t^{51}+233703193656671906762 t^{50}-97512280751879156935 t^{49}-574254834770444085732 t^{48}+586674839228629929804 t^{47}+1083263750846858925970 t^{46}-1802965062181369763923 t^{45}-1631300004874103605864 t^{44}+4112982860402644961800 t^{43}+2036531214436010045123 t^{42}-7689272647226347670040 t^{41}-2294118158275554259350 t^{40}+12301931927167646377243 t^{39}+2814180476849968537612 t^{38}-17153233830961638573153 t^{37}-4365305181814800876755 t^{36}+20827937932039007524311 t^{35}+7505486456109939465781 t^{34}-21571470084726275163176 t^{33}-11721021095759950793024 t^{32}+18152467663288182414563 t^{31}+15079172694249745749873 t^{30}-11083881669190283278003 t^{29}-15237771706051877602358 t^{28}+3087315180612533825304 t^{27}+11477944575919633235086 t^{26}+2356069312764509289638 t^{25}-5784836373318055661159 t^{24}-3658566537823576396337 t^{23}+1302369899981749680498 t^{22}+2236144572240545872362 t^{21}+472821995953901318836 t^{20}-621879603458238013699 t^{19}-450934383158431508636 t^{18}-22729233916906696903 t^{17}+112385400600001107773 t^{16}+58779148994748221560 t^{15}+3541801877396799006 t^{14}-9559619485915669166 t^{13}-5097952158289907038 t^{12}-972422707714000354 t^{11}+213156707300142119 t^{10}+211653732508026058 t^9+75622647098371298 t^8+15258364902953850 t^7+996337469709241 t^6-441115010189126 t^5-169171840515575 t^4-29709161257731 t^3-2893228398405 t^2-139623480903 t-2052700584\right)+d^{54} \left(t^{78}-104 t^{77}-2323 t^{76}-16758 t^{75}-49640 t^{74}-24853 t^{73}+242228 t^{72}+668215 t^{71}+414976 t^{70}-1270959 t^{69}-2983815 t^{68}-1629136 t^{67}+2946308 t^{66}+5836555 t^{65}+2982774 t^{64}-2726773 t^{63}-5171951 t^{62}-2925912 t^{61}+354925 t^{60}+1654770 t^{59}+1210496 t^{58}+466245 t^{57}+89956 t^{56}-1728 t^{55}-5648 t^{54}-1436 t^{53}-168 t^{52}-8 t^{51}\right)+d^{53} \left(4 t^{78}-4818 t^{77}-88502 t^{76}-537004 t^{75}-1138697 t^{74}+943157 t^{73}+8193582 t^{72}+9492668 t^{71}-14395324 t^{70}-39201360 t^{69}+8242055 t^{68}+105245797 t^{67}+58751184 t^{66}-196481262 t^{65}-318702296 t^{64}+20259517 t^{63}+500887197 t^{62}+480730471 t^{61}-62719599 t^{60}-488728440 t^{59}-397447463 t^{58}-43995848 t^{57}+166538898 t^{56}+152513228 t^{55}+61999095 t^{54}+6228481 t^{53}-6880113 t^{52}-4345990 t^{51}-1349486 t^{50}-255254 t^{49}-28812 t^{48}-1548 t^{47}+12 t^{46}+4 t^{45}\right)+d^{32} \left(23402516280 t^{78}-1854853982640 t^{77}+41260955963260 t^{76}-377634104112512 t^{75}+1611345162243710 t^{74}-1838788879060246 t^{73}-11766109994904934 t^{72}+48818634299968026 t^{71}-17738926438005668 t^{70}-300198549609425497 t^{69}+622431821006786827 t^{68}+683944668922456482 t^{67}-4081417925623584762 t^{66}+2197004864378548072 t^{65}+14907513104895380076 t^{64}-25893544497459962867 t^{63}-30256925516413005048 t^{62}+124033843748641348397 t^{61}-76831790727625005 t^{60}-413234250259527418102 t^{59}+263213447803766240292 t^{58}+1097746148903717897475 t^{57}-1211604211467050228106 t^{56}-2527937670884712382315 t^{55}+3654339712002243676245 t^{54}+5403759307507899908715 t^{53}-8644877530314600079928 t^{52}-11259640350885672108906 t^{51}+16794580028601024392868 t^{50}+22966041652306610010430 t^{49}-26754654548830981500232 t^{48}-44579655767708161572894 t^{47}+32533295990842950749140 t^{46}+78084649699564437028451 t^{45}-22811975023310142959108 t^{44}-117977314091176401575601 t^{43}-15802321990380016598526 t^{42}+144650584929807380599302 t^{41}+86983180394601977401680 t^{40}-122583689193604265729407 t^{39}-153349698869109391072484 t^{38}+57695738541052800317673 t^{37}+207259126784488150947936 t^{36}+101746690085450358870326 t^{35}-74964733165088303523700 t^{34}-71740956673899660011495 t^{33}+79784279956561759099857 t^{32}+160392845076202686186380 t^{31}+71580283642209756740627 t^{30}-83055553432578206029978 t^{29}-164058337760711444441419 t^{28}-138154581216346440155908 t^{27}-62839168831994498144346 t^{26}-950441951326607822465 t^{25}+25217293448119424639197 t^{24}+25353402376747438972740 t^{23}+16366329394895118188698 t^{22}+8416939956050867834433 t^{21}+3962456237597633078881 t^{20}+1925821074662594809071 t^{19}+969049675233422301995 t^{18}+453044165820591993556 t^{17}+181454096333023793104 t^{16}+65465692096080871450 t^{15}+27672497303324795893 t^{14}+16122797588201368981 t^{13}+9940651989628682175 t^{12}+5234188091506521730 t^{11}+2235825885981260749 t^{10}+774812335320742524 t^9+219358894538583631 t^8+50924874342840084 t^7+9675720743557955 t^6+1490813538848916 t^5+182723500479882 t^4+17209608158052 t^3+1171717854245 t^2+51312003392 t+1083038559\right)+d^{37} \left(72986984104 t^{78}+320153000119 t^{77}-12059314026921 t^{76}+53477517128749 t^{75}+42329164405762 t^{74}-825278015891248 t^{73}+1256030998984672 t^{72}+4633009585246966 t^{71}-15262486513852017 t^{70}-7684857550124869 t^{69}+84119100037878371 t^{68}-49912315155620784 t^{67}-277469922337619907 t^{66}+404451273613582835 t^{65}+521872840985393079 t^{64}-1585665169839197707 t^{63}-45343499236729842 t^{62}+4190269955113978224 t^{61}-3926471965915351258 t^{60}-8148912243269547564 t^{59}+18127588486119203734 t^{58}+10974781943710237314 t^{57}-57345504465062966265 t^{56}-8957337383694525138 t^{55}+146368098468002117198 t^{54}-657319777154303713 t^{53}-325200916883138399087 t^{52}+959692227977505376 t^{51}+638219058705672784376 t^{50}+75217994529889745061 t^{49}-1069470007424152845627 t^{48}-272208974337008105017 t^{47}+1671551693525317819049 t^{46}+949455389835133521175 t^{45}-1815563690207745911996 t^{44}-1449099829841766478548 t^{43}+2235081514187015819171 t^{42}+3083744619152087888444 t^{41}-638341316529922140753 t^{40}-2897360550974565179073 t^{39}-287394197019258992250 t^{38}+2441123028587303171170 t^{37}+604632077282470637357 t^{36}-3380167950285182371992 t^{35}-4530616386935532443987 t^{34}-2100080833946756380938 t^{33}+1022317400794800252709 t^{32}+2657122367457738995332 t^{31}+2724808267231153290903 t^{30}+1902341331980741518248 t^{29}+725772046373977550757 t^{28}-336316634955418959106 t^{27}-898244072319755927058 t^{26}-898457535411570955339 t^{25}-589493049414978895013 t^{24}-265740804584070240705 t^{23}-66159984681362302198 t^{22}+15440384704766139722 t^{21}+33185013661077010480 t^{20}+27897595354118675614 t^{19}+18077431467649940628 t^{18}+9843434744237698873 t^{17}+4550822844342942264 t^{16}+1790996538359631437 t^{15}+613529446806308099 t^{14}+195395375937738627 t^{13}+64374160425279395 t^{12}+23154905794134174 t^{11}+8451045243215143 t^{10}+2807982756686086 t^9+795521135289549 t^8+186517134497172 t^7+35598774113870 t^6+5443392439988 t^5+652010507339 t^4+59037176385 t^3+3804862709 t^2+155682330 t+3041213\right)+d^{22} \left(128660366807 t^{78}-3855043276488 t^{77}+53590339044047 t^{76}-458513845412806 t^{75}+2695216411522818 t^{74}-11388426282316575 t^{73}+33849345709115558 t^{72}-55574797346645339 t^{71}-67335077092213380 t^{70}+783292949854236287 t^{69}-2342566779526101577 t^{68}+1577581004340256552 t^{67}+11997557903100703816 t^{66}-39521887082953351655 t^{65}+14596389998832648605 t^{64}+181986437901443244055 t^{63}-363661179322157931333 t^{62}-298098189247351118793 t^{61}+1846895464138761349246 t^{60}-815654183424320879061 t^{59}-5719232179297959871299 t^{58}+7071588687531427425318 t^{57}+12711023019272422970114 t^{56}-27028239387036792485755 t^{55}-21622235793552650276565 t^{54}+75626630465902734276414 t^{53}+29342787229440931053440 t^{52}-175700964642942146877911 t^{51}-34234225837746003321607 t^{50}+358198388489712672937176 t^{49}+42494551983534892580267 t^{48}-656884266996945988507228 t^{47}-73024590047429525802394 t^{46}+1093982553855831177487315 t^{45}+153604952025413516649852 t^{44}-1665880334579077256661469 t^{43}-310248098531087845435196 t^{42}+2351805695199160902856645 t^{41}+581878093092641879344899 t^{40}-3136487459316930408272453 t^{39}-1102395906024069111754553 t^{38}+3939214978839279885448799 t^{37}+2162227950626090790608313 t^{36}-4349064255308240406253477 t^{35}-3917909737925515183635640 t^{34}+3495260468295346822670056 t^{33}+5633288242399520339325734 t^{32}-895797524255827000567094 t^{31}-5610037228694552964071749 t^{30}-2052807891631911613652646 t^{29}+3287776776198046914444017 t^{28}+2923197856608584676786283 t^{27}-1146993947410980958721772 t^{26}-2672209319012599249459349 t^{25}-250618824914692780837698 t^{24}+2636736567517823239875376 t^{23}+3244111433893638785568785 t^{22}+2024420835245913241851765 t^{21}+707678964151197823030804 t^{20}+139175384814598629911526 t^{19}+105416907674874751003860 t^{18}+167179569863114533064845 t^{17}+147099622474281992669241 t^{16}+78777803436133013675824 t^{15}+24064547895126271126560 t^{14}+98760135682028823750 t^{13}-4537184161283396162634 t^{12}-2958931359890974639591 t^{11}-1173624920986445428619 t^{10}-325109408087238975977 t^9-60152786142048800413 t^8-4692860797062564195 t^7+1257001262505930044 t^6+588888155881219725 t^5+128221615855876361 t^4+17931847151352795 t^3+1641584372271937 t^2+90276416427511 t+2269227608972\right)+d^{36} \left(384932548504 t^{78}-2459505097528 t^{77}-9758661939149 t^{76}+127353109159917 t^{75}-319593113228708 t^{74}-625405437816492 t^{73}+4518167849684387 t^{72}-3996736379153446 t^{71}-24356825421243841 t^{70}+63346262559787054 t^{69}+43329289299532408 t^{68}-381736886278396375 t^{67}+261336719794077101 t^{66}+1398212719983713749 t^{65}-2479069776702307208 t^{64}-3275021936719236361 t^{63}+11551140214198692504 t^{62}+3690537088994060184 t^{61}-39182082727755928645 t^{60}+6371991141397707109 t^{59}+108227755882514868623 t^{58}-47356615949150132176 t^{57}-260299611485284471873 t^{56}+146758668099789668986 t^{55}+562166082705507377293 t^{54}-322587326153506348086 t^{53}-1118378771149329835403 t^{52}+523292828466781995567 t^{51}+2036529312495594340402 t^{50}-571772767100051471875 t^{49}-3342044204733695793390 t^{48}+172942447188869661624 t^{47}+4949727210428813410352 t^{46}+1309524376608831231170 t^{45}-5790762825790030186872 t^{44}-3111853011077153086275 t^{43}+6481013488659809054446 t^{42}+7136336757959235615615 t^{41}-2503147356803402032760 t^{40}-6588227900336203642509 t^{39}+1200272704425728027753 t^{38}+8178353906811710085720 t^{37}+3888184692137847118190 t^{36}-5596846611819235223176 t^{35}-9605956188533143450697 t^{34}-6928116556549678964722 t^{33}-2763814690031271272168 t^{32}+152183731804747862481 t^{31}+2353578252157031552976 t^{30}+3926816298885191558145 t^{29}+3982777542883858435084 t^{28}+2492289213455344604665 t^{27}+586413717702813175777 t^{26}-682830983250050867111 t^{25}-1083028494324015752511 t^{24}-931452142323800689818 t^{23}-599903903819544961471 t^{22}-304036245355122072169 t^{21}-115357145106072287581 t^{20}-24891900033310597976 t^{19}+5105162533694291770 t^{18}+9064093361501507073 t^{17}+6270529937960409919 t^{16}+3517060339120086745 t^{15}+1846765684854057207 t^{14}+916906934865346205 t^{13}+412207849333036029 t^{12}+161179659078011792 t^{11}+53583338256230990 t^{10}+14975673761520465 t^9+3494590841143771 t^8+676307927419529 t^7+107584008733245 t^6+13884396234039 t^5+1425142822676 t^4+112708631376 t^3+6499875338 t^2+245131593 t+4565122\right)+d^{23} \left(520237856200 t^{78}-15674405166886 t^{77}+213613370094560 t^{76}-1708668034356786 t^{75}+8585854206916946 t^{74}-25691074717049516 t^{73}+27551110310400026 t^{72}+109399451447485854 t^{71}-509043138968311830 t^{70}+614230720113210054 t^{69}+1291014060317050500 t^{68}-4853009857291901138 t^{67}+1841332617071569293 t^{66}+13622088692577373827 t^{65}-14764607976807660927 t^{64}-27856247928567090340 t^{63}+28674895250295692855 t^{62}+96793538298560065014 t^{61}-25816016970490110988 t^{60}-425597775813725145570 t^{59}+8903597973048106691 t^{58}+1498342332682434773111 t^{57}+278528643533413454102 t^{56}-4434669517336917688960 t^{55}-2660621760629601671563 t^{54}+12326231830701655500540 t^{53}+13231546585818495757170 t^{52}-32599136717180169881866 t^{51}-45467857258474490856481 t^{50}+76953884660187222734865 t^{49}+120775010148683243474636 t^{48}-151844726600677919304969 t^{47}-260076842938701062978320 t^{46}+238229434289506160389614 t^{45}+456730212213749836833502 t^{44}-283198846605944973328768 t^{43}-633808849007757918060990 t^{42}+251636677770645153258560 t^{41}+641718995844715339691583 t^{40}-245915579216988871525929 t^{39}-405195108842549986757953 t^{38}+535712453601587577381142 t^{37}+201468397674296521264945 t^{36}-1221793802275842474350810 t^{35}-645672135295353571962194 t^{34}+1667859143220451028719491 t^{33}+1829528614189919103150115 t^{32}-824631018426991513231438 t^{31}-2434607062846833373557768 t^{30}-951364514640150521232840 t^{29}+1101596281173837173237466 t^{28}+1120693106053115262273818 t^{27}-27624087761673121622393 t^{26}-132124558665316506500611 t^{25}+1109816219005136952528164 t^{24}+2248999028854080758395404 t^{23}+2245372120597425745955820 t^{22}+1388292456957456553879605 t^{21}+513575320254631295987186 t^{20}+74564276253194500849497 t^{19}+1700726216992859657277 t^{18}+51160571042075697374358 t^{17}+76821446766476979682046 t^{16}+60136854655974222280080 t^{15}+30985872101277377995270 t^{14}+10533392627354794186307 t^{13}+1655559496452458811933 t^{12}-573977364155378922323 t^{11}-559382764624372913543 t^{10}-245051750248527727783 t^9-73826295529483012175 t^8-16492934090622898081 t^7-2761958554172357425 t^6-340626500899010049 t^5-29787010747900684 t^4-1769179399296255 t^3-75132558120960 t^2-3255914724817 t-124826257162\right)+d^{33} \left(654037596008 t^{78}-10160966161442 t^{77}+70006991368526 t^{76}-232566168304950 t^{75}-3048516050826 t^{74}+3168629961600414 t^{73}-10262138197998560 t^{72}-2585902800968546 t^{71}+88143263337023060 t^{70}-146711867584386838 t^{69}-290850253755141055 t^{68}+1148912580584805839 t^{67}-21625566527529526 t^{66}-4524288579041807355 t^{65}+4054550058789802392 t^{64}+10612435668408690965 t^{63}-18360494275178218138 t^{62}-11622755731791583248 t^{61}+44211483077244593949 t^{60}-20627819777204439446 t^{59}-46832759310996739414 t^{58}+152612269315647531689 t^{57}-106971959974797991861 t^{56}-531322799068389923263 t^{55}+725777806308564832381 t^{54}+1493484215498990446464 t^{53}-2324198535594146761066 t^{52}-3823311769411925614004 t^{51}+5365364728836263449829 t^{50}+8992718165701017445951 t^{49}-9605450373631323141125 t^{48}-19240090321685300932494 t^{47}+12554309590341947395052 t^{46}+35977328839646784894507 t^{45}-8829607054369911157844 t^{44}-56919263794784671820063 t^{43}-7928229751610505878794 t^{42}+74547223802432030434097 t^{41}+44187248276819104051360 t^{40}-64980881488026389473784 t^{39}-73048403146888915987522 t^{38}+45994400722015586175688 t^{37}+117593205816919239394803 t^{36}+48183290137779780976544 t^{35}-44251633213326837805722 t^{34}-34657858396043935176463 t^{33}+32622320846763388391993 t^{32}+43208578169162541971685 t^{31}-19191066819202009181467 t^{30}-77984810557609140052098 t^{29}-78694487534331269631373 t^{28}-37322313508085475692188 t^{27}+3305918994328944199486 t^{26}+21417715582949070937611 t^{25}+20864712137034670908049 t^{24}+13270787887261422355584 t^{23}+6182348956205137853809 t^{22}+1897494773317104584786 t^{21}+46935927318422118337 t^{20}-421147391190955273159 t^{19}-363153993861806444165 t^{18}-220088743821602412447 t^{17}-121773258486235907000 t^{16}-67191928967778879813 t^{15}-35681616475915443259 t^{14}-16870924242991870003 t^{13}-6707448089699022016 t^{12}-2159636504331587189 t^{11}-539658840658406353 t^{10}-95024977325980876 t^9-7463534826536393 t^8+1833145350502920 t^7+899681723055646 t^6+207487337763037 t^5+31982875093341 t^4+3447850471842 t^3+252014945917 t^2+11282032869 t+233957861\right)+d^{26} \left(675978136912 t^{78}-17135584266552 t^{77}+179974044276562 t^{76}-912599384191282 t^{75}+1097404554570964 t^{74}+13560826955440832 t^{73}-82783288464394560 t^{72}+158405118101552024 t^{71}+307108486055954390 t^{70}-2173655169493926570 t^{69}+2901889989304403702 t^{68}+7999545054846817600 t^{67}-30936266501440746732 t^{66}+7021655137078511766 t^{65}+135817417365097812901 t^{64}-192255887261884253849 t^{63}-338743028667854825494 t^{62}+1007558451003986566048 t^{61}+382206705270286484480 t^{60}-3444274468332611307922 t^{59}+714019152477316423050 t^{58}+9278220326876406849046 t^{57}-5053788209282806958548 t^{56}-21582078703695996443112 t^{55}+15639566550683151661395 t^{54}+45733839198189308795922 t^{53}-34336550387552217444788 t^{52}-90156610374907391306510 t^{51}+56170231702738096480627 t^{50}+163407130266810623547342 t^{49}-59674655787100839841498 t^{48}-260974340231967460261742 t^{47}+1379539820945602522975 t^{46}+337355991736851476351861 t^{45}+162387269952090328397329 t^{44}-279819533153184521617525 t^{43}-401647530895617404618072 t^{42}-57868582293607116920946 t^{41}+515641259742587397418566 t^{40}+688681142230757597125130 t^{39}-165793150470240212399830 t^{38}-1263311589433764390361365 t^{37}-795435576972012167321111 t^{36}+1094611975754783586306770 t^{35}+1805947994521233034507392 t^{34}+120041263723506144853053 t^{33}-1765373380222620639449333 t^{32}-1506752084937680410601914 t^{31}+230957441089910035348667 t^{30}+1351006601274254281335522 t^{29}+1302480718243875455908294 t^{28}+1029281509841449133926798 t^{27}+1080130664802908538522808 t^{26}+1094997012919857117778404 t^{25}+738967014294474705125999 t^{24}+220213625365992444182685 t^{23}-106398789883913842239068 t^{22}-164716108592947135153710 t^{21}-103127120592856899540123 t^{20}-52471722297650948898488 t^{19}-37279606422220871920476 t^{18}-32794588907678932138156 t^{17}-23825654818318932672397 t^{16}-12500220329345417090980 t^{15}-4279171697737781114493 t^{14}-490355197693774215016 t^{13}+480554206988052866945 t^{12}+409502507441656273097 t^{11}+192906764337718614980 t^{10}+65963310056596974135 t^9+17430143430369149581 t^8+3617285226594311851 t^7+588820712988449327 t^6+74605122243978491 t^5+7333387690440310 t^4+568274076038157 t^3+35867870347521 t^2+1766148235252 t+49073994451\right)+d^{35} \left(720526249688 t^{78}-7010645489810 t^{77}+11077759154072 t^{76}+140843894223083 t^{75}-809897084003131 t^{74}+983840705559132 t^{73}+5319546947779826 t^{72}-20556726130019450 t^{71}+1605550588680928 t^{70}+132635006342215004 t^{69}-206650729927928190 t^{68}-459752550867404639 t^{67}+1549307982701522478 t^{66}+647795364882288820 t^{65}-7163364028908857981 t^{64}+2431698305038297500 t^{63}+24827426919455484085 t^{62}-20524281364303306505 t^{61}-70212906970997335889 t^{60}+83201755897669398082 t^{59}+171551389844240114919 t^{58}-245469930933549032925 t^{57}-382262820286088549077 t^{56}+576804721785443411904 t^{55}+803112251488544699525 t^{54}-1118904945840085706526 t^{53}-1621482581686479499505 t^{52}+1763227343340282756769 t^{51}+3067269096523896815914 t^{50}-2138050935428863661858 t^{49}-5290770914450501855965 t^{48}+1498528773264185362320 t^{47}+8015797644547723122922 t^{46}+1203279511675834584480 t^{45}-9652868856152804928673 t^{44}-5385766809299188629737 t^{43}+9933229762116032604537 t^{42}+12759134882910238815182 t^{41}-2115428800047898699208 t^{40}-11729173152191784778221 t^{39}-363977823486213704978 t^{38}+16375988825957691325988 t^{37}+15519766536535744691036 t^{36}-1229972324657443338661 t^{35}-14269276032782504235048 t^{34}-14325830604653757959827 t^{33}-9048867764944908265728 t^{32}-6594544149127612547186 t^{31}-5691278159836054830724 t^{30}-2138356595717609140551 t^{29}+3446597007871164043415 t^{28}+7073776899213011684248 t^{27}+6681430921766236888336 t^{26}+3683846561246733795847 t^{25}+657615384967629175008 t^{24}-971125023869343762514 t^{23}-1274009404202258002582 t^{22}-949657788693484944240 t^{21}-549112722251665980849 t^{20}-276226222863700766553 t^{19}-128582724906637896444 t^{18}-55529979629131247544 t^{17}-21013620671941373854 t^{16}-6299687399877923169 t^{15}-1233920360361496893 t^{14}-47836864033698089 t^{13}+42068372586618041 t^{12}-7450091989024936 t^{11}-19869450652832325 t^{10}-12087476108846390 t^9-4653416768108787 t^8-1313199665622414 t^7-284357482887583 t^6-47754134860516 t^5-6158556927927 t^4-592295194289 t^3-40126296103 t^2-1710718935 t-34539545\right)+d^{34} \left(875832352864 t^{78}-10916598348792 t^{77}+46723361817458 t^{76}+10975906022788 t^{75}-887913010231882 t^{74}+3214105750401673 t^{73}-480229674466093 t^{72}-27542378010755875 t^{71}+62623704900933253 t^{70}+74093515767134121 t^{69}-485325594136563836 t^{68}+205576741385517393 t^{67}+2132914869429733708 t^{66}-2715450969556059198 t^{65}-6672016858566371362 t^{64}+13769767444182934384 t^{63}+16541846276685936152 t^{62}-49167733628788272470 t^{61}-35826833301425388767 t^{60}+140195667110486601507 t^{59}+76903770663614183264 t^{58}-334541123911003085199 t^{57}-185429908731965940270 t^{56}+672692774637986099651 t^{55}+489381663442078660993 t^{54}-1117911047823572835598 t^{53}-1266456774879065409469 t^{52}+1377055378918480714963 t^{51}+2871144959656525222378 t^{50}-733418980002441935205 t^{49}-5491115165632687910492 t^{48}-2132811892787574053774 t^{47}+8330176143555216292867 t^{46}+8542280234880854860836 t^{45}-8821699280362914556402 t^{44}-17758635475363413917478 t^{43}+4700624532912000848922 t^{42}+29046851990875540548435 t^{41}+11635972970852520587157 t^{40}-25623880221423049232655 t^{39}-20357416745689074812239 t^{38}+27203303519967375225030 t^{37}+49478596916874601959368 t^{36}+16918711738809071965890 t^{35}-22273706086049402239690 t^{34}-23048705060181970148824 t^{33}-3782314412284835263011 t^{32}-3207943803811018416188 t^{31}-21515277840775593732886 t^{30}-30670884861327982048375 t^{29}-18168014293731099906241 t^{28}+2495422562169689436354 t^{27}+14418596978978385163616 t^{26}+14138426181093357084763 t^{25}+8133286119722398969278 t^{24}+2718091759753469322416 t^{23}-79096463355730170911 t^{22}-936182867113115560382 t^{21}-926278702411963461269 t^{20}-666008299374658271659 t^{19}-400427922952148946873 t^{18}-207999569586971575249 t^{17}-96074324230766663785 t^{16}-41624885975994602336 t^{15}-18049064903050989614 t^{14}-8005503406187795392 t^{13}-3469684564794694220 t^{12}-1374908591206502482 t^{11}-475526719028918266 t^{10}-140108965495117985 t^9-34733501690996366 t^8-7183428248048920 t^7-1228234892023861 t^6-171420658108302 t^5-19141966746853 t^4-1654330519327 t^3-104372401879 t^2-4288918437 t-86180198\right)+d^{24} \left(893320001192 t^{78}-25748788868864 t^{77}+330698130867528 t^{76}-2427524659919022 t^{75}+10559883567530448 t^{74}-22303939239635008 t^{73}-20949556648300394 t^{72}+265722336519224824 t^{71}-546805035380933904 t^{70}-649980463380501274 t^{69}+4844297125156299610 t^{68}-4430193138430051684 t^{67}-20160212821359958296 t^{66}+50242612165907045105 t^{65}+34194414564945475529 t^{64}-257648172636645914851 t^{63}+116985136372244636776 t^{62}+852733026378463143958 t^{61}-1074381397657498071722 t^{60}-1917044315027232197949 t^{59}+4278982999309681427596 t^{58}+2710964941616120487196 t^{57}-11567595721721422352085 t^{56}-1131192738603683192971 t^{55}+23216317928673995894141 t^{54}-5398597695306121525441 t^{53}-34488346134467026454508 t^{52}+17529113806609182292125 t^{51}+32015042399927190215273 t^{50}-34225261361994112194004 t^{49}+7173293340792997441058 t^{48}+63436183657701967769623 t^{47}-106730903508437620481477 t^{46}-144389604342599153633715 t^{45}+257867998715411276535727 t^{44}+355834531588289636849733 t^{43}-357763482844051117753723 t^{42}-750337538386274016200315 t^{41}+178521224385529852279169 t^{40}+1184566192862845240438842 t^{39}+484086328464144088987124 t^{38}-1203543070892361469370930 t^{37}-1420661740563918526044011 t^{36}+349769663652757895686109 t^{35}+1772942052032991635958965 t^{34}+1005518226704563557367299 t^{33}-804311209455756949890770 t^{32}-1446038200153950150356222 t^{31}-652968989946819519612501 t^{30}+189729758603273320933058 t^{29}+358754070944286427067910 t^{28}+398525627033960395456122 t^{27}+842082289895284984446892 t^{26}+1455449370751654427164961 t^{25}+1750583497328591742597673 t^{24}+1584803203579732154506846 t^{23}+1138639943589505779009993 t^{22}+643139664805268478528963 t^{21}+252080986570440009351002 t^{20}+31553017652278702966470 t^{19}-35013635529558911176981 t^{18}-18357053636844115175903 t^{17}+11824857376098800825476 t^{16}+23793767860446494051484 t^{15}+19314421996972454366430 t^{14}+10298047359185899947902 t^{13}+3873164611214981728582 t^{12}+967152078573021465307 t^{11}+92800567876194167697 t^{10}-47523489134423209754 t^9-30710686999879492085 t^8-10438871184034863636 t^7-2552456133437928170 t^6-481034801536442759 t^5-70729540721302237 t^4-7944865488827248 t^3-643898793292985 t^2-33458055656690 t-832493232833\right)+d^{25} \left(1006864247288 t^{78}-27429469233766 t^{77}+325929503406538 t^{76}-2123306774384964 t^{75}+7295558569034720 t^{74}-4265428662453408 t^{73}-73222497572308530 t^{72}+290462502549158984 t^{71}-157133356979701836 t^{70}-1979064525704575810 t^{69}+5506380351834325636 t^{68}+2097518635169496492 t^{67}-35710227344366447245 t^{66}+43541102584665380374 t^{65}+112057577189214507984 t^{64}-324520458798354429166 t^{63}-105773903939048385454 t^{62}+1290772220946614759146 t^{61}-684481624097730610355 t^{60}-3551590523830661152854 t^{59}+4091533214767155483881 t^{58}+7420862112892451390320 t^{57}-13166218477917084928056 t^{56}-12597251307740466052553 t^{55}+31003102593554392570220 t^{54}+18963392279346182463023 t^{53}-57789316176884619537252 t^{52}-28277410737261722724381 t^{51}+85851759087798948808095 t^{50}+42869478889534205753066 t^{49}-93896822381021927344568 t^{48}-53863483222764127026231 t^{47}+48368943815401966132545 t^{46}+16012807134629246925708 t^{45}+68023582421260087960836 t^{44}+168964958446633756800492 t^{43}-184442687062040281850301 t^{42}-598180371837135149589900 t^{41}+73054631980496561243791 t^{40}+1187237743531401478745824 t^{39}+554498586673441907304516 t^{38}-1482326217805572960385587 t^{37}-1653567555809003066495513 t^{36}+841171065612695559908591 t^{35}+2421833605647856142729764 t^{34}+706799356838240209512868 t^{33}-1790476850875970562731672 t^{32}-1839417517748973108297663 t^{31}-68748458391147131130264 t^{30}+963530389394508799486808 t^{29}+751468514323575584325256 t^{28}+647426014811063488544958 t^{27}+1220677025231166595232064 t^{26}+1707527480097131704629427 t^{25}+1490448491658437039564670 t^{24}+846009646079438914058496 t^{23}+320357854013912774765648 t^{22}+88788839917993816828252 t^{21}+18100579221119090090278 t^{20}-18484173334701539483813 t^{19}-41654123423631509719240 t^{18}-39620231398585459743596 t^{17}-20851023219714362621856 t^{16}-3561956235946701374149 t^{15}+4048760070893905956873 t^{14}+4471024353766991963441 t^{13}+2598607736861146678294 t^{12}+1061083513382861700236 t^{11}+321493767735845584061 t^{10}+70315842655578105678 t^9+9135703601344443521 t^8-330425955310812563 t^7-542209759143788359 t^6-161318507774921645 t^5-29722536461618108 t^4-3742470935653356 t^3-315703328060969 t^2-16157740932997 t-379447963767\right)+169

==> polynomials/Q_7,11.tex <==
d^7 \left(4 t^{11}-4 t^{10}-13 t^9-5 t^8+2 t^7+t^6\right)+d^6 \left(16 t^{11}-40 t^{10}-33 t^9+75 t^8+17 t^7-141 t^6-135 t^5-21 t^4+35 t^3+26 t^2+8 t+1\right)+d^5 \left(20 t^{11}-76 t^{10}+4 t^9+184 t^8-91 t^7-348 t^6-189 t^5-60 t^4-113 t^3-119 t^2-51 t-8\right)+d^4 \left(16 t^{10}-69 t^9+13 t^8+152 t^7-12 t^6-454 t^5-697 t^4-401 t^3-27 t^2+53 t+14\right)+d^3 \left(-20 t^{11}+164 t^{10}-359 t^9-147 t^8+1063 t^7+130 t^6-1480 t^5-1014 t^4+88 t^3+317 t^2+118 t+13\right)+d^2 \left(-16 t^{11}+152 t^{10}-401 t^9-51 t^8+1253 t^7-218 t^6-1689 t^5-335 t^4+623 t^3+233 t^2-29 t-13\right)+d \left(-4 t^{11}+44 t^{10}-128 t^9-44 t^8+520 t^7-55 t^6-806 t^5-92 t^4+449 t^3+115 t^2-88 t-32\right)+7 t^9-49 t^8+72 t^7+95 t^6-193 t^5-98 t^4+157 t^3+61 t^2-47 t-20

==> polynomials/Q_8,12.tex <==
d^8 \left(4 t^{12}+2 t^{11}\right)+d^7 \left(20 t^{12}-17 t^{11}-11 t^{10}+70 t^9+52 t^8+t^7-6 t^6-t^5\right)+d^6 \left(36 t^{12}-76 t^{11}-3 t^{10}+266 t^9+9 t^8-118 t^7+285 t^6+353 t^5+80 t^4-55 t^3-39 t^2-10 t-1\right)+d^5 \left(20 t^{12}-56 t^{11}-21 t^{10}+298 t^9-37 t^8-353 t^7+567 t^6+1100 t^5+568 t^4+168 t^3+87 t^2+36 t+5\right)+d^4 \left(-20 t^{12}+125 t^{11}-260 t^{10}+14 t^9+695 t^8-519 t^7-759 t^6+1349 t^5+2058 t^4+1030 t^3+297 t^2+77 t+13\right)+d^3 \left(-36 t^{12}+247 t^{11}-505 t^{10}-194 t^9+1702 t^8-566 t^7-2892 t^6+770 t^5+3692 t^4+1904 t^3-11 t^2-211 t-40\right)+d^2 \left(-20 t^{12}+158 t^{11}-351 t^{10}-206 t^9+1491 t^8-281 t^7-2875 t^6+78 t^5+3183 t^4+1679 t^3-341 t^2-429 t-74\right)+d \left(-4 t^{12}+34 t^{11}-63 t^{10}-158 t^9+531 t^8+162 t^7-1257 t^6-328 t^5+1325 t^4+861 t^3-173 t^2-308 t-82\right)-t^{11}+14 t^{10}-58 t^9+53 t^8+162 t^7-251 t^6-223 t^5+313 t^4+230 t^3-90 t^2-82 t-10
